Field-based Security Testing of SDN configuration Updates

Software-defined systems revolutionized the management of hardware devices but introduced quality assurance challenges that remain to be tackled. For example, software defined networks (SDNs) became a key technology for the prompt reconfigurations of network services in many sectors including telecommunications, data centers, financial services, cloud providers, and manufacturing industry. Unfortunately, reconfigurations may lead to mistakes that compromise the dependability of the provided services. In this paper, we focus on the reconfigurations of network services in the satellite communication sector, and target security requirements, which are often hard to verify; for example, although connectivity may function properly, confidentiality may be broken by packets forwarded to a wrong destination. We propose an approach for FIeld-based Security Testing of SDN Configurations Updates (FISTS). First, it probes the network before and after configuration updates. Then, using the collected data, it relies on unsupervised machine learning algorithms to prioritize the inspection of suspicious node responses, after identifying the network nodes that likely match across the two configurations. Our empirical evaluation has been conducted with network data from simulated and real SDN configuration updates for our industry partner, a world-leading satellite operator. Our results show that, when combined with K-Nearest Neighbour, FISTS leads to best results (up to 0.95 precision and 1.00 recall). Further, we demonstrated its scalability.

==> RQ2plots.tex <==
% !TEX root =  MAIN.tex

\begin{figure*}
\begin{minipage}{.45\textwidth}
	\includegraphics[width=7cm]{data/RQ1_SameActionBudget_ALL_1Hour_COMPARISON_modifiedMethodCoverage}
	\vspace{-1cm}
      \caption{Percentage of updated methods covered for each version of the case studies (budget=1 hour).}
      \label{fig:RQ1:Method:1}
\end{minipage}\hspace{5mm}
\begin{minipage}{.45\textwidth}
	\includegraphics[width=7cm]{data/RQ1_SameActionBudget_ALL_5Hours_COMPARISON_modifiedMethodCoverage}
		\vspace{-1cm}
      \caption{Percentage of updated methods covered for each version of the case studies (budget=5 hours).}
      \label{fig:RQ1:Method:5}
\end{minipage}
\begin{minipage}{.45\textwidth}
	\vspace{-7mm}
	\includegraphics[width=7cm]{data/RQ1_SameActionBudget_ALL_1Hour_COMPARISON_modifiedInstructionsCoverage}
		\vspace{-1cm}
      \caption{Percentage of instructions belonging to updated methods that are covered for each version of the case studies (budget=1 hour).}
      \label{fig:RQ1:Instr:1}
\end{minipage}\hspace{5mm}
\begin{minipage}{.45\textwidth}
	\vspace{-7mm}
	\includegraphics[width=7cm]{data/RQ1_SameActionBudget_ALL_5Hours_COMPARISON_modifiedInstructionsCoverage}
		\vspace{-1cm}
      \caption{Percentage of instructions belonging to updated methods that are covered for each version of the case studies (budget=5 hours).}
      \label{fig:RQ1:Instr:5}
\end{minipage}
\end{figure*}


==> algos/executeTesting.tex <==
% !TEX root =  ../Main.tex

%\vspace{-3mm}
\begin{algorithm}[tb]

\begin{algorithmic}[1]

%\footnotesize
\scriptsize
%\Require \emph{MR}, the bytecode of the metamorphic relation to be executed
%\Require \emph{dataProvider}, an object that exposes the data collected by the crawlers
%\Ensure \emph{Failures}, a list of failing executions with contextual information
% (source inputs, follow-up inputs, output data).

\While { ( NOT stagnation() ) AND ( NOT phaseBudgetConsumed( \emph{phaseBudget}) ) AND (NOT coverageTargetsExercised() ) } \label{algo:test:loop}
	\If { target not selected OR target already exercised OR \emph{visitBudget} exhausted}	\label{algo:test:checkSelectedTarget}
		\State selectTarget() \label{algo:test:select}
		\State identifyPathToTarget() \label{algo:test:path}
	\ElsIf { target unreachable}	\label{algo:test:target:unreachable}
		\State identifyPathToTarget() \label{algo:test:unreachable:path}
	\EndIf


	
\If { NOT\ targetReached() }   \label{algo:test:notTarget}

		\State reachTargetNode( \emph{reachabilityBudget} ) \label{algo:test:reachTarget}
\Else	\label{algo:test:TargetReached}
%	\If { first time the active window is visited }	
%		\State performRandomScrolling()  \label{algo:test:randomScolling}
%	\EndIf	
	\State exerciseTarget( \emph{targetBudget} )	\label{algo:test:execTarget}
\EndIf

	\If {additional random exploration required }   \label{algo:test:randomRequired}
		\State performRandomExploration( \emph{randomExplorationBudget} )	\label{algo:test:execRandom}
	\EndIf
	
\EndWhile



\end{algorithmic}

\caption{\APPR testing algorithm.}
%\vspace{-0.2cm}
\label{alg:testing}
\end{algorithm}



==> algos/generateUpdatedAppModel.tex <==
% !TEX root =  ../Main.tex

%\vspace{-3mm}
\begin{algorithm}[tb]

\begin{algorithmic}[1]

%\footnotesize
\scriptsize
\Require \emph{$M_b$}, the base App Model
\Require \emph{$MW_u$}, the EWTG of the updated version, generated by an extension of Gator
\Require \emph{Diff}, the EWTGDiff computed in the step

%\Require \emph{dataProvider}, an object that exposes the data collected by the crawlers
%\Ensure \emph{Failures}, a list of failing executions with contextual information
% (source inputs, follow-up inputs, output data).
%Fabrizio: since we do not have. a formal definition of the structure of Diff, it is better to have an informal descriptio, same for theothers
\For {each diff $\in$ Window differences set in Diff}
    \If {diff is Addition}
        \State w $\gets$ (diff$\rightarrow$getAddedElement())
        \State markWindowAsAddition(w) \label{algo:genUpdate:markAddition1}
    \ElsIf {diff is Deletion}
        \State w $\gets$ (diff$\rightarrow$getDeletedElement())
        \State removeAbstractStates(w) \label{algo:genUpdate:removeAbstractStates}
    \Else
        \State windowReplacement $\gets$ (diff$\rightarrow$getReplacementElement())
        \State reassignAbstractStatesToNewWindow(windowReplacement)
    \EndIf
\EndFor
\For {each diff $\in$ Widget differences set in Diff}
    \If {diff is Addition}
        \State w $\gets$ (diff$\rightarrow$getAddedElement())
        \State markWidgetAsAddition(w) \label{algo:genUpdate:markAddition2}
    \ElsIf {diff is Deletion}
        \State w $\gets$ (diff$\rightarrow$getDeletedElement())
        \State removeAbstractValuationMaps(w) \label{algo:genUpdate:removeAVMs}
    \Else
        \State widgetReplacement $\gets$ (diff$\rightarrow$getReplacementElement())
        \State reassignAttributeValuationMapsToNewWidget(widgetReplacement)
    \EndIf
\EndFor
\For {each diff $\in$ Diff$\rightarrow$ Transition differences set in Diff}
    \If {diff is Addition}
        \State w $\gets$ (diff$\rightarrow$getAddedElement())
        \State markTransitionAsAddition(w) \label{algo:genUpdate:markAddition3}
    \ElsIf {diff is Deletion}
        \State w $\gets$ (diff$\rightarrow$getDeletedElement())
        \State removeAbstractTransitions(w) \label{algo:genUpdate:removeAbTransitions}
    \Else
        \State transitionReplacement $\gets$ (diff$\rightarrow$getReplacementElement())
        \State t $\gets$ (transitionReplacement$\rightarrow$replaced)
        \State removeAbstractTransitions(t)
    \EndIf
\EndFor
\end{algorithmic}

\caption{\APPR's Updated App model generation}
%\vspace{-0.2cm}
\label{algo:generateUpdatedAppModel}
\end{algorithm}



==> oldRQ2.tex <==

\subsection{RQ2: Test effort over lifecycle}

\subsubsection{Experiment design}

A surrogate measure of the effort required to test an App over its lifecycle is the overall number of instructions belonging to updated methods that are not covered by automated testing. Indeed, engineers have to manually implement test cases that exercise these instructions. Therefore, for all the case study Apps, we identify all the instructions belonging to the updated methods of versions V0 to V9 that that need to be tested manually. 
For a given test automation tool $T$ and an App $A$, we measure the effort required to test $A$ over its lifecycle as the sum of the number of instructions that need to be tested manually in the i-th run according to the formula
$\mathit{effort}_{T,A,i}=\sum_{v=\mathit{V1}}^{\mathit{VL}}{\mathit{missing}_{T}(v)}$,
where $\mathit{missing}(v)$ is the number of instructions not covered by the test automation tool $T$ for version $v$, and VL is the last available version for the App A (usually V9).

For each subject of the study, we measure, in percentage points, the effort reduction of \AutAut with respect to another test automation approach $O$, according to the formula
$$\mathit{reduction}_{O,i}=\frac{\mathit{effort}_{O}-\mathit{effort}_{\APPR}}{\mathit{effort}_{O}}*100$$

We inspect the distribution of the effort reduction for the different approaches and case study systems. To positively answer our research question, the effort reduction should be always positive and significant.



\subsubsection{Results}

Figures~\ref{fig:RQ2:InstrNotCovered:1} and ~\ref{fig:RQ2:InstrNotCovered:5} show, for each case study, the percentage of instructions that should be manually tested, when a certain test automation tools is used. \APPR achieves the best results since the median and the average number of instructions to be manually tested is below the one obtained by the other techniques.

Table~\ref{table:RQ2} shows the effort reduction of \AutAut with respect to the other test automation approaches. In general, \AutAut shows a positive reduction, which indicates that \APPR is a better  choice to test Apps in their lifecycle. Further, \APPR performs better than other approaches with a larger test execution budget as well, thus suggesting that the generated models enable an optimal use of the test budget.

\begin{figure}[t]
  \centering
	\includegraphics[width=8.5cm]{data/RQ2_1Hour_COMPARISON_instructions_NotCovered_over_lifecycle}
      \caption{Percentage of instructions that need to be manually tested for each subject of the study (budget=1 hour).}
      \label{fig:RQ2:InstrNotCovered:1}
\end{figure}

\begin{figure}[t]
  \centering
	\includegraphics[width=8.5cm]{data/RQ2_5Hours_COMPARISON_instructions_NotCovered_over_lifecycle}
      \caption{Percentage of instructions that need to be manually tested for each subject of the study (budget=5 hours).}
      \label{fig:RQ2:InstrNotCovered:5}
\end{figure}

\input{tables/RQ2.tex}








==> old_approach.tex <==
% !TEX root =  MAIN.tex

\section{Proposed Approach: \APPR}
\label{sec:approach}
\begin{figure}
\includegraphics[width=8.4cm]{images/updateProcess.png}
\caption{\APPR process}
\label{fig:updateprocess}
\end{figure}
\APPR supports engineers in testing App upgrades by incrementally refining App models. By reusing the DSTG generated for a base App version, \APPR aims to optimize testing efficiency by minimizing the effort spent to generate AbstractStates and AbstractTransitions, for every version. Similarly to \ATUA, for every App version, \APPR aims to exercise all the methods that are either introduced in the updated App (i.e., new methods) or whose implementation has been modified between the two App versions (i.e., modified methods). We refer to such methods as \emph{updated methods}.

For the first version of the App under test (hereafter, App V0), \APPR relies on the same strategy implemented by \ATUA to automatically test the App and generate an App model. For App V0, \APPR treats each method as a modified method. 
%\FIXME{For methods not automatically exercised by \ATUA, we expect engineers to manually test the App in order to ensure method coverage. After testing App V0, an App model including the results of manual testing is kept; it will be reused for testing following App versions.}

For every App version following V0, \APPR relies on the App model produced for the previous App version to drive testing. 
We refer to the previous version of an App as \emph{base App version}, the new version of the App is the \emph{updated App version}. Similarly, we refer to App models as \emph{base App model} and \emph{updated App model}.

To test an updated App, \APPR works in four steps, shown in Figure~\ref{fig:updateprocess}. In Step 1, \APPR relies on an extension of RCVDiff to 
compare the EWTGs generated by \ATUA's extended Gator for the base and updated version of the App.

In Step 2, \APPR relies on the identified differences to generate an updated App model by adapting the EWTG and the DSTG of the base App model. 

In Step 3, \APPR relies on \ATUA to test the updated App. However, \APPR extends the testing process implemented in \ATUA such that, during testing, the AbstractState reached after every input is compared with the AbstractState expected according to the App model. In case of mismatches, \APPR updates the model to reflect the actual behaviour of the App under test. Furthermore, to assist the identification of test sequence reaching desired inputs, \APPR employs \emph{probabilistic path}, which in general is based on the prediction of missing AbstractTransitions.

The output of Step 3 is an App model for the updated App version. Also, \APPR generates a report with a set of triples $<$GUI screenshot, target action, GUI screenshot$>$ reporting for every target action\footnote{According to \ATUA, a target action is an action that triggers the execution of a target method (see Section~\ref{sec:background}).} triggered by \APPR the screenshot before and after the execution of the action. An example is shown in Figure~\ref{fig:actionOutput}). To avoid wasting engineers time, only actions that increase code coverage (i.e., that exercise instructions not tested yet) are reported. The generated triples support crowdsourcing-based oracles (e.g., they can be shared among a set of App user to determine if the output is functionally correct or not). 
%The output generated by non target actions, instead, might be used as automated oracle to detect regression faults. More precisely, by comparing the GSTG generated for two App versions, we can automatically determine likely regression faults by looking for non target actions that are triggered in the same App state (e.g., same screenshot or abstract state before the action) but bring the App in different App states (i.e., different screenshot or abstract state after the action). 

\begin{figure}
\includegraphics[width=8.4cm]{images/actionReport.png}
\caption{Example of action output being reported to the end-user}
\label{fig:actionOutput}
\end{figure}

In Step 4, after testing, \APPR refines the App model and the test input sequence. Step 4 aims to eliminate  non-determinism and infeasible paths in the App model. It consists of re-executing the testing sequence recorded in the GSTG and annotating the AbstractStates in the GSTG that do not match the observed ones. the latter, are oftendue to obsolescent states, which are AbstractStates unlikely to be reached again (e.g., the one characterizing a news list that changes every minute). Finally, it aims to minimize the sequence of test inputs to be presented to engineers.
The  output of Step 4 is a refined App model for the updated App and a minimized sequence of test inputs and outputs (i.e., App screenshots and App GUItrees) generated during testing.

In the following sections, 
after discussing the App changes that should be reflected in the updated App model (Section~\ref{sec:updatedAppModel}),
we provide the details of the four steps implemented by \APPR.

%Fabrizio: in the picture of the process, it would be nice if somehow you show that DSTG V2 comes from DSTGV1 while EWTG-V2 comes from static analysis.
\subsection{Updated App Models}
\label{sec:updatedAppModel}


%Fabrizio: we need this section to motivate what we are doing
An App model contains three submodels: EWTG, DSTG, and GSTG. In \ATUA and, consequently, in \APPR, the EWTG and the DSTG are used to (1) identify the sequence of inputs required to reach a desired Window or a specific AbstractState and then (2) trigger an input that exercises a target transition. The GSTG, instead, is used to keep track of all the inputs triggered and all the GUITrees encountered during testing. When the testing process ends, the GSTG is used to derive 
%at the end of testing 
the sequence of inputs and outputs provided to the engineer. 
During testing, the GSTG is used to refine the DSTG in the presence of nondeterminism; more precisely, to split a state leading to nondeterminism into multiple deterministic states,
\ATUA applies the refined state abstraction function to the information stored in the GSTG and regenerates the AttributeValuationMaps (see Section~\ref{back:atua}).
%the refinement of abstract states lead to the replacement of an abstract state with multiple abstract states. Consequently, state transitions departing from the original state should be replaced with new state transitions departing from the new sub states. To regenerate state transitions, \ATUA simply  

To speed-up testing, we aim to automatically generate an updated App model containing information that is likely correct for the updated App and can be inherited from the base App model. 

The updated EWTG does not need to be derived from the base EWTG because it
 is automatically generated by means of static program analysis applied to the updated App.

%In \ATUA, the DSTG is generated at runtime, based on the App outputs for the triggered inputs. 
%Since the DSTG plays a critical role to optimize the test budget and identify a reduced set of input events, inheriting the DSTG from the base version would enable a more efficient use of the test budget. 
%Since the DSTG reflects the behavior of the App, which might change across versions (e.g., the output for two inputs might be different across two versions), the DSTG of the updated App (hereafter, updated DSTG) might differ from the  DSTG for the base App (base DSTG). 

The updated DSTG, instead, should be derived from the base DSTG because it cannot be generated by means of static analysis. When generating the updated DSTG, we should take into account the differences between the two App versions, which
 might be due to either changes in the GUI structure (e.g., the removal of a button impedes a state transition observable with the base App) or changes in the implementation of the App (e.g., a change of the event handlers logic leads to different outputs for a same set of inputs across two versions).
The effect that changes in the GUI structure have on the DSTG, can be determined based on the changes between the base and the updated EWTG 
(e.g., the removal of a widget impedes the triggering of input events for that widget); 
the effect of implementation changes, instead, cannot be determined without executing the App.
For these reasons, to generate the updated App model, \APPR creates a copy of the base DSTG and automatically modifies it to reflect changes in the GUI structure that have been detected with static analysis.
Also, \APPR continuously updates the DSTG at runtime, during testing, based on the observed behaviour, to reflect differences due to the updated program logic. More precisely, every time an unexpected abstract state is reached, \APPR determines if the actual and the expected abstract states are equivalent, and updates the DSTG accordingly.

% The updated GSTG can be inherited from the base App model and updated at runtime similarly to the DSTG; an inherited GSTG may provide the benefit of enabling the refinement of App states using historical data. However, since any inherited GUI state might be outdated, the result of such refinement might still lead to outdated abstract states, thus resulting in wasting test budget (outdated abstract states lead to invalid input sequences and may need to be reconstructed). 
% Therefore, \APPR does not inherit the GSTG.

\APPR does not inherit the GSTG because any inherited GUI state might be outdated thus leading to outdated abstract states and resulting in wasting test budget.
%The problem might be further exacerbated by the large number of GUI states;
%indeed the GSTG contains a different GUI state for every GUITree differing for widget properties or for cosmetic (rendering) aspects.



%the large number of GUI states makes it particularly expensive.
%The DSTG plays a
% critical role to optimize the test budget and identify a reduced set of input events; indeed, it helps
%determine a correct and reduced sequence of events necessary to reach a specific Window from
% another one.


\subsection{Detect EWTG differences}

\begin{figure}
\includegraphics[width=8.4cm]{images/rcvdiff-staruml/rcvdiff-wtg.png}
\caption{EWTG represented as an RCVModel. See Table~\ref{tab:ewtgmodel} for legend.}
\label{fig:rcvdiff:wtg}
\end{figure}



\input{tables/ewtgmodel}


%To detect differences in EWTG, \APPR extends RCVDiff with  comparison functions specific for EWTG elements. 
%They are described below.
%
% We leverage RCVDiff to compute the WTGDiff. This is done by four steps that extend the RCVDiff process.



In Step 1, \APPR compares two EWTGs to identify a set of differences, which we refer to as EWTGDiff (Extended Window Transition Graph Differences). 
To generate an EWTGDiff, \APPR extends the RCVDiff process with three activities, described below: (1) \emph{Generate an RCVModel from the base and updated EWTGs}, (2) \emph{Identify differences with EWTG-specific comparison functions}, and (3) \emph{Generate an EWTGDiff from the DifferencesModel}.


\subsubsection{Generate an RCVModel from the base and updated EWTGs}

To identify differences with RCVDiff, \APPR transforms parts of the EWTG models for two App versions into an RCVModel. 
When generating the RCVModel, \APPR considers only a subset of the properties of Window, Widgets, and Transitions.
Figure~\ref{fig:rcvdiff:wtg} shows how the EWTG elements are modeled within an RCVModel. For example, a \emph{Window} is associated to its \emph{windowType}, \emph{className}, and the contained \emph{Widget}s.


%Specifically, a \emph{Window} is associated to its \emph{windowType} (e.g., Activity, Dialog, or OptionsMenu), \emph{className}, and the contained \emph{Widget}s; %\FIXME{Moreover, if a Window is a Dialog, it is additional associated to the \emph{ownerActivity} and the \emph{created location}; if a Window is an OptionsMenu, it is associated to the \emph{ownerActivity} };
%a \emph{Widget} is associated with its \emph{className}, \emph{resourceId}, \emph{xpath}, \emph{parent} and its \emph{children}; finally, a \emph{Transition} is associated with a \emph{source} Window, a \emph{destination} Window, an \emph{actionType}, and a \emph{targetWidget}. The \emph{actionType} and the \emph{targetWidget} are used to model the input triggering a transition.

\subsubsection{Identify differences with EWTG-specific comparison functions}


To identify differences between two App models, we extend the difference calculation process of RCVDiff with signature-based and EWTG-specific similarity functions.

RCVDiff relies on a tree-matching algorithm that identifies matching elements based on attributes, references, and sub-elements (see Section~\ref{rcvdiff}). In our extension, each of these elements are first compared using a signature-based function.
The signature-based function is used to identify matching elements (e.g., Windows) independently from their content (e.g., the widgets contained in a Window may change across versions despite the window remains the same). This is achieved by constructing signatures from a subset of properties specific for the different EWTG element types. 
More precisely,
we generate a signature for an EWTG element by combining the values of the attributes and references captured in the RCVModel.
Signature-based matching simply relies on  string matching, i.e., two elements match when their signatures are the same.


For every element for which a signature match is not found, \APPR configures the RCVDiff matching process to rely on an EWTG-specific similarity function that takes into account the semantic of the EWTG elements.
The EWTG-specific similarity function implements the following rules:
\begin{itemize}
%Fabrizi: I do not find a good reason for the change you made
%    \item \FIXME{A Widget could be changed in several ways. We assume that a widget's changes should be related to only one of its attributes or its parent. For example, two Widgets match when all their attributes match and their parents are different.}
    \item Since a Widget could be moved to another container (i.e., its parent changes), two Widgets can match when all their attributes, except \emph{parent}, match. Also, since a Widget could be replaced with another one implementing similar features (e.g., a button replaced by a clickable image), they can match when all their attributes, except \emph{className}, match.
   % \item \FIXME{To match, two widgets should be of the same \emph{locator}. A \emph{locator} could be a full locator or a partly one. A full locator of a widget is the combination of the \emph{resourceId}, the \emph{className}, the \emph{xpath}, the \emph{parent}, and the \emph{children} of the widget. A \emph{partly locator} is represented by five out of the six components of the full locator.}
    \item To match, two Windows should extend the same Window Type (i.e., Activity, Dialog, OptionsMenu, or ContextMenu) and their other properties should match (e.g., class name). 
    \item To match, two Transitions should start from matching sources (i.e., Windows) and trigger the same action on a matching widget (e.g., a Button).
        \item To match, element attributes
        %, which are always strings (for the attributes selected by \APPR), 
        should have a low string similarity distance. More precisely, we rely on the Levenshtein ratio with a threshold of 40\% to compare string values. The Levenshtein ratio is employed because most strings in this context are relatively short (i.e., less than {256} characters). The chosen threshold has been empirically demonstrated to be appropriate in related work~\cite{Pan2020a}, as it enables handling cosmetic changes (e.g., fixing typos in a textual label).
        %
        {However, for xPaths, which represent the position of a Widget in the containing Window following a specific grammar (e.g., the symbol \emph{/} separates ancestor Windows), we rely on token-based distance. \emph{Token-based distance functions} split each string into tokens (we use the symbol \emph{/} as separator) and compute similarity between the two token sets; we rely on \emph{Cosine similarity}~\cite{Yu2016}.}
        %\FIXME{However, this is not applied to \emph{xPath} attributes since a difference of a single char in a \emph{xPath} is sufficient to indicate a very different element. xPath attributes match only if they synctatically match.}
     \end{itemize}
     
     \begin{figure}
\includegraphics[width=8cm]{images/rcvdiff-staruml/ewtgdiff.png}
\caption{EWTGDiff metamodel.}
\label{fig:rcvdiff:EWTGDiff}
\end{figure}



\begin{figure*}
\includegraphics[width=13cm]{images/rcvdiff-staruml/rcvdiff-wtg-diff-example.png}
\caption{Example Detected EWTG differences}
\label{fig:rcvdiff:wtgdiff}
\end{figure*}
     
\subsubsection{Generate an EWTGDiff from the DifferencesModel}

Figure~\ref{fig:rcvdiff:EWTGDiff} provides the EWTGDiff metamodel. It captures the differences concerning the EWTG element types processed in Step 2 to generate an updated the App model, which are \emph{Window}, \emph{Widget} and \emph{Transition}. For each element, \APPR identifies three types of differences: \emph{Addition}, \emph{Deletion}, and \emph{Replacement}, which are collected in the respective \emph{AdditionSet}, \emph{DeletionSet}, and \emph{ReplacementSet}. Addition and Deletion are straightforward. A Replacement indicates that an element E1 in the base model has been replaced by an element E2 in the updated model. 
%In the EWTGDiff, the above-mentioned differences are represented by the following model elements 
%AddedElement, DeletedElement, and ReplacedElement. Also, the EWTGDiff captures differences among referenced models as AddedReference, DeletedReference, and ReplacedReference.
%For attributes, which are stable across versions because depend on our toolsets for extracting static and dynamic data, \APPR reports only changes in their valuation (i.e., ChangeAttribute).
%The EWTG contains

%Fabrizio never use "/" in the text     
To produce an EWTGDiff, \APPR processes the DifferencesModel generated by RCVDiff. For each AddedElement (or DeletedElement), it puts the referred element to the Addition set (or Deletion set) of the corresponding element type. For example, \APPR puts a Widget labeled by RCVDiff as an AddedElement in the Addition set of Widget differences. 
 For each ReplacedElement, we construct a pair including the element in V1 and the element in V2.
 % (i.e., reportedElement and newElement respectively).

  
Figure~\ref{fig:rcvdiff:wtgdiff} illustrates the detection of EWTG differences with an example. In Figure~\ref{fig:rcvdiff:wtgdiff}, we visualize two EWTG models using a UML object diagram  in which each MElement (e.g., a Window) is represented as an object, each MAttribute is represented as an object attribute, and each MReference is represented with a link. For example, a window of type \emph{MainActivity} is represented as a Window-typed object with the  field \emph{className} valued "MainActivity". %Furthermore, the links between the elements and the models are hidden to enhance visibility. 
%Fabrizio: you wrote Difference Meta model, not sure what is correct, but we should minimize the use of differnet terms
%Chanh Duc: Differences metamodel is an extended part of RCVDiff's EMMM.
The items with a red border are elements belonging to the DifferencesModel. In the example in Figure~\ref{fig:rcvdiff:wtgdiff}, the differences between models V1 and V2 are:
\begin{itemize}
    \item The Window named \emph{MainActivity} has been renamed as \emph{HomeActivity}
    \item In the \emph{MainActivity} Window, the value of the className attribute of the widget \emph{addNewItem} has been changed from \emph{Button} to \emph{ImageView}.
    \item In the \emph{EditActivity} Window, a new widget has been added (i.e., the Button named \emph{cancel}). Consequently, a new transition triggered by this widget has been added.
\end{itemize}

%Fabrizio: you were missing many verbs here, you cannot write 'ChangedElement to the "MainActivity" Window'
%Chanh Duc: I see. Thanks
The DifferencesModel, in red in Figure~\ref{fig:rcvdiff:wtgdiff}, reflects the differences listed above and thus contains:
\begin{itemize}
%Fabrizio: in the Figure the red associations point to the updated model, while in this text you refer to the base one, we should be consistent
%Chanh Duc: Not sure I understand which part of the text you referred to. But in the Figure, there are two red associations; one points to the base model, the other points to the updated model
%Fabrizio what is "w1" ?
%Chanh Duc: I wanted to name the element with a name that is used in the explanation of the generation of EWTGDiff
    \item A ReplacedElement associated to the \emph{MainActivity} Window (w1). It is composed of an \emph{AttributeDifference} associated to the attribute \emph{className} and a \emph{ReplacedElement} associated to the  Button  \emph{addNewItem} (wid1).
    \item A ReplacedElement associated to the Window \emph{EditActivity} (w2). It is comprised of an \emph{AddedElement} associated to the \emph{Cancel} Button (wid2).
    \item An AddedElement associated to the Transition (t1) that has the \emph{Cancel} Button as its targetWidget (in the App model, the targetWidget indicates which Widget triggers the transition).
\end{itemize}

The EWTGDiff generated by \APPR contains the following difference sets:
\begin{itemize}
    \item Window differences: Addition=$\emptyset$,  Deletion=$\emptyset$,  
    Replacement= $\{w1[MainActivity\rightarrow HomeActivity]\}$; 
    \item Widget differences: Addition=$\{wid2\}$, Deletion=$\emptyset$, Replacement= $\{wid1[ImageView\rightarrow Button]\}$
    \item Transition differences: Addition=$\{t1\}$, Deletion=$\emptyset$, Replacement= $\emptyset$
\end{itemize}

\subsection{Generating an Updated App model}
\input{algos/generateUpdatedAppModel}
%Fabrizio: many steps are misisng in your description
%Since (1) the EWTG and the DSTG are strongly coupled (i.e., there are a multitude of references between DSTG and EWTG elements), and (2) the base EWTG includes refinements made during testing (e.g., to remove infeasible transitions), \APPR, instead of including in the updated App model the EWTG generated for the updated App, it modifies the base EWTG to match the updated one. 
The generation of the updated App model consists of four activities: (1) copying the base App model, (2) removing all the GSTG elements (see Section~\ref{sec:updatedAppModel}), (3) replace the base EWTG with the updated EWTG, and (4) update the DSTG. 
Since the first fur activities are straightforward, we describe only the procedure for updating the DSTG, which is provided also  in 
Algorithm~\ref{algo:generateUpdatedAppModel}.

Algorithm~\ref{algo:generateUpdatedAppModel} receives as input the base App model, the EWTG of the updated App, and the EWTGDiff.
It is described in the following paragraphs.


%\FIXME{Concerning the DSTG, it copies all the elements belonging to the DSTG (nodes and associations), then it updates the associations connecting DSTG elements and EWTG elements. More precisely, for each DSTG element, for each association ending with an EWTG element present in the base App model, it creates, in the updated App model, an association to the EWTG element  that matched the one in the base model, according to the DifferencesModel.}

%Fabrizio: below, Merge is not the rght verb, in addition, you are not saying what you do for nodes that are not modified
%The EWTG of the base version (V1) of an App needs to be merged with the EWTG of the updated version (V2) with regard to the computed WTGDiff, to become a new model. 

%Fabrizio:use \emph not "
\APPR removes from the updated DSTG all the elements in the EWTGDiff's \emph{Deletion} sets. More precisely, if the deleted element is a Window, \APPR removes all the abstract states associated with the Window 
%Fabrizio: pleae add line references for all the following sentences
(Line~\ref{algo:genUpdate:removeAbstractStates} in Algorithm~\ref{algo:generateUpdatedAppModel}). If the deleted element is a Widget, \APPR removes all the AttributeValuationMaps associated with the Widget 
{(Line~\ref{algo:genUpdate:removeAVMs})}. If the deleted element is a Transition, \APPR removes all the abstract transitions associated with the transition 
{(Line~\ref{algo:genUpdate:removeAbTransitions})}.



%Fabrizio: we need a running example to describe this whole section
{For each ReplacementPair in the \emph{Window Replacement} set, \APPR assigns the replaced element's AbstractStates to the replacing element. Concerning ReplacementPairs in the \emph{Transition Replacement} set, since they indicate a change in the source or destination window but there is no mean to determine the mapping to an abstract state for that window, we simply remove the AbstractTransitions associated to the replaced Transition.}

The elements in the \emph{Addition} sets do not lead to any update of the DSTG because such elements were not present in the  base version and, consequently, they do not appear in the updated DSTG. However, we keep track all the added elements in the updated EWTG {(see markAsAddition in Lines~\ref{algo:genUpdate:markAddition1}, ~\ref{algo:genUpdate:markAddition2}, ~\ref{algo:genUpdate:markAddition3})}.

\subsection{Extension of testing process}
\subsubsection{Runtime adaptation of the updated DSTG}
\label{sec:runtime:adapt}

\input{algos/runtimeAdapation}
The runtime adaptation of the updated DSTG is necessary to preserve the reuse of the base DSTG, even in the presence of mismatches due to changes in the programming logic of the updated App. 
The adaptation is performed at runtime, while the testing algorithm (i.e, ATUA) executes a test input sequence. 
In \ATUA, test input sequences are used to reach an abstract state of a target Window and to  trigger a target transition once the target Window is reached.
Test input sequences are derived from the App model; 
consequently, for every test input it is possible to identify an abstract state that is expected to be reached. When the expected abstract state is not reached, we are in the presence of nondeterminism, that is, a same input may lead to two different abstract states, namely \emph{StateA} and \emph{StateB}. 
\ATUA tries to prevent nondeterminism by refining the state abstraction function; the refinement has the objective to replace the departing state for the nondeterministic transition in order to distinguish between the case in which the input leads to \emph{StateA} and to \emph{StateB}. 
If the refinement of the state abstraction function does not help removing nondeterminism, \ATUA keeps a nondeterministic model.

In the presence of a DSTG model derived from the base App model, we might
reach a state different than the expected one not only because of nondeterminism or lack of proper refinement strategy but also because of a change in the updated App. 
In the second case, it is important to distinguish between an abstract state that is equivalent to the expected one and an abstract state that is nonequivalent. 
An equivalent state presents a different set of widgets but enables end-users to perform the same actions for the expected state and, consequently, to reach the same expected follow-up states.
Detecting equivalent states is important to preserve the reuse of the DSTG derived from the base App model. 
For example, if the updated App version introduces a reset button for a Window with a form, an input sequence exercising the submit button, which has not been modified, should remain executable in the updated version.

%Nonequivalent states simply indicate that the App behaves differently than expected; they should be handled by introducing a new abstract state in the DSTG. 
For the reasons above, \APPR, 
%Fabrizio: will we still do it?
%
{before trying to remove nondeterminism by relying on the \ATUA's testing process,} determines if the observed state is equivalent to the expected one.
%Fabrizio: the algorithm should describe what we do when a state is equivalent and nonequiavelent (ie., first refine the abstract function, if refinement does not go well a new state is added and then the expected state tagged for removal - a state tagged for removal and never observed in a test execution is removed at the end of the process)
The process followed by \APPR is depicted in Algorithm~\ref{algo:runtimeadaptation}. It is executed every time a transition is triggered. Algorithm~\ref{algo:runtimeadaptation} receives as input the departing state $s_d$ (i.e., the abstract state reached by the application before triggering the last input), the observed state $s_o$ (i.e., the state reached after triggering the last input), and the expected state $s_e$ (i.e., the state expected based on the DSTG).
Before describing the algorithm, we present the concepts of \emph{AttributeValuationMap equivalence} and \emph{state backward-equivalence}, which are building blocks of the approach.

{In \ATUA and, consequently, in \APPR, each AttributeValuationMap is univocally identified by its attribute valuations and its cardinality. Therefore, two AttributeValuationsMaps are equivalent when their attribute valuations and cardinality match.}
{In addition, in \APPR, to preserve input sequences in the presence of replaced widgets (e.g., a button replaced by a clickable image), two AttributeValuationMaps are equivalent even if not all their attribute valuations match but only their interactive attributes (e.g., clickable, see Table~\ref{table:reducers}) match and they are both associated with a same EWTG widget, which should be a replacing widget.}

We introduce the notion of \emph{state backward-equivalence} to identify abstract states of the updated App that enable end-users to perform the same actions that could be performed in backward-equivalent states of the base App. A backward-equivalent abstract state, in practice, enables end-users to trigger, on the updated App, the inputs that could be triggered on the base App. Two states are backward-equivalent when they differ only for Widgets that have been introduced in the updated App {or the ones that only detected at runtime (i.e., not detected by the static analysis)}.
More precisely, an abstract state $s_o$ observed in the updated App is backward-equivalent to a state $s_e$ derived from the base DSTG when:

%Fabrizio: you were not motivating your choices, it is important
\begin{itemize}
    \item $s_e$ and $s_o$ are associated to the same Window. Otherwise, since different Windows are used for different features, they cannot be equivalent, by definition.
    \item Every AttributeValuationMap in $s_e$ , except the ones belonging to the widgets detected at runtime, matches (i.e., is equivalent to) an AttributeValuationMap in $s_o$. Otherwise, it would not be possible to trigger in $s_o$ the same inputs triggerable in $s_e$.
    %Fabrizio: does it really make sense what we have below?
    %Chanh Duc: Could  it be that an AttributeValuationMap is actually a newly added one in $S_0$ but does not belong to any EWTG widget because of the limitation of static analysis or due to the guitree generation of Android? In that case, the following will make $S_O$ and $S_E$ not backward-equivalent.
    \item Every AttributeValuationMap in $s_o$, except the ones for EWTG widgets belonging to the Addition sets of the EWTGDiff and the ones belonging to the widgets detected at runtime, matches an AttributeValuationMap in $s_e$. 
    If this condition does not hold, a Widget may have two different AttributeValuationMaps in the two App versions (e.g., a checkbox is no longer checked). A widget with a different AttributeValuationMap in the base and updated App indicates that the updated App has changed its behaviour and, consequently, a same test input may not lead to the same state in the base and upgraded version.
\end{itemize}


%We introduce the notion of \emph{quasi-backward-equivalence} to identify states in the updated App that enable the execution of a subset of the inputs that could be executed in the corresponding state of the base App.
%An abstract state $S_O$ observed in the updated App is quasi-backward-equivalent to a state $S_E$ derived from the base DSTG when
%\begin{itemize}
 %   \item $S_E$ and $S_O$ are associated to the same Window,  as for backward-equivalence;
 %   \item the next input in the test input sequence leads to either the expected state, a backward-equivalent state, or a quasi-backward-equivalent state.
%\end{itemize}

We now describe the procedure for updating the App model, which is shown in Algorithm~\ref{algo:runtimeadaptation}. When the expected ($s_e$) and the observed state ($s_o$) match, the algorithm does not have to remove the non-determinism in the DSTG and \APPR proceeds with triggering the next input in the test input sequence (Line~\ref{algo:update:continuewhenbackequv}).

%Fabrizio: the algorithm should have, at the end, lines dedicated to handling nonequiavelnt cases (Another one below)
If $s_o$ and $s_e$ are non-equivalent, reaching $s_o$ is likely the result of a change in the App implementation. Consequently, \APPR  removes from the DSTG the abstract transition connecting $s_d$  to $S_e$ (Line~\ref{algo:update:removeabstracttransition1}).
Also, if $s_e$ has already been observed while testing the updated App, $s_o$ simply represents a new abstract state and there is no need to check for backward-equivalence {(Line \ref{algo:update:stateobservedbefore})}.

%If $S_O$ belongs to the same Window of $S_E$  and $S_O$ and $S_E$ are not backward-equivalent {(Line \ref{algo:update:verifyquasibackequv})}, the algorithm proceeds verifying \emph{quasi-backward-equivalence}. In practice, 
%it verifies  for the AttributeValuationMap targeted by the next input.
%If it is not found, the algorithm considers the two states nonequivalent and proceeds accordingly (Line Y).
%it triggers the next input and verifies the expected output according to \emph{quasi-backward-equivalence} rules. The verification of \emph{quasi-backward-equivalence} is recursive, i.e., we might observe a sequence of potential \emph{quasi-backward-equivalent} states that are confirmed to be \emph{quasi-backward-equivalent} only after processing a sequence of test inputs that reaches an equivalent-state.
%To speed-up verification, if two states are recognized as being quasi-backward-equivalent for an input $i$, we track the information so that we do not need to check it again for other test sequences exercised later. Similarly, we keep track also of states that are recognized as not being quasi-backward-equivalent for an input $i$ (i.e., they reach nonequivalent states).
%
%\begin{itemize}
%    \item The resulting state $s2$ belongs to the same Window as the destination state $s1$ (of the abstract transition) is. If $s2$ is equivalent to $s1$, we update the abstract transition's destination to $s2$ and all the abstract transitions from the state $s1$ are transferred to the state $s1$. Otherwise, we try examining the \textbf{likely equivalent}  relationship between $s1$ and $s2$ by following the executing test sequence. If $s2$ is a likely equivalent to $s1$, it enables a test sequence through $s1$ to be replaced with $s2$.
%    If the AVM cannot be identified in $s2$, the examination terminates. Contrarily, the examination is achieved by triggering the corresponding input on the AVM in $s2$ expected by the current test sequence. If the expected state $s3$ is reached, which means that a resulting state $s4$ is equivalent to $s3$, $s1$ and $s2$ are tagged as being likely equivalent.
%    \item The resulting state $s2$ belongs to a different window than the destination state $s1$ is. In this case, we simply remove the invalid abstract transition.
%\end{itemize}

\subsubsection{Probabilistic path} \label{sec:probabilistic-path}

ATUA’s state abstraction mechanism enable determine if an App is in a different abstract state. It facilitates the identification of test input sequences when each App state depends on the immediately previous Abstract transition but it might be unsuccessful when it depends on older actions (or more in general persistent state information). This is particularly detrimental when reusing models to test a newer App because several abstract stats may be visible only if the App was put in a certain state by executing some action (but these actions are now not performed) or by executing long sequence of actions. Furthermore, the state space could be large so we would not exhaustively explore the Apps.

For that reason, we propose \emph{Probabilistic path}, which is a special mechanism allowing \APPR to identify paths reaching expected inputs based on the probabilistic of reaching inputs after exercising another one. When a path needs to be identified, \APPR augments the DSTG by adding transitions for every unexercised input in traversed state. These transitions are called meta-transitions. For an unexercised input $i$ in a state, one or more meta-transitions are added if it was exercised in the history. A meta-transition has destination as a meta-state, which is constructed based on the reachable widgets in the history when the input $i$ was exercised in other states. Each input of a meta-state is associated with a probability representing the confidentiality of the availability of the input. For example, if exercising an input $i_{1}$ brought Apps to states having a widget $w_1$ in 8 out of 10 times in the history, the probability of reaching $w_{1}$ by exercising $i_{1}$ is 0.8. Then, a meta-state has outgoing transition(s) for each input targeting any of the widgets in the state.

Since a meta-transition would be infeasible in practice, paths should not be selected based on the shortest sequence of actions. For example, a path formed by 5 "real" transitions should be more reliable then one formed by 4 meta-transitions. To assist the selection of paths, we propose cost calculation as the following:
\[ c(\phi)= \sum_{j=1}^{n} c(i_{j}) + \frac{\sum_{j=1}^{n} c(i_{j}}{2} \times \left( 1-\prod_{j=1}^{n+1} p(i_{j}|s_{j}) \right)\]

\begin{itemize}
    \item \(c(i)\) : atomic cost (i.e., cost of exercising an input i)
    \begin{itemize}
        \item \(c(i)=10\) if i is reset input 
        \item \(c(i)=1\) if i is not reset input 
    \end{itemize}
    \item \(p(i|s)\) : probability of an input \(i\) available in a state \(s\)
    \begin{itemize}
        \item \(p(i|s) = 1.0\) if s is not a meta-state.
        \item \(p(i|s)\) is the probability of the input i enabled by exercising the previous input in the sequence.
    \end{itemize}
\end{itemize}

The intuition of the formula is that when \APPR follows a probabilistic path, the path could be broken anytime. Then, on average, half of the test budget would be wasted.

\subsubsection{Memory-guarded abstract transition}

\begin{figure}[h!]
     \centering
     \begin{subfigure}[b]{0.5\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/memory-guarded-example1.png}
         \caption{Closing a dialog brings App back to the exact state in that the dialog was opened.}
         \label{fig:memory-guarded-example1}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.5\textwidth}
         \centering
         \includegraphics[width=\textwidth]{images/memory-guared-example2.png}
         \caption{Adding a new activity brings App to a state similar to a state before the "Add" action but with the newly added activity.}
         \label{fig:memory-guarded-example2}
     \end{subfigure}
     \hfill
      \caption{Examples from Activity Diary App\footnote{https://f-droid.org/en/packages/de.rampro.activitydiary/} of particular transitions which bring App back to a previous Activity}
    \label{fig:memory-guarded-example}
\end{figure}
A limitation of ATUA is the presence of nondeterministic due to particular transitions of which the destinations are (derivation of) states observed in the test sequence. These transitions are transitions bring App back to a previous Activity. Figure~\ref{fig:memory-guarded-example} illustrates some examples of this type of transitions. In example~\ref{fig:memory-guarded-example1}, given that App is in a state $s_{1}$ of the MainActivity, the "Edit Note" dialog is opened and then is closed, and App is brought back to $s_{1}$. In example~\ref{fig:memory-guarded-example2}, after adding a new activity with input $i_4$, App is brought back to state $s_5$, which is derived from state $s_1$
% One common category of these transitions are an input on a Dialog brings App to the Activity opening that Dialog. When returning to the previous Activity, the state reached by this input could be the same as the one before the dialog is opened or it could be a similar one. Figure~\ref{} illustrates an example of this type of transition. In both cases (a) and (b), the same input on the same state of the Dialog brings App back to the states in that the Dialog was opened. This problem not only results in nondeterminism but also increases inaccuracy of probabilistic paths (described in section \ref{sec:probabilistic-path}). In case that an input brings Apps to a previous Activity, the availability of inputs does not depend only on the exercise of an input but it also depends on if these inputs are available in the most recent state.
These situations mislead ATUA attempting to reach the some dependent states such as $s_1$ and $s_5$ in examples~\ref{fig:memory-guarded-example1} and ~\ref{fig:memory-guarded-example2} respectively. Furthermore, they increase inaccuracy of probabilistic paths (described in section \ref{sec:probabilistic-path}). In case that an input brings Apps to a previous Activity, the availability of inputs does not depend only on the exercise of an input but it also depends on if these inputs are available in the most recent state.

To tackle the problems, \APPR guards abstract transitions with the previous state which is the most recent layout-similar to their destinations if these transitions bring App to a previous Activity. An abstract transition guarded with this mechanism is called a \emph{memory-guarded abstract transition}. We refer to the layout-similar state because an Activity could have different layouts (e.g., by replacing different fragments) and a transition could bring App back to a specific layout of the Activity. In example \ref{fig:memory-guarded-example2}, the transition from $s_4$ to $s_5$, triggered by the input $i_4$, should be guarded by $s_1$, not $s_2$.

Layout of an abstract state can be derived by employing level 1 of granularity of abstraction functions for all widgets in GUI Trees. With level 1, only static information of widget (i.e., resource id, class name, parent) is considered. In the other words, we transform an abstract state to a layout-level abstract state by keeping only static information of attribute valuation maps in the abstract state. We refer these attribute valuation maps as \emph{layout-components} (or \emph{components} for short).  Two layouts are similar if they share a majority of components. Given two layouts denoted $L_1$ and $L_2$ and $\Pi_{L_1}$, $\Pi_{L_2}$ is set of layout-components in $L_i$, $L_2$ respectively, the shared proportion $\Theta$ between $L_1$ and $L_2$ is calculated as following:
\[\Theta(L_1,L_2)=\frac{2 \times |L_1 \cap  L_2|}{|L_1|+|L_2|}\]
To be similar, $\Theta(L_1, L_2)$ should be less than a threshold $\omega_{\Theta}$. Based on our experience, we set $\omega_{\Theta}$ as 0.8.
\subsection{Refine the App model.}

The refinement of the App Model consists of removing information that is obsolescent. There are two types of obsolescent information.
% (i.e., abstract states and state transitions that correctly model a previous version of the App but are not representative for the current App version under test) and therefore shall not be kept to test future App versions. Keeping obsolete abstract states is detrimental for testing because they make the algorithm identify test paths that, during testing, should be discarded because they do not bring to the desired state.
\subsubsection{Removing information not representative for the updated App version}
Please note that the \APPR's runtime adaptation algorithm already detects changes in the App behaviour between two App versions that affect what is visualized on the GUI after an action (i.e., show a different window or an unexpected abstract state). Such changes lead to the removal of abstract transitions that are obsolete from the DSTG (see Section~\ref{sec:runtime:adapt}). However, the \APPR's runtime adaptation algorithm cannot determine if a subset of abstract states becomes unreachable in practice. For example, the testing algorithm never triggers a certain state transition. For nondeterministic transitions such behavior may depend on the fact that the App behaviour changes, for other transitions it might depend on the fact that the transition is never selected to reach a target window (i.e., a window to test).
Since we cannot be sure about the reasons for which a state transition is never triggered and, consequently, an abstract app state is never reached, to determine if an abstract state is obsolete, we look for abstract states that are not visualized and belong to windows traversed during testing. Such abstract states are considered obsolete and removed from the DSTG. The others, instead, are kept.

%When refining the App model, \APPR also complements some limitations of static analysis by removing from the EWTG widgets that are never observed during testing (i.e., they do not appear in the DSTG). These widgets are for example widgets that, within a Window hierarchy, belong to the parent Window but not to the  In principle, the trimmed model would contain only the information that is interesting for the next version.

\subsubsection{Obsolescent state identification}
For some Apps the content of a window and consequently the App state depends on the data provided by a remote component (e.g., server) whose responses change over time. We refer these App states as \emph{obsolescent states}. Since the obsolescent states could not be reached again after a period of time, the effort that attempts to bring Apps to these states in the testing of upgrades is wasteful.

Apparent obsolescent states could be easily identified by replaying recently executed test sequences. During re-executing a test sequence, if the observed App state \(s_o\) is not the same as the expected one \(s_e\), \(s_e\) is annotated as obsolescent. To tackle test flakiness (e.g., a state is retrieved when its elements have not been completely loaded), when a state observed is not as expected, we wait until App is stable (i.e., not any new element appears). 

In the testing of updated versions, \APPR will not try reaching the obsolescent states if they are not observed again. Furthermore, for any abstract state belonging to a window having obsolescent abstract states, if it could not be reached by an attempt, \APPR annotates it as obsolescent, and consequently the abstract state would not be attempted to reach anymore.

==> tables/NMAP_SCAN.tex <==
% !TEX root =  ../MAIN.tex

% \begin{table}[tb]
% \caption{\NMAP scan options.}
% \label{table:NMAP:scans}
% \footnotesize
% \begin{tabular}{|p{2cm}|p{6cm}|}
% \hline

% \textbf{Scan type}&\textbf{Description}\\
% \hline
%  TCP SYN&Sends a request port connection.\\
%  TCP Connect()&Establishes a connection with the target issuing the connect system call provided by the OS (used when TCP SYN is not feasible).\\
%  TCP ACK&Used to determine if a stateful firewall had been configured. Sends probes with only ACK flag set. Ports replyng with an RST packet are labeled as unfiltered, fitered otherwise.\\
%  TCP Window&Sends an ACK probe and interprets non-zero Window values to determine open ports.\\
%  TCP Maimon&Sends a FIN/ACK probe, which is dropped in BSD if port is open.\\
% UDP&Sends UPD packets with payload set based on the port.\\
%  TCP Null&Do not set any bit.\\
%  TCP FIN&Set the FIN flag.\\
%  TCP Xmas scans&Sets the FIN, PSH, and URG flags.\\
%  TCP custom& Customized selection of flags is possible.\\
%   Idle scan&Trigger connection from a third part and probe the therd pary IP ID.\\
%   %-sY/sZ: SCTP INIT/COOKIE-ECHO scans
%   IP&Use IP packet headers to determine available IP protocols and ports.\\
%   %-b <FTP relay host>: FTP bounce scan
% \hline
% \end{tabular}
% \end{table}%



% Please add the following required packages to your document preamble:
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table}[tb]
%\footnotesize
\caption{\NMAP scan options.}
\label{table:NMAP:scans}
\scriptsize
\begin{tabular}{cp{2.3in}}
\hline
\hline
\textbf{Scan type }     & \textbf{Description}                                                                                                                                                                       \\ \hline\hline
 TCP SYN        & Sends a request port connection.                                                                                                                                                  \\ \hline
TCP Connect()  & Establishes a connection with the target issuing the connect system call provided by the OS (used when TCP SYN is not feasible).                                                  \\ \hline
TCP ACK        & Used to determine if a stateful firewall had been configured. Sends probes with only ACK flag set. Ports replyng with an RST packet are labeled as unfiltered, fitered otherwise. \\ \hline
TCP Window     & Sends an ACK probe and interprets non-zero Window values to determine open ports.                                                                                                 \\ \hline
TCP Maimon     & Sends a FIN/ACK probe, which is dropped in BSD if port is open.                                                                                                                   \\ \hline
UDP            & Sends UDP packets with payload set based on the port.                                                                                                                             \\ \hline
TCP Null       & Do not set any bit.                                                                                                                                                               \\ \hline
TCP FIN        & Set the FIN flag.                                                                                                                                                                 \\ \hline
TCP Xmas scans & Sets the FIN, PSH, and URG flags.                                                                                                                                                 \\ \hline
TCP custom     & Customized selection of flags is possible.                                                                                                                                        \\ \hline
Idle scan      & Trigger connection from a third part and probe the third party IP ID.                                                                                                              \\ \hline
IP             & Use IP packet headers to determine available IP protocols and ports.                                                                                                              \\ \hline \hline
\end{tabular}
\end{table}

==> tables/NSCR_state_table_Detailed.tex <==
\begin{table*}[]

\caption{NCSR report example}
\label{NSCR_state_table_Detailed}
\centering
\scriptsize
\begin{tabular}{cccccccccc}
\hline \hline
\textbf{IP'}   & \textbf{IP"}   & \textbf{tcp\_Port 22}     & \textbf{udp\_Port 22}           & \textbf{tcp\_Port 445} &  \textbf{udp\_Port 445}              & \textbf{tcp\_Port 8080}                  & \textbf{...}                            & \textbf{udp\_Port 5674 }     \\ \hline \hline
192.168.56.113 & 192.168.56.113 & ClosedToClosed & ClosedToClosed  & ClosedToClosed                   & ClosedToClosed& ClosedToClosed & ...                 & ClosedToClosed \\ \hline
192.168.56.114 & 192.168.56.214 & ClosedToClosed & ClosedToClosed  & ClosedToClosed                   & \textit{\textbf{OpenToClosed}} & ClosedToClosed& ... & ClosedToClosed \\ \hline
192.168.56.15  & 192.168.56.115  & ClosedToClosed & ClosedToClosed  & ClosedToClosed & ClosedToClosed& ClosedToClosed & ...                 & ClosedToClosed \\ \hline

... & ... & ...&  ...                  & ... & ...         &...        & ...& ... \\
\hline
192.168.56.118 & 192.168.56.118 & ClosedToClosed & ClosedToClosed  & \textit{\textbf{OpenToFiltered}}        & ClosedToClosed           & ClosedToClosed & ...                 & ClosedToClosed \\ \hline \hline


\end{tabular}
\end{table*}

==> tables/RQ1_MannWhitney_VDA_Summary.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[tb]
\footnotesize
\caption{Number of versions in which \APPR performs significantly better than competing approaches and vice-versa. }
\label{table:RQ1_versions}
\begin{tabular}{|p{11mm}|l|l|l|l|}
\hline
\multirow{2}{*}{\textbf{Tool}}   & \multicolumn{2}{c|}{\textbf{Target method coverage}} & \multicolumn{2}{c|}{\textbf{Target instruction coverage}} \\
                            & CALM better          & CALM  worse       & CALM better             & CALM worse            \\ \hline 
% ATUA                        & 39 (75\%)              & 0 (0\%)               & 43 (82.69\%)                & 0 (0\%)                  \\ \hline 
ATUA-U              & 41 (78.85\%)              & 0 (0\%)               & 46 (88.46\%)                & 0 (0\%)                  \\ \hline 
ATUA-R-U              & 37 (71.15\%)              & 2 (3.85\%)               & 37 (71.15\%)                & 2 (3.85\%)                  \\ \hline 
% APE                         & 23 (44.23\%)              & 15 (28.85\%)             & 22 (42.31\%)                & 16 (30.77\%)                \\ \hline 
APE-U & 44 (84.62\%)              & 2 (3.85\%)               & 50 (96.15\%)                & 0 (0\%)                 \\ \hline 
Monkey                      & 35 (67.31\%)              & 4 (7.69\%)               & 35 (67.31\%)                & 4 (7.69\%)  \\  \hline             
Fastbot2                      & 38 (73.08\%)              & 1 (1.92\%)               & 37 (71.15\%)                & 2 (3.85\%)  \\  \hline   
\end{tabular}
\end{table}

==> tables/RQ1_VDA_Mannwhitney.tex <==
\begin{table*}[]
\footnotesize
\label{table:RQ1:vda_mannwhitney}
\begin{tabular}{|c|c|c|cccccccc|cccccccc|}
\hline
\multicolumn{1}{|c|}{}             & \textbf{}   & \textbf{}   & \multicolumn{8}{c|}{\textbf{Coverage of target methods}}                                                                                                                                                                                                                        & \multicolumn{8}{c|}{\textbf{Coverage of target instructions}}                                                                                                                                                                                                                   \\ \hline
\multicolumn{1}{|c|}{}             & \textbf{}   & \textbf{}   & \multicolumn{4}{c|}{\textbf{A12}}                                                                                                        & \multicolumn{4}{c|}{\textbf{p-value}}                                                                                                & \multicolumn{4}{c|}{\textbf{A12}}                                                                                                        & \multicolumn{4}{c|}{\textbf{p-value}}                                                                                                \\ \hline
\multicolumn{1}{|c|}{\textbf{App}} & \textbf{V1} & \textbf{V2} & \multicolumn{1}{c|}{\textbf{AT}} & \multicolumn{1}{c|}{\textbf{AP}} & \multicolumn{1}{c|}{\textbf{AU}} & \multicolumn{1}{c|}{\textbf{M}} & \multicolumn{1}{c|}{\textbf{AT}}     & \multicolumn{1}{c|}{\textbf{AP}}     & \multicolumn{1}{c|}{\textbf{AU}}     & \textbf{M}      & \multicolumn{1}{c|}{\textbf{AT}} & \multicolumn{1}{c|}{\textbf{AP}} & \multicolumn{1}{c|}{\textbf{AU}} & \multicolumn{1}{c|}{\textbf{M}} & \multicolumn{1}{c|}{\textbf{AT}}     & \multicolumn{1}{c|}{\textbf{AP}}     & \multicolumn{1}{c|}{\textbf{AU}}     & \textbf{M}      \\ \hline
activitydiary                      & 105         & 111         & \multicolumn{1}{c|}{0.50}        & \multicolumn{1}{c|}{0.00}        & \multicolumn{1}{c|}{0.07}        & \multicolumn{1}{c|}{0.03}       & \multicolumn{1}{c|}{-}               & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 & \multicolumn{1}{c|}{0.50}        & \multicolumn{1}{c|}{0.00}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{1.00}       & \multicolumn{1}{c|}{-}               & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 \\ \hline
activitydiary                      & 111         & 115         & \multicolumn{1}{c|}{0.50}        & \multicolumn{1}{c|}{0.50}        & \multicolumn{1}{c|}{0.60}        & \multicolumn{1}{c|}{0.65}       & \multicolumn{1}{c|}{-}               & \multicolumn{1}{c|}{-}               & \multicolumn{1}{c|}{0.07}            & \textless{}0.05 & \multicolumn{1}{c|}{0.50}        & \multicolumn{1}{c|}{0.50}        & \multicolumn{1}{c|}{0.65}        & \multicolumn{1}{c|}{1.00}       & \multicolumn{1}{c|}{-}               & \multicolumn{1}{c|}{-}               & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 \\ \hline
activitydiary                      & 115         & 118         & \multicolumn{1}{c|}{0.50}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{1.00}       & \multicolumn{1}{c|}{-}               & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 & \multicolumn{1}{c|}{0.50}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{1.00}       & \multicolumn{1}{c|}{-}               & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 \\ \hline
activitydiary                      & 118         & 122         & \multicolumn{1}{c|}{0.95}        & \multicolumn{1}{c|}{0.94}        & \multicolumn{1}{c|}{0.97}        & \multicolumn{1}{c|}{1.00}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.94}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{1.00}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 \\ \hline
activitydiary                      & 122         & 125         & \multicolumn{1}{c|}{0.88}        & \multicolumn{1}{c|}{0.85}        & \multicolumn{1}{c|}{0.94}        & \multicolumn{1}{c|}{0.95}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 & \multicolumn{1}{c|}{0.66}        & \multicolumn{1}{c|}{0.85}        & \multicolumn{1}{c|}{0.98}        & \multicolumn{1}{c|}{1.00}       & \multicolumn{1}{c|}{0.12}            & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 \\ \hline
activitydiary                      & 125         & 130         & \multicolumn{1}{c|}{0.93}        & \multicolumn{1}{c|}{0.58}        & \multicolumn{1}{c|}{0.80}        & \multicolumn{1}{c|}{1.00}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{0.26}            & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 & \multicolumn{1}{c|}{0.98}        & \multicolumn{1}{c|}{0.58}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{1.00}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{0.26}            & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 \\ \hline
activitydiary                      & 130         & 131         & \multicolumn{1}{c|}{0.50}        & \multicolumn{1}{c|}{0.50}        & \multicolumn{1}{c|}{0.50}        & \multicolumn{1}{c|}{0.40}       & \multicolumn{1}{c|}{-}               & \multicolumn{1}{c|}{-}               & \multicolumn{1}{c|}{-}               & 0.07            & \multicolumn{1}{c|}{0.50}        & \multicolumn{1}{c|}{0.50}        & \multicolumn{1}{c|}{0.50}        & \multicolumn{1}{c|}{0.80}       & \multicolumn{1}{c|}{-}               & \multicolumn{1}{c|}{-}               & \multicolumn{1}{c|}{-}               & \textless{}0.05 \\ \hline
activitydiary                      & 131         & 134         & \multicolumn{1}{c|}{0.85}        & \multicolumn{1}{c|}{0.95}        & \multicolumn{1}{c|}{0.99}        & \multicolumn{1}{c|}{1.00}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 & \multicolumn{1}{c|}{0.79}        & \multicolumn{1}{c|}{0.95}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{1.00}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 \\ \hline
amazefile                          & 11          & 12          & \multicolumn{1}{c|}{0.89}        & \multicolumn{1}{c|}{0.12}        & \multicolumn{1}{c|}{0.89}        & \multicolumn{1}{c|}{0.96}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 & \multicolumn{1}{c|}{0.90}        & \multicolumn{1}{c|}{0.12}        & \multicolumn{1}{c|}{0.94}        & \multicolumn{1}{c|}{0.97}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 \\ \hline
amazefile                          & 12          & 16          & \multicolumn{1}{c|}{0.97}        & \multicolumn{1}{c|}{0.79}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{1.00}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.79}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{1.00}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 \\ \hline
amazefile                          & 16          & 17          & \multicolumn{1}{c|}{0.95}        & \multicolumn{1}{c|}{0.46}        & \multicolumn{1}{c|}{0.61}        & \multicolumn{1}{c|}{1.00}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{-}               & \multicolumn{1}{c|}{0.16}            & \textless{}0.05 & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.46}        & \multicolumn{1}{c|}{0.94}        & \multicolumn{1}{c|}{1.00}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{-}               & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 \\ \hline
amazefile                          & 17          & 18          & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.86}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{1.00}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.86}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.98}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 \\ \hline
bbc                                & 16          & 17          & \multicolumn{1}{c|}{0.73}        & \multicolumn{1}{c|}{0.27}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.79}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 & \multicolumn{1}{c|}{0.81}        & \multicolumn{1}{c|}{0.27}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.79}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 \\ \hline
bbc                                & 17          & 18          & \multicolumn{1}{c|}{0.86}        & \multicolumn{1}{c|}{0.26}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.88}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 & \multicolumn{1}{c|}{0.88}        & \multicolumn{1}{c|}{0.26}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{1.00}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 \\ \hline
bbc                                & 18          & 19          & \multicolumn{1}{c|}{0.99}        & \multicolumn{1}{c|}{0.67}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.99}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{0.08}            & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.67}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.69}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{0.08}            & \multicolumn{1}{c|}{\textless{}0.05} & 0.07            \\ \hline
bbc                                & 19          & 20          & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.66}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.99}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{0.11}            & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 & \multicolumn{1}{c|}{0.88}        & \multicolumn{1}{c|}{0.66}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.52}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{0.11}            & \multicolumn{1}{c|}{\textless{}0.05} & -               \\ \hline
bbc                                & 20          & 21          & \multicolumn{1}{c|}{0.99}        & \multicolumn{1}{c|}{0.13}        & \multicolumn{1}{c|}{0.91}        & \multicolumn{1}{c|}{0.70}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & 0.07            & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.13}        & \multicolumn{1}{c|}{0.93}        & \multicolumn{1}{c|}{0.70}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & 0.07            \\ \hline
bbc                                & 21          & 22          & \multicolumn{1}{c|}{0.60}        & \multicolumn{1}{c|}{0.20}        & \multicolumn{1}{c|}{0.88}        & \multicolumn{1}{c|}{0.73}       & \multicolumn{1}{c|}{0.26}            & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 & \multicolumn{1}{c|}{0.66}        & \multicolumn{1}{c|}{0.20}        & \multicolumn{1}{c|}{0.95}        & \multicolumn{1}{c|}{0.73}       & \multicolumn{1}{c|}{0.12}            & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 \\ \hline
bbc                                & 22          & 24          & \multicolumn{1}{c|}{0.88}        & \multicolumn{1}{c|}{0.39}        & \multicolumn{1}{c|}{0.91}        & \multicolumn{1}{c|}{0.37}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{0.20}            & \multicolumn{1}{c|}{\textless{}0.05} & 0.25            & \multicolumn{1}{c|}{0.88}        & \multicolumn{1}{c|}{0.39}        & \multicolumn{1}{c|}{0.94}        & \multicolumn{1}{c|}{0.38}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{0.20}            & \multicolumn{1}{c|}{\textless{}0.05} & 0.27            \\ \hline
bbc                                & 24          & 25          & \multicolumn{1}{c|}{0.71}        & \multicolumn{1}{c|}{0.06}        & \multicolumn{1}{c|}{0.83}        & \multicolumn{1}{c|}{0.68}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & 0.09            & \multicolumn{1}{c|}{0.64}        & \multicolumn{1}{c|}{0.06}        & \multicolumn{1}{c|}{0.82}        & \multicolumn{1}{c|}{0.67}       & \multicolumn{1}{c|}{0.11}            & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & 0.10            \\ \hline
bbc                                & 25          & 26          & \multicolumn{1}{c|}{0.66}        & \multicolumn{1}{c|}{0.36}        & \multicolumn{1}{c|}{0.99}        & \multicolumn{1}{c|}{0.86}       & \multicolumn{1}{c|}{0.19}            & \multicolumn{1}{c|}{0.10}            & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 & \multicolumn{1}{c|}{0.67}        & \multicolumn{1}{c|}{0.36}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.80}       & \multicolumn{1}{c|}{0.17}            & \multicolumn{1}{c|}{0.10}            & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 \\ \hline
citymapper                         & 91          & 92          & \multicolumn{1}{c|}{0.81}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.91}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 & \multicolumn{1}{c|}{0.86}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.85}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 \\ \hline
citymapper                         & 92          & 93          & \multicolumn{1}{c|}{0.97}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.77}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 & \multicolumn{1}{c|}{0.85}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.62}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & 0.18            \\ \hline
citymapper                         & 93          & 94          & \multicolumn{1}{c|}{0.84}        & \multicolumn{1}{c|}{0.98}        & \multicolumn{1}{c|}{0.98}        & \multicolumn{1}{c|}{0.26}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 & \multicolumn{1}{c|}{0.94}        & \multicolumn{1}{c|}{0.98}        & \multicolumn{1}{c|}{0.98}        & \multicolumn{1}{c|}{0.17}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 \\ \hline
citymapper                         & 94          & 95          & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.58}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & 0.28            & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.44}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & 0.33            \\ \hline
citymapper                         & 95          & 96          & \multicolumn{1}{c|}{0.94}        & \multicolumn{1}{c|}{0.97}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.51}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & -               & \multicolumn{1}{c|}{0.94}        & \multicolumn{1}{c|}{0.97}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.67}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & 0.10            \\ \hline
citymapper                         & 96          & 97          & \multicolumn{1}{c|}{0.95}        & \multicolumn{1}{c|}{0.97}        & \multicolumn{1}{c|}{0.97}        & \multicolumn{1}{c|}{0.50}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & -               & \multicolumn{1}{c|}{0.96}        & \multicolumn{1}{c|}{0.97}        & \multicolumn{1}{c|}{0.96}        & \multicolumn{1}{c|}{0.60}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & 0.22            \\ \hline
citymapper                         & 97          & 98          & \multicolumn{1}{c|}{0.77}        & \multicolumn{1}{c|}{0.97}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.62}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & 0.15            & \multicolumn{1}{c|}{0.68}        & \multicolumn{1}{c|}{0.97}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.46}       & \multicolumn{1}{c|}{0.13}            & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & -               \\ \hline
citymapper                         & 98          & 99          & \multicolumn{1}{c|}{0.73}        & \multicolumn{1}{c|}{0.76}        & \multicolumn{1}{c|}{0.88}        & \multicolumn{1}{c|}{0.15}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 & \multicolumn{1}{c|}{0.70}        & \multicolumn{1}{c|}{0.76}        & \multicolumn{1}{c|}{0.97}        & \multicolumn{1}{c|}{0.03}       & \multicolumn{1}{c|}{0.06}            & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 \\ \hline
citymapper                         & 99          & 100         & \multicolumn{1}{c|}{0.99}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.36}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & 0.14            & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.42}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & 0.27            \\ \hline
vlc                                & 17          & 18          & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.01}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{1.00}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.01}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{1.00}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 \\ \hline
vlc                                & 18          & 19          & \multicolumn{1}{c|}{0.74}        & \multicolumn{1}{c|}{0.34}        & \multicolumn{1}{c|}{0.76}        & \multicolumn{1}{c|}{0.52}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{0.11}            & \multicolumn{1}{c|}{\textless{}0.05} & -               & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.34}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.93}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{0.11}            & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 \\ \hline
vlc                                & 19          & 22          & \multicolumn{1}{c|}{0.99}        & \multicolumn{1}{c|}{0.15}        & \multicolumn{1}{c|}{0.95}        & \multicolumn{1}{c|}{0.71}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & 0.09            & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.15}        & \multicolumn{1}{c|}{0.98}        & \multicolumn{1}{c|}{0.65}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & 0.18            \\ \hline
vlc                                & 22          & 23          & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.37}        & \multicolumn{1}{c|}{0.91}        & \multicolumn{1}{c|}{0.74}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{0.15}            & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 & \multicolumn{1}{c|}{0.97}        & \multicolumn{1}{c|}{0.37}        & \multicolumn{1}{c|}{0.98}        & \multicolumn{1}{c|}{0.23}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{0.15}            & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 \\ \hline
vlc                                & 23          & 24          & \multicolumn{1}{c|}{0.69}        & \multicolumn{1}{c|}{0.50}        & \multicolumn{1}{c|}{0.75}        & \multicolumn{1}{c|}{0.50}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{-}               & \multicolumn{1}{c|}{\textless{}0.05} & -               & \multicolumn{1}{c|}{0.76}        & \multicolumn{1}{c|}{0.50}        & \multicolumn{1}{c|}{0.77}        & \multicolumn{1}{c|}{0.10}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{-}               & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 \\ \hline
vlc                                & 24          & 25          & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.45}        & \multicolumn{1}{c|}{0.91}        & \multicolumn{1}{c|}{0.62}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{-}               & \multicolumn{1}{c|}{\textless{}0.05} & 0.18            & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.45}        & \multicolumn{1}{c|}{0.96}        & \multicolumn{1}{c|}{0.40}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{-}               & \multicolumn{1}{c|}{\textless{}0.05} & 0.22            \\ \hline
vlc                                & 25          & 26          & \multicolumn{1}{c|}{0.88}        & \multicolumn{1}{c|}{0.58}        & \multicolumn{1}{c|}{0.84}        & \multicolumn{1}{c|}{0.98}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{0.25}            & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.58}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.87}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{0.25}            & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 \\ \hline
vlc                                & 26          & 27          & \multicolumn{1}{c|}{0.80}        & \multicolumn{1}{c|}{0.00}        & \multicolumn{1}{c|}{0.44}        & \multicolumn{1}{c|}{0.94}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{0.30}            & \textless{}0.05 & \multicolumn{1}{c|}{0.84}        & \multicolumn{1}{c|}{0.00}        & \multicolumn{1}{c|}{0.87}        & \multicolumn{1}{c|}{0.21}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 \\ \hline
wikipedia                          & 15          & 16          & \multicolumn{1}{c|}{0.95}        & \multicolumn{1}{c|}{0.21}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{1.00}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.21}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{1.00}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 \\ \hline
wikipedia                          & 16          & 17          & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.11}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{1.00}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.11}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{1.00}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 \\ \hline
wikipedia                          & 17          & 18          & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{1.00}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{1.00}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 \\ \hline
wikipedia                          & 18          & 19          & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.58}        & \multicolumn{1}{c|}{0.96}        & \multicolumn{1}{c|}{0.96}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{0.27}            & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.58}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.96}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{0.27}            & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 \\ \hline
wikipedia                          & 19          & 20          & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.96}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.88}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.96}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{1.00}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 \\ \hline
yahooweather                       & \textbf{10} & 11          & \multicolumn{1}{c|}{0.50}        & \multicolumn{1}{c|}{0.60}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{1.00}       & \multicolumn{1}{c|}{-}               & \multicolumn{1}{c|}{0.07}            & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 & \multicolumn{1}{c|}{0.90}        & \multicolumn{1}{c|}{0.60}        & \multicolumn{1}{c|}{0.99}        & \multicolumn{1}{c|}{1.00}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{0.07}            & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 \\ \hline
yahooweather                       & 11          & 12          & \multicolumn{1}{c|}{0.50}        & \multicolumn{1}{c|}{0.65}        & \multicolumn{1}{c|}{0.65}        & \multicolumn{1}{c|}{1.00}       & \multicolumn{1}{c|}{-}               & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 & \multicolumn{1}{c|}{0.50}        & \multicolumn{1}{c|}{0.65}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{1.00}       & \multicolumn{1}{c|}{-}               & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 \\ \hline
yahooweather                       & 12          & 13          & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.87}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.70}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & 0.06            & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.87}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.80}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 \\ \hline
yahooweather                       & 13          & 15          & \multicolumn{1}{c|}{0.56}        & \multicolumn{1}{c|}{0.55}        & \multicolumn{1}{c|}{0.55}        & \multicolumn{1}{c|}{0.20}       & \multicolumn{1}{c|}{-}               & \multicolumn{1}{c|}{-}               & \multicolumn{1}{c|}{-}               & \textless{}0.05 & \multicolumn{1}{c|}{0.80}        & \multicolumn{1}{c|}{0.55}        & \multicolumn{1}{c|}{0.96}        & \multicolumn{1}{c|}{0.09}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{-}               & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 \\ \hline
yahooweather                       & 15          & 16          & \multicolumn{1}{c|}{0.96}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.50}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & -               & \multicolumn{1}{c|}{0.91}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.50}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & -               \\ \hline
yahooweather                       & 16          & 17          & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.00}        & \multicolumn{1}{c|}{0.63}        & \multicolumn{1}{c|}{1.00}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{0.16}            & \textless{}0.05 & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.00}        & \multicolumn{1}{c|}{0.75}        & \multicolumn{1}{c|}{1.00}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 \\ \hline
yahooweather                       & 17          & 18          & \multicolumn{1}{c|}{0.95}        & \multicolumn{1}{c|}{0.09}        & \multicolumn{1}{c|}{0.63}        & \multicolumn{1}{c|}{0.96}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{0.17}            & \textless{}0.05 & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.09}        & \multicolumn{1}{c|}{0.85}        & \multicolumn{1}{c|}{1.00}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 \\ \hline
yahooweather                       & 18          & 19          & \multicolumn{1}{c|}{0.80}        & \multicolumn{1}{c|}{0.80}        & \multicolumn{1}{c|}{0.88}        & \multicolumn{1}{c|}{0.63}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 & \multicolumn{1}{c|}{1.00}        & \multicolumn{1}{c|}{0.80}        & \multicolumn{1}{c|}{0.93}        & \multicolumn{1}{c|}{0.53}       & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & -               \\ \hline
yahooweather                       & 19          & 20          & \multicolumn{1}{c|}{0.50}        & \multicolumn{1}{c|}{0.00}        & \multicolumn{1}{c|}{0.15}        & \multicolumn{1}{c|}{0.10}       & \multicolumn{1}{c|}{-}               & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{\textless{}0.05} & \textless{}0.05 & \multicolumn{1}{c|}{0.60}        & \multicolumn{1}{c|}{0.00}        & \multicolumn{1}{c|}{0.58}        & \multicolumn{1}{c|}{0.00}       & \multicolumn{1}{c|}{0.14}            & \multicolumn{1}{c|}{\textless{}0.05} & \multicolumn{1}{c|}{0.26}            & \textless{}0.05 \\ \hline
\end{tabular}

\textbf{Legend}: Compared with \emph{AT}, ATUA. \emph{AP}, APE, \emph{AU}, APE-U , \emph{M}, Monkey. For cases in that CALM and the compared tool perform the same (i.e., \(0.44 < A_{12} < 0.56\)), we ignore the p-value.
\caption{Statistical significance and effect size for RQ1}
\end{table*}

==> tables/RQ1_mannwhitney.tex <==
\begin{table}[]
\caption{Statistics signification for RQ1}
\label{table:RQ1:mannwhitney}
\begin{tabular}{|l|l|l|l|l|}
\hline
\textbf{App}  & \textbf{V1} & \textbf{V2} & \textbf{p\_value\_M} & \textbf{p\_value\_I} \\ \hline
activitydiary & 105         & 111         & 0.338                & 0.141                \\ \hline
activitydiary & 111         & 115         & 0.259                & 0.259                \\ \hline
activitydiary & 115         & 118         & 0.035                & 0.057                \\ \hline
activitydiary & 118         & 122         & 0.117                & 0.084                \\ \hline
activitydiary & 122         & 125         & 0.134                & 0.040                \\ \hline
activitydiary & 125         & 130         & 0.037                & 0.047                \\ \hline
activitydiary & 130         & 131         & 0.000                & 0.000                \\ \hline
activitydiary & 131         & 134         & 0.019                & 0.014                \\ \hline
amazefile     & 11          & 12          & 0.032                & 0.022                \\ \hline
amazefile     & 12          & 16          & 0.253                & 0.354                \\ \hline
amazefile     & 16          & 17          & 0.339                & 0.005                \\ \hline
amazefile     & 17          & 18          & 0.186                & 0.209                \\ \hline
amazefile     & 18          & 20          & 0.000                & 0.000                \\ \hline
bbc           & 16          & 17          & 0.301                & 0.431                \\ \hline
bbc           & 17          & 18          & 0.326                & 0.465                \\ \hline
bbc           & 18          & 19          & 0.142                & 0.114                \\ \hline
bbc           & 19          & 20          & 0.378                & 0.037                \\ \hline
bbc           & 20          & 21          & 0.343                & 0.343                \\ \hline
bbc           & 21          & 22          & 0.091                & 0.149                \\ \hline
bbc           & 22          & 24          & 0.422                & 0.435                \\ \hline
bbc           & 24          & 25          & 0.003                & 0.007                \\ \hline
bbc           & 25          & 26          & 0.318                & 0.461                \\ \hline
citymapper    & 91          & 92          & 0.394                & 0.477                \\ \hline
citymapper    & 92          & 93          & 0.464                & 0.375                \\ \hline
citymapper    & 93          & 94          & 0.151                & 0.343                \\ \hline
citymapper    & 94          & 95          & 0.055                & 0.074                \\ \hline
citymapper    & 95          & 96          & 0.177                & 0.322                \\ \hline
citymapper    & 96          & 97          & 0.021                & 0.013                \\ \hline
citymapper    & 97          & 98          & 0.147                & 0.102                \\ \hline
citymapper    & 98          & 99          & 0.262                & 0.341                \\ \hline
citymapper    & 99          & 100         & 0.117                & 0.146                \\ \hline
wikipedia     & 10          & 11          & 0.339                & 0.418                \\ \hline
wikipedia     & 11          & 12          & 0.158                & 0.429                \\ \hline
wikipedia     & 12          & 13          & 0.087                & 0.217                \\ \hline
wikipedia     & 13          & 15          & 0.221                & 0.370                \\ \hline
wikipedia     & 15          & 16          & 0.056                & 0.065                \\ \hline
wikipedia     & 16          & 17          & 0.163                & 0.193                \\ \hline
wikipedia     & 17          & 18          & 0.017                & 0.039                \\ \hline
wikipedia     & 18          & 19          & 0.333                & 0.400                \\ \hline
wikipedia     & 19          & 20          & 0.006                & 0.002                \\ \hline
\end{tabular}
\end{table}

==> tables/RQ1_meanByApp_updatedMethods.tex <==
\begin{table}[h]
\label{table:RQ1:meanByApp}
\caption{Average percentage of covered updated methods and their instructions across Apps}
\begin{tabular}{l|l l l l l}
\hline
\textbf{App}  & \textbf{ATUA} & \textbf{CALM} & \textbf{APE} & \textbf{APE-U} & \textbf{Monkey} \\ \hline
activitydiary & 87.74         & 90.02         & 91.72        & 89.01          & 77.28           \\ \hline
amazefile     & 53.10         & 56.93         & 59.99        & 55.40          & 42.68           \\ \hline
bbc           & 58.06         & 62.53         & 67.08        & 54.38          & 58.88           \\ \hline
citymapper    & 46.05         & 56.69         & 29.96        & 29.32          & 50.67           \\ \hline
vlc           & 63.91         & 71.53         & 76.35        & 68.85          & 68.63           \\ \hline
wikipedia     & 53.69         & 67.96         & 71.16        & 59.43          & 60.50           \\ \hline
yahooweather  & 61.26         & 65.08         & 63.71        & 61.41          & 55.43           \\ \hline \hline
             \textbf{Average} & \textbf{61.19}         & \textbf{67.94}         & \textbf{65.29}        & \textbf{59.16}          & \textbf{60.6}            \\ \hline
\end{tabular}
\end{table}

==> tables/RQ2.tex <==
% !TEX root =  ../MAIN.tex

\begin{table}[tb]
\footnotesize
\begin{tabular}{|p{2cm}|p{3cm}|}
\hline
\textbf{Case}&\multicolumn{1}{|c|}{\textbf{Effort Reduction (avg/min/max)}}\\
\textbf{study}&\multicolumn{1}{|c|}{\textbf{wrt DM2}}\\
\hline
\input{data/RQ2_1Hour_COMPARISON_instructions_coverage_over_lifecycle_DELTA.tex}
\hline
\input{data/RQ2_5Hours_COMPARISON_instructions_coverage_over_lifecycle_DELTA.tex}
\hline
\end{tabular}
\caption{Effort reduction with respect to other approaches. Top part shows results with budget of one hour, bottom part shows results for five hours.}
\label{table:RQ2}
\end{table}%


==> tables/RQ2_input.tex <==
\begin{table*}[tb]
\caption{Input data for RQ2}
\label{table:RQ2:input}
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|}
\hline
\textbf{App}  & \textbf{V1} & \textbf{V2} & \textbf{AM\%} & \textbf{CM\%} & \textbf{AW\%} & \textbf{DW\%} & \textbf{CW\%} & \textbf{Aw\%} & \textbf{Dw\%} & \textbf{Cw\%} \\ \hline
activitydiary                          & 105                                   & 111                                   & 3.00                                    & 2.40                                    & 0.00                                    & 0.00                                    & 0.00                           & 0.25                           & 7.48                           & 77.81                          \\ \hline
activitydiary                          & 111                                   & 115                                   & 0.00                                    & 0.90                                    & 0.00                                    & 0.00                                    & 0.00                           & 3.13                           & 3.13                           & 61.10                          \\ \hline
activitydiary                          & 115                                   & 118                                   & 0.90                                    & 4.80                                    & 0.00                                    & 0.00                                    & 0.00                           & 1.59                           & 4.77                           & 65.25                          \\ \hline
activitydiary                          & 118                                   & 122                                   & 4.67                                    & 22.00                                   & 26.67                                   & 0.00                                    & 0.00                           & 39.97                          & 1.94                           & 45.63                          \\ \hline
activitydiary                          & 122                                   & 125                                   & 2.51                                    & 6.05                                    & 0.00                                    & 0.00                                    & 0.00                           & 0.17                           & 0.00                           & 49.92                          \\ \hline
activitydiary                          & 125                                   & 130                                   & 0.93                                    & 4.81                                    & 11.76                                   & 0.00                                    & 0.00                           & 33.75                          & 1.57                           & 41.39                          \\ \hline
activitydiary                          & 130                                   & 131                                   & 0.00                                    & 0.19                                    & 0.00                                    & 0.00                                    & 0.00                           & 1.93                           & 1.93                           & 52.41                          \\ \hline
activitydiary                          & 131                                   & 134                                   & 1.67                                    & 6.22                                    & 5.56                                    & 0.00                                    & 0.00                           & 6.52                           & 7.34                           & 65.14                          \\ \hline
amazefile                              & 11                                    & 12                                    & 6.10                                    & 8.30                                    & 0.00                                    & 0.00                                    & 0.00                           & 19.38                          & 5.54                           & 46.15                          \\ \hline
amazefile                              & 12                                    & 16                                    & 2.95                                    & 4.21                                    & 18.18                                   & 9.09                                    & 36.36                          & 27.21                          & 15.35                          & 45.35                          \\ \hline
amazefile                              & 16                                    & 17                                    & 0.15                                    & 0.20                                    & 0.00                                    & 0.00                                    & 0.00                           & 1.39                           & 1.39                           & 59.33                          \\ \hline
amazefile                              & 17                                    & 18                                    & 2.47                                    & 15.41                                   & 9.09                                    & 0.00                                    & 9.09                           & 10.61                          & 17.17                          & 44.70                          \\ \hline
amazefile                              & 18                                    & 20                                    & 0.00                                    & 0.05                                    & 0.00                                    & 0.00                                    & 0.00                           & 1.50                           & 1.50                           & 54.79                          \\ \hline
bbc                                    & 16                                    & 17                                    & 4.13                                    & 3.39                                    & 8.33                                    & 33.33                                   & 0.00                           & 27.17                          & 56.07                          & 1.16                           \\ \hline
bbc                                    & 17                                    & 18                                    & 0.17                                    & 0.14                                    & 0.00                                    & 0.00                                    & 0.00                           & 21.65                          & 21.65                          & 11.34                          \\ \hline
bbc                                    & 18                                    & 19                                    & 0.28                                    & 0.22                                    & 0.00                                    & 0.00                                    & 0.00                           & 33.33                          & 33.33                          & 4.39                           \\ \hline
bbc                                    & 19                                    & 20                                    & 0.19                                    & 0.09                                    & 4.00                                    & 0.00                                    & 0.00                           & 34.48                          & 32.76                          & 5.17                           \\ \hline
bbc                                    & 20                                    & 21                                    & 3.62                                    & 2.48                                    & 13.79                                   & 13.79                                   & 0.00                           & 36.07                          & 39.34                          & 2.46                           \\ \hline
bbc                                    & 21                                    & 22                                    & 0.96                                    & 1.38                                    & 0.00                                    & 0.00                                    & 0.00                           & 33.93                          & 33.93                          & 3.57                           \\ \hline
bbc                                    & 22                                    & 24                                    & 1.30                                    & 3.87                                    & 13.79                                   & 0.00                                    & 0.00                           & 39.84                          & 31.71                          & 3.25                           \\ \hline
bbc                                    & 24                                    & 25                                    & 0.56                                    & 0.20                                    & 0.00                                    & 10.34                                   & 0.00                           & 30.58                          & 35.54                          & 2.48                           \\ \hline
bbc                                    & 25                                    & 26                                    & 0.57                                    & 0.50                                    & 0.00                                    & 7.69                                    & 0.00                           & 32.76                          & 34.48                          & 4.31                           \\ \hline
citymapper                             & 91                                    & 92                                    & 0.27                                    & 0.26                                    & 0.00                                    & 1.39                                    & 0.00                           & 4.61                           & 4.61                           & 19.74                          \\ \hline
citymapper                             & 92                                    & 93                                    & 0.23                                    & 0.16                                    & 0.00                                    & 0.00                                    & 0.00                           & 5.23                           & 5.23                           & 24.18                          \\ \hline
citymapper                             & 93                                    & 94                                    & 0.40                                    & 0.18                                    & 0.00                                    & 7.04                                    & 0.00                           & 5.23                           & 5.88                           & 22.22                          \\ \hline
citymapper                             & 94                                    & 95                                    & 0.53                                    & 0.23                                    & 0.00                                    & 0.00                                    & 0.00                           & 4.00                           & 4.00                           & 21.33                          \\ \hline
citymapper                             & 95                                    & 96                                    & 0.62                                    & 0.60                                    & 0.00                                    & 0.00                                    & 0.00                           & 5.26                           & 5.26                           & 23.68                          \\ \hline
citymapper                             & 96                                    & 97                                    & 0.51                                    & 0.26                                    & 1.49                                    & 0.00                                    & 0.00                           & 4.00                           & 4.00                           & 20.00                          \\ \hline
citymapper                             & 97                                    & 98                                    & 0.53                                    & 0.20                                    & 0.00                                    & 0.00                                    & 0.00                           & 3.36                           & 3.36                           & 15.44                          \\ \hline
citymapper                             & 98                                    & 99                                    & 0.04                                    & 0.08                                    & 0.00                                    & 0.00                                    & 0.00                           & 4.00                           & 4.00                           & 21.33                          \\ \hline
citymapper                             & 99                                    & 100                                   & 0.55                                    & 0.14                                    & 1.47                                    & 2.94                                    & 0.00                           & 6.49                           & 6.49                           & 22.73                          \\ \hline
wikipedia                              & 10                                    & 11                                    & 4.83                                    & 4.15                                    & 6.90                                    & 13.79                                   & 13.79                          & 26.90                          & 23.43                          & 23.27                          \\ \hline
wikipedia                              & 11                                    & 12                                    & 1.91                                    & 1.63                                    & 0.00                                    & 8.00                                    & 8.00                           & 12.95                          & 35.46                          & 19.89                          \\ \hline
wikipedia                              & 12                                    & 13                                    & 0.82                                    & 0.87                                    & 8.00                                    & 4.00                                    & 4.00                           & 31.88                          & 29.11                          & 11.29                          \\ \hline
wikipedia                              & 13                                    & 15                                    & 2.94                                    & 2.43                                    & 17.24                                   & 0.00                                    & 20.69                          & 33.70                          & 29.81                          & 14.07                          \\ \hline
wikipedia                              & 15                                    & 16                                    & 2.10                                    & 1.85                                    & 6.45                                    & 0.00                                    & 9.68                           & 27.34                          & 9.56                           & 34.03                          \\ \hline
wikipedia                              & 16                                    & 17                                    & 5.99                                    & 10.36                                   & 31.11                                   & 6.67                                    & 8.89                           & 59.64                          & 9.13                           & 25.26                          \\ \hline
wikipedia                              & 17                                    & 18                                    & 2.21                                    & 3.93                                    & 10.64                                   & 4.26                                    & 6.38                           & 48.95                          & 24.07                          & 19.32                          \\ \hline
wikipedia                              & 18                                    & 19                                    & 0.00                                    & 0.15                                    & 0.00                                    & 0.00                                    & 2.22                           & 18.01                          & 17.91                          & 36.18                          \\ \hline
wikipedia                              & 19                                    & 20                                    & 0.31                                    & 0.76                                    & 0.00                                    & 0.00                                    & 2.22                           & 10.41                          & 10.24                          & 44.85                          \\ \hline
\end{tabular}

\footnotesize{\textbf{Legend:} AM\%: Added methods, CM\%: Changed methods, AW\%: Added windows, DW\%: Deleted windows, CW\%: Changed windows, Aw\%: Added widgets, Dw\%: Deleted widgets, Cw\%: Changed widgets }
\end{table*}

==> tables/RQ2_predictionResult.tex <==
% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
\begin{table}[]
\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
\textbf{App}  & \textbf{V1} & \textbf{V2} & \textbf{Y\_1}             & \textbf{P\_1}             & \textbf{Y\_2}             & \textbf{P\_2}             \\ \hline
activitydiary & 105         & 111         & 0                         & 0                         & \cellcolor[HTML]{FFF046}1 & \cellcolor[HTML]{FFF046}0 \\ \hline
activitydiary & 111         & 115         & \cellcolor[HTML]{FFF046}1 & \cellcolor[HTML]{FFF046}0 & \cellcolor[HTML]{FFF046}1 & \cellcolor[HTML]{FFF046}0 \\ \hline
activitydiary & 115         & 118         & 0                         & 0                         & 0                         & 0                         \\ \hline
activitydiary & 118         & 122         & 0                         & 0                         & 0                         & 0                         \\ \hline
activitydiary & 122         & 125         & 0                         & 0                         & 0                         & 0                         \\ \hline
activitydiary & 125         & 130         & 0                         & 0                         & 0                         & 0                         \\ \hline
activitydiary & 130         & 131         & 0                         & 0                         & 0                         & 0                         \\ \hline
activitydiary & 131         & 134         & 0                         & 0                         & 0                         & 0                         \\ \hline
amazefile     & 11          & 12          & 0                         & 0                         & 0                         & 0                         \\ \hline
amazefile     & 12          & 16          & 0                         & 0                         & 0                         & 0                         \\ \hline
amazefile     & 16          & 17          & 0                         & 0                         & \cellcolor[HTML]{FFF046}1 & \cellcolor[HTML]{FFF046}0 \\ \hline
amazefile     & 17          & 18          & 0                         & 0                         & 0                         & 0                         \\ \hline
amazefile     & 18          & 20          & 0                         & 0                         & 0                         & 0                         \\ \hline
bbc           & 16          & 17          & 0                         & 0                         & \cellcolor[HTML]{7BFF3E}0 & \cellcolor[HTML]{7BFF3E}1 \\ \hline
bbc           & 17          & 18          & \cellcolor[HTML]{7BFF3E}0 & \cellcolor[HTML]{7BFF3E}1 & 0                         & 0                         \\ \hline
bbc           & 18          & 19          & \cellcolor[HTML]{7BFF3E}0 & \cellcolor[HTML]{7BFF3E}1 & \cellcolor[HTML]{7BFF3E}0 & \cellcolor[HTML]{7BFF3E}1 \\ \hline
bbc           & 19          & 20          & 1                         & 1                         & 1                         & 1                         \\ \hline
bbc           & 20          & 21          & \cellcolor[HTML]{FFF046}1 & \cellcolor[HTML]{FFF046}0 & \cellcolor[HTML]{FFF046}1 & \cellcolor[HTML]{FFF046}0 \\ \hline
bbc           & 21          & 22          & 1                         & 1                         & 1                         & 1                         \\ \hline
bbc           & 22          & 24          & \cellcolor[HTML]{7BFF3E}0 & \cellcolor[HTML]{7BFF3E}1 & 0                         & 0                         \\ \hline
bbc           & 24          & 25          & 1                         & 1                         & 1                         & 1                         \\ \hline
bbc           & 25          & 26          & 1                         & 1                         & 1                         & 1                         \\ \hline
citymapper    & 91          & 92          & 0                         & 0                         & 0                         & 0                         \\ \hline
citymapper    & 92          & 93          & 0                         & 0                         & 0                         & 0                         \\ \hline
citymapper    & 93          & 94          & 0                         & 0                         & 0                         & 0                         \\ \hline
citymapper    & 94          & 95          & 0                         & 0                         & 0                         & 0                         \\ \hline
citymapper    & 95          & 96          & \cellcolor[HTML]{FFF046}1 & \cellcolor[HTML]{FFF046}0 & 0                         & 0                         \\ \hline
citymapper    & 96          & 97          & 0                         & 0                         & 0                         & 0                         \\ \hline
citymapper    & 97          & 98          & 0                         & 0                         & 0                         & 0                         \\ \hline
citymapper    & 98          & 99          & \cellcolor[HTML]{FFF046}1 & \cellcolor[HTML]{FFF046}0 & 0                         & 0                         \\ \hline
citymapper    & 99          & 100         & 0                         & 0                         & 0                         & 0                         \\ \hline
wikipedia     & 10          & 11          & 0                         & 0                         & 0                         & 0                         \\ \hline
wikipedia     & 11          & 12          & 0                         & 0                         & 0                         & 0                         \\ \hline
wikipedia     & 12          & 13          & 1                         & 1                         & \cellcolor[HTML]{FFF046}1 & \cellcolor[HTML]{FFF046}0 \\ \hline
wikipedia     & 13          & 15          & \cellcolor[HTML]{FFF046}1 & \cellcolor[HTML]{FFF046}0 & 0                         & 0                         \\ \hline
wikipedia     & 15          & 16          & 0                         & 0                         & 0                         & 0                         \\ \hline
wikipedia     & 16          & 17          & 0                         & 0                         & 0                         & 0                         \\ \hline
wikipedia     & 17          & 18          & 0                         & 0                         & 0                         & 0                         \\ \hline
wikipedia     & 18          & 19          & 0                         & 0                         & 0                         & 0                         \\ \hline
wikipedia     & 19          & 20          & 0                         & 0                         & 0                         & 0                         \\ \hline
\end{tabular}
\end{table}

==> tables/RQ2_score.tex <==
\begin{table*}[tb]
\caption{Logistic Regression Model score in predicting success of CALM}
\label{table:RQ2:score}
\begin{tabular}{|l|llll|llll|}
\hline
      & \multicolumn{4}{l|}{Success in coverage of target methods}                                              & \multicolumn{4}{l|}{Success in coverage of target instructions}                                \\ \hline
      & \multicolumn{1}{l|}{Precision} & \multicolumn{1}{l|}{Recall} & \multicolumn{1}{l|}{F1-score} & Support & \multicolumn{1}{l|}{Precision} & \multicolumn{1}{l|}{Recall} & \multicolumn{1}{l|}{F1-score} & Support \\ \hline
\ATUA performs better  & \multicolumn{1}{l|}{0.84}      & \multicolumn{1}{l|}{0.90}   & \multicolumn{1}{l|}{0.87}     & 30      & \multicolumn{1}{l|}{0.85}      & \multicolumn{1}{l|}{0.94}   & \multicolumn{1}{l|}{0.89}     & 31      \\ \hline
\APPR performs better & \multicolumn{1}{l|}{0.62}      & \multicolumn{1}{l|}{0.50}   & \multicolumn{1}{l|}{0.56}     & 10      & \multicolumn{1}{l|}{0.67}      & \multicolumn{1}{l|}{0.44}   & \multicolumn{1}{l|}{0.53}     & 9       \\ \hline
Accuracy   & \multicolumn{1}{l|}{}          & \multicolumn{1}{l|}{}       & \multicolumn{1}{l|}{0.8}      & 40      & \multicolumn{1}{l|}{}          & \multicolumn{1}{l|}{}       & \multicolumn{1}{l|}{0.82}     & 40      \\ \hline
\end{tabular}
\end{table*}

==> tables/Result_Real_5n10_Anomaly_groups.tex <==


\begin{table}[h]
\caption{Results for the real datasets}
\label{Table:result:real}
\centering
\tiny
\begin{tabular}{lccccc|ccccc}
\hline \hline
\multicolumn{6}{c|}{\textbf{Without Pruning}}                                                                                             & \multicolumn{5}{c}{\textbf{With Pruning}}                                                        \\ \hline \hline
\multicolumn{1}{c}{\textbf{Algorithm}} & \textbf{SC} & \textbf{Prec.}      & \textbf{Rec.}       & \textbf{F1}         & \textbf{DC}   & \textbf{SC} & \textbf{Prec.}      & \textbf{Rec.}       & \textbf{F1}         & \textbf{DC}    \\ \hline
\multicolumn{1}{l|}{SIF}               & 20          & \textbf{0.32}       & \ul{ 1.00}          & \ul{ 0.48}          & \textbf{9.99}    & 20          & \textbf{0.42}       & \ul{ 1.00}          & \ul{ 0.59}          & \textbf{14.49}   \\ \hline
\multicolumn{1}{l|}{SIF}               & 20          & 0.32                & \ul{ \textbf{1.00}} & \ul{ 0.48}          & \textbf{9.99}    & 20          & 0.42                & \ul{ \textbf{1.00}} & \ul{ 0.59}          & \textbf{14.49}   \\ \hline
\multicolumn{1}{l|}{SIF}               & 20          & 0.32                & \ul{ 1.00}          & \ul{ \textbf{0.48}} & \textbf{9.99}    & 20          & 0.42                & \ul{ 1.00}          & \ul{ \textbf{0.59}} & \textbf{14.49}   \\ \hline
\multicolumn{1}{l|}{IF}                & N/A         & \textbf{0.00}       & 0.34                & 0.01                & N/A              & N/A         & \ul{ \textbf{0.59}} & 0.97                & 0.73                & N/A              \\ \hline
\multicolumn{1}{l|}{SHAC}              & 1           & \ul{ \textbf{0.38}} & 0.50                & 0.43                & 10.40            & 20          & \textbf{0.42}       & \ul{ 1.00}          & \ul{ 0.59}          & 15.00            \\ \hline
\multicolumn{1}{l|}{SHAC}              & 20          & 0.32                & \ul{ \textbf{1.00}} & \ul{ 0.48}          & 10.40            & 20          & 0.42                & \ul{ \textbf{1.00}} & \ul{ 0.59}          & 15.00            \\ \hline
\multicolumn{1}{l|}{SHAC}              & 20          & 0.32                & \ul{ 1.00}          & \ul{ \textbf{0.48}} & 10.40            & 20          & 0.42                & \ul{ 1.00}          & \ul{ \textbf{0.59}} & 15.00            \\ \hline
\multicolumn{1}{l|}{SKM}               & 1           & \textbf{0.34}       & 0.45                & 0.39                & 10.01            & 20          & \textbf{0.42}       & \ul{ 1.00}          & \ul{ 0.59}          & 15.12            \\ \hline
\multicolumn{1}{l|}{SKM}               & 20          & 0.32                & \ul{ \textbf{1.00}} & \ul{ 0.48}          & 10.01            & 20          & 0.42                & \ul{ \textbf{1.00}} & \ul{ 0.59}          & 15.12            \\ \hline
\multicolumn{1}{l|}{SKM}               & 20          & 0.32                & \ul{ 1.00}          & \ul{ \textbf{0.48}} & 10.01            & 20          & 0.42                & \ul{ 1.00}          & \ul{ \textbf{0.59}} & 15.12            \\ \hline
\multicolumn{1}{l|}{LOF-10}            & N/A         & \textbf{0.32}       & \textbf{0.67}       & \textbf{0.43}       & N/A              & N/A         & \textbf{0.00}       & \textbf{0.00}       & \textbf{0.00}       & N/A              \\ \hline
\multicolumn{1}{l|}{LOF-15}            & N/A         & \textbf{0.32}       & \textbf{0.67}       & \textbf{0.43}       & N/A              & N/A         & \textbf{0.00}       & \textbf{0.00}       & \textbf{0.00}       & N/A              \\ \hline
\multicolumn{1}{l|}{LOF-20}            & N/A         & \textbf{0.32}       & \textbf{0.67}       & \textbf{0.43}       & N/A              & N/A         & \textbf{0.00}       & \textbf{0.00}       & \textbf{0.00}       & N/A              \\ \hline
\multicolumn{1}{l|}{LOF-25}            & N/A         & \textbf{0.32}       & \textbf{0.67}       & \textbf{0.43}       & N/A              & N/A         & \textbf{0.00}       & \textbf{0.00}       & \textbf{0.00}       & N/A              \\ \hline
\multicolumn{1}{l|}{SKNN-10}           & 20          & \textbf{0.32}       & \ul{ 1.00}          & \ul{ 0.48}          & 11.25            & 20          & \textbf{0.42}       & \ul{ 1.00}          & \ul{ 0.59}          & 17.50            \\ \hline
\multicolumn{1}{l|}{SKNN-10}           & 20          & 0.32                & \ul{ \textbf{1.00}} & \ul{ 0.48}          & 11.25            & 20          & 0.42                & \ul{ \textbf{1.00}} & \ul{ 0.59}          & 17.50            \\ \hline
\multicolumn{1}{l|}{SKNN-10}           & 20          & 0.32                & \ul{ 1.00}          & \ul{ \textbf{0.48}} & 11.25            & 20          & 0.42                & \ul{ 1.00}          & \ul{ \textbf{0.59}} & 17.50            \\ \hline
\multicolumn{1}{l|}{SKNN-15}           & 20          & \textbf{0.32}       & \ul{ 1.00}          & \ul{ 0.48}          & 10.85            & 20          & \textbf{0.42}       & \ul{ 1.00}          & \ul{ 0.59}          & 15.50            \\ \hline
\multicolumn{1}{l|}{SKNN-15}           & 20          & 0.32                & \ul{ \textbf{1.00}} & \ul{ 0.48}          & 10.85            & 20          & 0.42                & \ul{ \textbf{1.00}} & \ul{ 0.59}          & 15.50            \\ \hline
\multicolumn{1}{l|}{SKNN-15}           & 20          & 0.32                & \ul{ 1.00}          & \ul{ \textbf{0.48}} & 10.85            & 20          & 0.42                & \ul{ 1.00}          & \ul{ \textbf{0.59}} & 15.50            \\ \hline
\multicolumn{1}{l|}{SKNN-20}           & 20          & \textbf{0.32}       & \ul{ 1.00}          & \ul{ 0.48}          & 10.85            & 20          & \textbf{0.42}       & \ul{ 1.00}          & \ul{ 0.59}          & 15.50            \\ \hline
\multicolumn{1}{l|}{SKNN-20}           & 20          & 0.32                & \ul{ \textbf{1.00}} & \ul{ 0.48}          & 10.85            & 20          & 0.42                & \ul{ \textbf{1.00}} & \ul{ 0.59}          & 15.50            \\ \hline
\multicolumn{1}{l|}{SKNN-20}           & 20          & 0.32                & \ul{ 1.00}          & \ul{ \textbf{0.48}} & 10.85            & 20          & 0.42                & \ul{ 1.00}          & \ul{ \textbf{0.59}} & 15.50            \\ \hline
\multicolumn{1}{l|}{SKNN-25}           & 20          & \textbf{0.32}       & \ul{ 1.00}          & \ul{ 0.48}          & 10.85            & 20          & \textbf{0.42}       & \ul{ \textbf{1.00}} & \ul{ \textbf{0.59}} & 15.50            \\ \hline
\multicolumn{1}{l|}{SKNN-25}           & 20          & 0.32                & \ul{ \textbf{1.00}} & \ul{ 0.48}          & 10.85            & 20          & 0.42                & \ul{ \textbf{1.00}} & \ul{ 0.59}          & 15.50            \\ \hline
\multicolumn{1}{l|}{SKNN-25}           & 20          & 0.32                & \ul{ 1.00}          & \ul{ \textbf{0.48}} & 10.85            & 20          & 0.42                & \ul{ 1.00}          & \ul{ \textbf{0.59}} & 15.50 

\\ \hline \hline
% \begin{tabular}{lccccclllccccc}
% \hline\hline
% % \cline{1-6} \cline{9-14}
% \multicolumn{6}{c}{\textbf{Real without Pruning}}      &  &  & \multicolumn{6}{c}{\textbf{Real with pruning}}\\ \cline{1-6} \cline{9-14} 
% \multicolumn{1}{c}{\textbf{Algorithm}} & \textbf{SC} & \textbf{Precision} & \textbf{Recall} & \textbf{F1}   & \textbf{DC} &  &  & \multicolumn{1}{c}{\textbf{Algorithm}} & \textbf{SC} & \textbf{Precision} & \textbf{Recall} & \textbf{F1}   & \textbf{DC} \\ \cline{1-6} \cline{9-14} \hline \hline
% SIF& 20 & \textbf{0.32}      & \underline{1.00}   & \underline{0.48} & \textbf {9.99}       &  &  & SIF& 20 & \textbf{0.42}      & \underline{1.00}   & \underline{0.59} & \textbf{14.49}      \\ \cline{1-6} \cline{9-14} 
% SIF& 20 & 0.32      &\textbf{\underline{1.00}}   & \underline{0.48} & \textbf {9.99}       &  &  & SIF& 20 & 0.42      & \underline{\textbf{1.00}}   & \underline{0.59} & \textbf{14.49}      \\ \cline{1-6} \cline{9-14} 
% SIF& 20 & 0.32      & \underline{1.00}   &\textbf{\underline{0.48}} & \textbf {9.99}       &  &  & SIF& 20 & 0.42      & \underline{1.00}   & \underline{\textbf{0.59}} & \textbf{14.49}      \\ \cline{1-6} \cline{9-14} 
% IF    & N/A& \textbf{0.00}      & \textbf{0.34}   & \textbf{0.01} & N/A     &  &  & IF   & N/A& \textbf{\underline{0.59}}      & \textbf{0.97}   & \textbf{0.73} & N/A     \\ \cline{1-6} \cline{9-14} 
% SHAC& 1  & \textbf{\underline{0.38}}      & 0.50   & 0.43 & 10.40   &  &  & SHAC& 20 & \textbf{0.42}      & \underline{1.00}   & \underline{0.59} & 15.00   \\ \cline{1-6} \cline{9-14} 
% SHAC& 20 & 0.32      & \textbf{\underline{1.00}}   & \underline{0.48} & 10.40   &  &  & SHAC& 20 & 0.42      & \underline{\textbf{1.00}}   & \underline{0.59} & 15.00   \\ \cline{1-6} \cline{9-14} 
% SHAC& 20 & 0.32      & \underline{1.00}   &\textbf{\underline{0.48}}& 10.40   &  &  & SHAC& 20 & 0.42      & \underline{1.00}   & \underline{\textbf{0.59}} & 15.00   \\ \cline{1-6} \cline{9-14} 
% SKM& 1  &\textbf{0.34}      & 0.45   & 0.39 & 10.01   &  &  & SKM& 20 & \textbf{0.42}      & \underline{1.00}   & \underline{0.59} & 15.12   \\ \cline{1-6} \cline{9-14} 
% SKM& 20 & 0.32      & \textbf{\underline{1.00}}   & \underline{0.48} & 10.01   &  &  & SKM& 20 & 0.42      & \underline{\textbf{1.00}}   & \underline{0.59} & 15.12   \\ \cline{1-6} \cline{9-14} 
% SKM& 20 & 0.32      & \underline{1.00}   & \textbf{\underline{0.48}} & 10.01   &  &  & SKM& 20 & 0.42      & \underline{1.00}   & \underline{\textbf{0.59}} & 15.12   \\ \cline{1-6} \cline{9-14} 
% LOF-10      & N/A& \textbf{0.32}      & \textbf{0.67}   & \textbf{0.43} & N/A     &  &  & LOF-10      & N/A& \textbf{0.00}      & \textbf{0.00}   & \textbf{0.00} & N/A     \\ \cline{1-6} \cline{9-14} 
% LOF-15      & N/A& \textbf{0.32}      & \textbf{0.67}   & \textbf{0.43} & N/A     &  &  & LOF-15      & N/A& \textbf{0.00}      & \textbf{0.00}   & \textbf{0.00} & N/A     \\ \cline{1-6} \cline{9-14} 
% LOF-20      & N/A& \textbf{0.32}      & \textbf{0.67}   & \textbf{0.43} & N/A     &  &  & LOF-20      & N/A& \textbf{0.00}      & \textbf{0.00}   & \textbf{0.00} & N/A     \\ \cline{1-6} \cline{9-14} 
% LOF-25      & N/A& \textbf{0.32}      & \textbf{0.67}   & \textbf{0.43} & N/A     &  &  & LOF-25      & N/A& \textbf{0.00}      & \textbf{0.00}   & \textbf{0.00} & N/A     \\ \cline{1-6} \cline{9-14} 
% SKNN-10     & 20 &\textbf{0.32}      & \underline{1.00}   & \underline{0.48} & 11.25   &  &  & SKNN-10     & 20 & \textbf{0.42}      & \underline{1.00}   & \underline{0.59} & 17.50   \\ \cline{1-6} \cline{9-14} 
% SKNN-10     & 20 & 0.32      &\textbf{\underline{1.00}}   & \underline{0.48} & 11.25   &  &  & SKNN-10     & 20 & 0.42      & \underline{\textbf{1.00}}   & \underline{0.59} & 17.50   \\ \cline{1-6} \cline{9-14} 
% SKNN-10     & 20 & 0.32      & \underline{1.00}   & \textbf{\underline{0.48}} & 11.25   &  &  & SKNN-10     & 20 & 0.42      & \underline{1.00} & \underline{\textbf{0.59}} & 17.50   \\ \cline{1-6} \cline{9-14} 
% SKNN-15     & 20 & \textbf{0.32}      & \underline{1.00}   & \underline{0.48} & 10.85   &  &  & SKNN-15     & 20 & \textbf{0.42}      & \underline{1.00}   & \underline{0.59} & 15.50   \\ \cline{1-6} \cline{9-14} 
% SKNN-15     & 20 & 0.32      & \textbf{\underline{1.00}}   & \underline{0.48} & 10.85   &  &  & SKNN-15     & 20 & 0.42      & \underline{\textbf{1.00}}   & \underline{0.59} & 15.50   \\ \cline{1-6} \cline{9-14} 
% SKNN-15     & 20 & 0.32      & \underline{1.00}   & \textbf{\underline{0.48}} & 10.85   &  &  & SKNN-15     & 20 & 0.42      & \underline{1.00}   & \underline{\textbf{0.59}} & 15.50   \\ \cline{1-6} \cline{9-14} 
% SKNN-20     & 20 & \textbf{0.32}      &\underline{1.00}   & \underline{0.48} & 10.85   &  &  & SKNN-20     & 20 & \textbf{0.42}      & \underline{1.00}   & \underline{0.59} & 15.50   \\ \cline{1-6} \cline{9-14} 
% SKNN-20     & 20 & 0.32      & \textbf{\underline{1.00}}   & \underline{0.48} & 10.85   &  &  & SKNN-20     & 20 & 0.42      & \textbf{\underline{1.00}}   & \underline{0.59} & 15.50   \\ \cline{1-6} \cline{9-14} 
% SKNN-20     & 20 & 0.32      & \underline{1.00}   & \textbf{\underline{0.48}} & 10.85   &  &  & SKNN-20     & 20 & 0.42      &\underline{1.00}   & \textbf{\underline{0.59}} & 15.50   \\ \cline{1-6} \cline{9-14} 
% SKNN-25     & 20 & \textbf{0.32}      & \underline{1.00}   & \underline{0.48} & 10.85   &  &  & SKNN-25     & 20 & \textbf{0.42}      & \underline{1.00}   & \underline{0.59} & 15.50   \\ \cline{1-6} \cline{9-14} 
% SKNN-25     & 20 & 0.32      & \textbf{\underline{1.00}}   & \underline{0.48} & 10.85   &  &  & SKNN-25     & 20 & 0.42      & \underline{\textbf{1.00}}   & \underline{0.59} & 15.50   \\ \cline{1-6} \cline{9-14} 
% SKNN-25     & 20 & 0.32      & \underline{1.00}   & \textbf{\underline{0.48}} & 10.85   &  &  & SKNN-25     & 20 & 0.42      & \underline{1.00}   & \underline{\textbf{0.59}} & 15.50  





\end{tabular}
\end{table}

==> tables/Result_Realistic_5n10_Anomaly_groups.tex <==

\begin{table*}[]
\caption{Results for Realistic data Filtered and Unfiltered for 5 and 10 Anomaly Groups}
\label{Table:result:realistic:five}
\begin{tabular}{lccccclllccccc}
\hline \hline
\multicolumn{6}{c}{\textbf{Realistic Data Unfiltered}}                                                                                &  &  & \multicolumn{6}{c}{\textbf{Realistic Data Filtered}}                                                                   \\ \cline{1-6} \cline{9-14} 
\multicolumn{1}{c}{\textbf{Algorithm}} & \textbf{SC} & \textbf{Precision} & \textbf{Recall} & \textbf{F1}    & \textbf{Ins@100} &  &  & \multicolumn{1}{c}{\textbf{Algorithm}} & \textbf{SC} & \textbf{Precision} & \textbf{Recall} & \textbf{F1}    & \textbf{Ins@100} \\ \hline \hline


Isolation Forest                       & 1           & \textbf{0.86}      & 0.95            & 0.90          & 8.83             &  &  & Isolation Forest                       & 1           & \textbf{0.87}      & 0.99            & 0.93          & 7.73             \\ \cline{1-6} \cline{9-14} 
Isolation Forest                       & 20          & 0.26               & \textbf{1.00}   & 0.41          & 8.83             &  &  & Isolation Forest                       & 20          & 0.26               & \textbf{1.00}   & 0.42          & 7.73             \\ \cline{1-6} \cline{9-14} 
Isolation Forest                       & 1           & 0.86               & 0.95            & \textbf{0.90} & 8.83             &  &  & Isolation Forest                       & 1           & 0.87               & 0.99            & \textbf{0.93} & 7.73             \\ \cline{1-6} \cline{9-14} 
Isolation Fores-N                      & N/A         & \textbf{0.00}      & 0.00            & 0.00          & N/A              &  &  & Isolation Forest-N                     & N/A         & \textbf{0.00}      & 0.00            & 0.00          & N/A              \\ \cline{1-6} \cline{9-14} 
AG                                     & 1           & \textbf{0.00}      & 0.00            & 0.00          & 262.88           &  &  & AG                                     & 1           & \textbf{0.87}      & 1.00            & 0.93          & 17.25            \\ \cline{1-6} \cline{9-14} 
AG                                     & 1           & 0.00               & \textbf{0.00}   & 0.00          & 262.88           &  &  & AG                                     & 1           & 0.87               & \textbf{1.00}   & 0.93          & 17.25            \\ \cline{1-6} \cline{9-14} 
AG                                     & 1           & 0.00               & 0.00            & \textbf{0.00} & 262.88           &  &  & AG                                     & 1           & 0.87               & 1.00            & \textbf{0.93} & 17.25            \\ \cline{1-6} \cline{9-14} 
k-means                                & 1           & \textbf{0.00}      & 0.00            & 0.00          & 311.44           &  &  & k-means                                & 1           & \textbf{0.87}      & 0.98            & 0.92          & 27.80            \\ \cline{1-6} \cline{9-14} 
k-means                                & 1           & 0.00               & \textbf{0.00}   & 0.00          & 311.44           &  &  & k-means                                & 1           & 0.87               & \textbf{0.98}   & 0.92          & 27.80            \\ \cline{1-6} \cline{9-14} 
k-means                                & 1           & 0.00               & 0.00            & \textbf{0.00} & 311.44           &  &  & k-means                                & 1           & 0.87               & 0.98            & \textbf{0.92} & 27.80            \\ \cline{1-6} \cline{9-14} 


LOL Normal 10                          & N/A         & \textbf{1,00}      & 0,50            & 0,67          & N/A              &  &  & LOL Normal 10                          & N/A         & \textbf{1,00}      & 0,76            & 0,86                & N/A              \\ \cline{1-6} \cline{9-14} 
LOL Normal 15                          & N/A         & 0,46               & \textbf{0,75}   & 0,57          & N/A              &  &  & LOL Normal 15                          & N/A         & 1,00               & \textbf{0,75}   & 0,86                & N/A              \\ \cline{1-6} \cline{9-14} 
LOL Normal 20                          & N/A         & 0,36               & \textbf{0,83}   & 0,50          & N/A              &  &  & LOL Normal 20                          & N/A         & \textbf{1,00}      & 0,78            & 0,88                & N/A              \\ \cline{1-6} \cline{9-14} 
LOL Normal 25                          & N/A         & 0,31               & \textbf{0,88}   & 0,46          & N/A              &  &  & LOL Normal 25                          & N/A         & 1,00               & 0,73            & \textbf{0,84}       & N/A              \\ \cline{1-6} \cline{9-14} 


KNN-10                                 & 1           & \textbf{0.00}      & 0.00            & 0.00          & 295.30           &  &  & KNN-10                                 & 1           & \textbf{0.87}      & 1.00            & 0.93          & 7.50             \\ \cline{1-6} \cline{9-14} 
KNN-10                                 & 1           & 0.00               & \textbf{0.00}   & 0.00          & 295.30           &  &  & KNN-10                                 & 1           & 0.87               & \textbf{1.00}   & 0.93          & 7.50             \\ \cline{1-6} \cline{9-14} 
KNN-10                                 & 1           & 0.00               & 0.00            & \textbf{0.00} & 295.30           &  &  & KNN-10                                 & 1           & 0.87               & 1.00            & \textbf{0.93} & 7.50             \\ \cline{1-6} \cline{9-14} 
KNN-15                                 & 1           & \textbf{0.00}      & 0.00            & 0.00          & 294.10           &  &  & KNN-15                                 & 1           & \textbf{0.87}      & 1.00            & 0.93          & 7.50             \\ \cline{1-6} \cline{9-14} 
KNN-15                                 & 1           & 0.00               & \textbf{0.00}   & 0.00          & 294.10           &  &  & KNN-15                                 & 1           & 0.87               & \textbf{1.00}   & 0.93          & 7.50             \\ \cline{1-6} \cline{9-14} 
KNN-15                                 & 1           & 0.00               & 0.00            & \textbf{0.00} & 294.10           &  &  & KNN-15                                 & 1           & 0.87               & 1.00            & \textbf{0.93} & 7.50             \\ \cline{1-6} \cline{9-14} 
KNN-20                                 & 1           & \textbf{0.00}      & 0.00            & 0.00          & 294.00           &  &  & KNN-20                                 & 1           & \textbf{0.87}      & 1.00            & 0.93          & 7.50             \\ \cline{1-6} \cline{9-14} 
KNN-20                                 & 1           & 0.00               & \textbf{0.00}   & 0.00          & 294.00           &  &  & KNN-20                                 & 1           & 0.87               & \textbf{1.00}   & 0.93          & 7.50             \\ \cline{1-6} \cline{9-14} 
KNN-20                                 & 1           & 0.00               & 0.00            & \textbf{0.00} & 294.00           &  &  & KNN-20                                 & 1           & 0.87               & 1.00            & \textbf{0.93} & 7.50             \\ \cline{1-6} \cline{9-14} 
KNN-25                                 & 1           & \textbf{0.00}      & 0.00            & 0.00          & 294.00           &  &  & KNN-25                                 & 1           & \textbf{0.87}      & 1.00            & 0.93          & 7.50             \\ \cline{1-6} \cline{9-14} 
KNN-25                                 & 1           & 0.00               & \textbf{0.00}   & 0.00          & 294.00           &  &  & KNN-25                                 & 1           & 0.87               & \textbf{1.00}   & 0.93          & 7.50             \\ \cline{1-6} \cline{9-14} 
KNN-25                                 & 1           & 0.00               & 0.00            & \textbf{0.00} & 294.00           &  &  & KNN-25                                 & 1           & 0.87               & 1.00            & \textbf{0.93} & 7.50            

       \\ \hline \hline
\end{tabular}
\end{table*}

==> tables/Result_Realistic_all_Anomaly_groups.tex <==

\begin{table}[h]
\caption{Results for the realistic datasets}
\label{Table:result:realistic}

\centering
\tiny

% \begin{tabular}{lccccclllccccc}
% % \cline{1-6} \cline{9-14}
% \hline \hline
% \multicolumn{6}{c}{\textbf{Realistic Data Not Pruned}}&  &  & \multicolumn{6}{c}{\textbf{Realistic Data Pruned}}  \\ \cline{1-6} \cline{9-14} 
% \multicolumn{1}{c}{\textbf{Algorithm}} & \textbf{SC} & \textbf{Precision} & \textbf{Recall} & \textbf{F1}    & \textbf{Ins@100} &  &  & \multicolumn{1}{c}{\textbf{Algorithm}} & \textbf{SC} & \textbf{Precision} & \textbf{Recall} & \textbf{F1}    & \textbf{Ins@100} \\ \hline \hline



% SIF   & 20& \textbf{\underline{0.37}} & \underline{0.96}  & \underline{0.53}& \textbf{46.52}  &  &  & SIF   & 20& \textbf{0.39} & 0.93  & 0.55& 53.91  \\ \cline{1-6} \cline{9-14} 
% SIF   & 20& \underline{0.37}& \textbf{\underline{0.96}}   & \underline{0.53}& \textbf{46.52}  &  &  & SIF   & 20& 0.39& \textbf{0.93}   & 0.55& 53.91  \\ \cline{1-6} \cline{9-14} 
% SIF   & 20& \underline{0.37}& \underline{0.96}  & \textbf{\underline{0.53}} &\textbf{46.52}  &  &  & SIF   & 20& 0.39& 0.93  & \textbf{0.55} & 53.91  \\ \cline{1-6} \cline{9-14} 
% IF & N/A    & \textbf{0.00} & 0.00  & 0.00& N/A    &  &  & IF & N/A    & \textbf{0.53} & 0.51  & 0.52& N/A    \\ \cline{1-6} \cline{9-14} 
% SHAC  & 20& \textbf{0.00} & 0.00  & 0.00& 353.53 &  &  & SHAC  & 1 & \textbf{0.94} & 0.84  & \underline{0.88}& 47.80  \\ \cline{1-6} \cline{9-14} 
% SHAC  & 20& 0.00& \textbf{0.00}   & 0.00& 353.53 &  &  & SHAC  & 20& 0.48& \textbf{0.87}   & 0.62& 47.80  \\ \cline{1-6} \cline{9-14} 
% SHAC  & 20& 0.00& 0.00  & \textbf{0.00} & 353.53 &  &  & SHAC  & 1 & 0.94& 0.84  & \textbf{\underline{0.88}} & 47.80  \\ \cline{1-6} \cline{9-14} 
% SKM  & 20& \textbf{0.00} & 0.00  & 0.00& 365.52 &  &  & SKM  & 1 & \textbf{0.94} & 0.83  & 0.88& 49.81  \\ \cline{1-6} \cline{9-14} 
% SKM  & 20& 0.00& \textbf{0.00}   & 0.00& 365.52 &  &  & SKM  & 7 & 0.70& \textbf{0.84}   & 0.76& 49.81  \\ \cline{1-6} \cline{9-14} 
% SKM  & 20& 0.00& 0.00  & \textbf{0.00} & 365.52 &  &  & SKM  & 1 & 0.94& 0.83  & \textbf{\underline{0.88}} & 49.81  \\ \cline{1-6} \cline{9-14} 
% LOF-10 & N/A    & \textbf{0.11}& \textbf{0.10}& \textbf{0.10}   & N/A    &  &  & LOF-10 & N/A    & \textbf{\underline{1.00}}& \textbf{0.75} & \textbf{0.86} & N/A    \\ \cline{1-6} \cline{9-14} 
% LOF-15 & N/A    & \textbf{0.07}    & \textbf{0.15}  & \textbf{0.09}    & N/A    &  &  & LOF-15 & N/A    & \textbf{\underline{1.00}}    & \textbf{0.70}  & \textbf{0.85}& N/A    \\ \cline{1-6} \cline{9-14} 
% LOF-20 & N/A    & \textbf{0.07}    & \textbf{0.20}  & \textbf{0.10}    & N/A    &  &  & LOF-20 & N/A    & \textbf{\underline{1.00}}& \textbf{0.78} & \textbf{0.87}& N/A    \\ \cline{1-6} \cline{9-14} 
% LOF-25 & N/A    & \textbf{0.07}   & \textbf{0.25}  & \textbf{0.11}   & N/A    &  &  & LOF-25 & N/A    & \textbf{\underline{1.00}}    & \textbf{0.72}   & \textbf{0.84} & N/A    \\ \cline{1-6} \cline{9-14} 

% SKNN-10   & 1 & \textbf{0.00} & 0.00  & 0.00& 363.27 &  &  & SKNN-10   & 1 & \textbf{0.89} & 0.65  & 0.75& 36.31  \\ \cline{1-6} \cline{9-14} 
% SKNN-10   & 1 & 0.00& \textbf{0.00}   & 0.00& 363.27 &  &  & SKNN-10   & 20& 0.48& \textbf{0.98}   & 0.65& 36.31  \\ \cline{1-6} \cline{9-14} 
% SKNN-10   & 1 & 0.00& 0.00  & \textbf{0.00} & 363.27 &  &  & SKNN-10   & 1 & 0.89& 0.65  & \textbf{0.75} & 36.31  \\ \cline{1-6} \cline{9-14} 
% SKNN-15   & 1 & \textbf{0.00} & 0.00  & 0.00& 363.26 &  &  & SKNN-15   & 1 & \textbf{0.90} & 0.66  & 0.76& 30.92  \\ \cline{1-6} \cline{9-14} 
% SKNN-15   & 1 & 0.00& \textbf{0.00}   & 0.00& 363.26 &  &  & SKNN-15   & 20& 0.51& \textbf{\underline{1.00}}   & 0.67& 30.92  \\ \cline{1-6} \cline{9-14} 
% SKNN-15   & 1 & 0.00& 0.00  & \textbf{0.00} & 363.26 &  &  & SKNN-15   & 4 & 0.78& 0.95  & \textbf{0.86} & 30.92  \\ \cline{1-6} \cline{9-14} 
% SKNN-20   & 1 & \textbf{0.00} & 0.00  & 0.00& 361.53 &  &  & SKNN-20   & 1 & \textbf{0.91} & 0.66  & 0.77& \textbf{30.65}  \\ \cline{1-6} \cline{9-14} 
% SKNN-20   & 1 & 0.00& \textbf{0.00}   & 0.00& 361.53 &  &  & SKNN-20   & 20& 0.51& \textbf{\underline{1.00}}   & 0.67& \textbf{30.65}  \\ \cline{1-6} \cline{9-14} 
% SKNN-20   & 1 & 0.00& 0.00  & \textbf{0.00} & 361.53 &  &  & SKNN-20   & 4 & 0.78& 0.97  & \textbf{0.87} &\textbf{30.65}  \\ \cline{1-6} \cline{9-14} 
% SKNN-25   & 1 & \textbf{0.00} & 0.00  & 0.00& 361.63 &  &  & SKNN-25   & 1 & \textbf{0.91} & 0.66  & 0.76& 31.19  \\ \cline{1-6} \cline{9-14} 
% SKNN-25   & 1 & 0.00& \textbf{0.00}   & 0.00& 361.63 &  &  & SKNN-25   & 20& 0.50& \textbf{\underline{1.00}}   & 0.67& 31.19  \\ \cline{1-6} \cline{9-14} 
% SKNN-25   & 1 & 0.00& 0.00  & \textbf{0.00} & 361.63 &  &  & SKNN-25   & 4 & 0.78& 0.96  & \textbf{0.86} & 31.19  
\begin{tabular}{lccccc|ccccc}
\hline \hline

\multicolumn{6}{c|}{\textbf{Without Pruning}}                                                                                            & \multicolumn{5}{c}{\textbf{With Pruning}}                                                      \\ \hline \hline
\multicolumn{1}{c|}{\textbf{Algorithm}} & \textbf{SC} & \textbf{Prec.}      & \textbf{Rec.}       & \textbf{F1}         & \textbf{DC}    & \textbf{SC} & \textbf{Prec.}      & \textbf{Rec.}       & \textbf{F1}         & \textbf{DC}    \\ \hline
\multicolumn{1}{l|}{SIF}                & 20          & \ul{ \textbf{0.37}} & \ul{ 0.96}          & \ul{ 0.53}          & \textbf{46.52} & 20          & \textbf{0.39}       & 0.93                & 0.55                & 53.91          \\ \hline
\multicolumn{1}{l|}{SIF}                & 20          & \ul{ 0.37}          & \ul{ \textbf{0.96}} & \ul{ 0.53}          & \textbf{46.52} & 20          & 0.39                & \textbf{0.93}       & 0.55                & 53.91          \\ \hline
\multicolumn{1}{l|}{SIF}                & 20          & \ul{ 0.37}          & \ul{ 0.96}          & \ul{ \textbf{0.53}} & \textbf{46.52} & 20          & 0.39                & 0.93                & \textbf{0.55}       & 53.91          \\ \hline
\multicolumn{1}{l|}{IF}                 & N/A         & \textbf{0.00}       & 0.00                & 0.00                & N/A            & N/A         & \textbf{0.53}       & 0.51                & 0.52                & N/A            \\ \hline
\multicolumn{1}{l|}{SHAC}               & 20          & \textbf{0.00}       & 0.00                & 0.00                & 353.53         & 1           & \textbf{0.94}       & 0.84                & \ul{ 0.88}          & 47.80          \\ \hline
\multicolumn{1}{l|}{SHAC}               & 20          & 0.00                & \textbf{0.00}       & 0.00                & 353.53         & 20          & 0.48                & \textbf{0.87}       & 0.62                & 47.80          \\ \hline
\multicolumn{1}{l|}{SHAC}               & 20          & 0.00                & 0.00                & \textbf{0.00}       & 353.53         & 1           & 0.94                & 0.84                & \ul{ \textbf{0.88}} & 47.80          \\ \hline
\multicolumn{1}{l|}{SKM}                & 20          & \textbf{0.00}       & 0.00                & 0.00                & 365.52         & 1           & \textbf{0.94}       & 0.83                & \ul{ 0.88}          & 49.81          \\ \hline
\multicolumn{1}{l|}{SKM}                & 20          & 0.00                & \textbf{0.00}       & 0.00                & 365.52         & 7           & 0.70                & \textbf{0.84}       & 0.76                & 49.81          \\ \hline
\multicolumn{1}{l|}{SKM}                & 20          & 0.00                & 0.00                & \textbf{0.00}       & 365.52         & 1           & 0.94                & 0.83                & \ul{ \textbf{0.88}} & 49.81          \\ \hline
\multicolumn{1}{l|}{LOF-10}             & N/A         & \textbf{0.11}       & \textbf{0.10}       & \textbf{0.11}       & N/A            & N/A         & \ul{ \textbf{1.00}} & \textbf{0.75}       & \textbf{0.86}       & N/A            \\ \hline
\multicolumn{1}{l|}{LOF-15}             & N/A         & \textbf{0.07}       & \textbf{0.15}       & \textbf{0.09}       & N/A            & N/A         & \ul{ \textbf{1.00}} & \textbf{0.70}       & \textbf{0.85}       & N/A            \\ \hline
\multicolumn{1}{l|}{LOF-20}             & N/A         & \textbf{0.07}       & \textbf{0.20}       & \textbf{0.10}       & N/A            & N/A         & \ul{ \textbf{1.00}} & \textbf{0.78}       & \textbf{0.87}       & N/A            \\ \hline
\multicolumn{1}{l|}{LOF-25}             & N/A         & \textbf{0.07}       & \textbf{0.25}       & \textbf{0.11}       & N/A            & N/A         & \ul{ \textbf{1.00}} & \textbf{0.72}       & \textbf{0.84}       & N/A            \\ \hline
\multicolumn{1}{l|}{SKNN-10}            & 1           & \textbf{0.00}       & 0.00                & 0.00                & 363.27         & 1           & \textbf{0.89}       & 0.65                & 0.75                & 36.31          \\ \hline
\multicolumn{1}{l|}{SKNN-10}            & 1           & 0.00                & \textbf{0.00}       & 0.00                & 363.27         & 20          & 0.48                & \textbf{0.98}       & 0.65                & 36.31          \\ \hline
\multicolumn{1}{l|}{SKNN-10}            & 1           & 0.00                & 0.00                & \textbf{0.00}       & 363.27         & 1           & 0.89                & 0.65                & \textbf{0.75}       & 36.31          \\ \hline
\multicolumn{1}{l|}{SKNN-15}            & 1           & \textbf{0.00}       & 0.00                & 0.00                & 363.26         & 1           & \textbf{0.90}       & 0.66                & 0.76                & 30.92          \\ \hline
\multicolumn{1}{l|}{SKNN-15}            & 1           & 0.00                & \textbf{0.00}       & 0.00                & 363.26         & 20          & 0.51                & \ul{ \textbf{1.00}} & 0.67                & 30.92          \\ \hline
\multicolumn{1}{l|}{SKNN-15}            & 1           & 0.00                & 0.00                & \textbf{0.00}       & 363.26         & 4           & 0.78                & 0.95                & \textbf{0.86}       & 30.92          \\ \hline
\multicolumn{1}{l|}{SKNN-20}            & 1           & \textbf{0.00}       & 0.00                & 0.00                & 361.53         & 1           & \textbf{0.91}       & 0.66                & 0.77                & \textbf{30.65} \\ \hline
\multicolumn{1}{l|}{SKNN-20}            & 1           & 0.00                & \textbf{0.00}       & 0.00                & 361.53         & 20          & 0.51                & \ul{ \textbf{1.00}} & 0.67                & \textbf{30.65} \\ \hline
\multicolumn{1}{l|}{SKNN-20}            & 1           & 0.00                & 0.00                & \textbf{0.00}       & 361.53         & 4           & 0.78                & 0.97                & \textbf{0.87}       & \textbf{30.65} \\ \hline
\multicolumn{1}{l|}{SKNN-25}            & 1           & \textbf{0.00}       & 0.00                & 0.00                & 361.63         & 1           & \textbf{0.91}       & 0.66                & 0.76                & 31.19          \\ \hline
\multicolumn{1}{l|}{SKNN-25}            & 1           & 0.00                & \textbf{0.00}       & 0.00                & 361.63         & 20          & 0.50                & \ul{ \textbf{1.00}} & 0.67                & 31.19          \\ \hline
\multicolumn{1}{l|}{SKNN-25}            & 1           & 0.00                & 0.00                & \textbf{0.00}       & 361.63         & 4           & 0.78                & 0.96                & \textbf{0.86}       & 31.19 

\\ \hline \hline 
\end{tabular}
\end{table}

==> tables/Result_Synthetic_5n10_Anomaly_groups.tex <==

\begin{table*}[]
\caption{Results for Synthetic data Filtered and Unfiltered for 5 and 10 Anomaly Groups}
\label{Table:result:synthetic:five}
\begin{tabular}{lccccclllccccc}
\hline \hline
\multicolumn{6}{c}{\textbf{Synthetic Data Unfiltered}}                                                                                &  &  & \multicolumn{6}{c}{\textbf{Synthetic Data Filtered}}                                                                   \\ \cline{1-6} \cline{9-14} 
\multicolumn{1}{c}{\textbf{Algorithm}} & \textbf{SC} & \textbf{Precision} & \textbf{Recall} & \textbf{F1}    & \textbf{Ins@100} &  &  & \multicolumn{1}{c}{\textbf{Algorithm}} & \textbf{SC} & \textbf{Precision} & \textbf{Recall} & \textbf{F1}    & \textbf{Ins@100} \\ \hline \hline


Isolation Forest                       & 1           & \textbf{0.94}      & 0.88            & 0.91          & 41.29            &  &  & Isolation Forest                       & 1           & \textbf{0.88}      & 1.00            & 0.93          & 7.81             \\ \cline{1-6} \cline{9-14} 
Isolation Forest                       & 20          & 0.50               & \textbf{0.94}   & 0.65          & 41.29            &  &  & Isolation Forest                       & 1           & 0.88               & \textbf{1.00}   & 0.93          & 7.81             \\ \cline{1-6} \cline{9-14} 
Isolation Forest                       & 1           & 0.94               & 0.88            & \textbf{0.91} & 41.29            &  &  & Isolation Forest                       & 1           & 0.88               & 1.00            & \textbf{0.93} & 7.81             \\ \cline{1-6} \cline{9-14} 
Isolation Fores-N                      & N/A         & \textbf{0.00}      & 0.00            & 0.00          & N/A              &  &  & Isolation Forest-N                     & N/A         & \textbf{0.00}      & 0.00            & 0.00          & N/A              \\ \cline{1-6} \cline{9-14} 
AG                                     & 1           & \textbf{0.92}      & 0.75            & 0.83          & 247.79           &  &  & AG                                     & 1           & \textbf{0.80}      & 0.80            & 0.80          & 40.64            \\ \cline{1-6} \cline{9-14} 
AG                                     & 20          & 0.46               & \textbf{0.76}   & 0.58          & 247.79           &  &  & AG                                     & 20          & 0.24               & \textbf{0.85}   & 0.37          & 40.64            \\ \cline{1-6} \cline{9-14} 
AG                                     & 1           & 0.92               & 0.75            & \textbf{0.83} & 247.79           &  &  & AG                                     & 1           & 0.80               & 0.80            & \textbf{0.80} & 40.64            \\ \cline{1-6} \cline{9-14} 
k-means                                & 1           & \textbf{0.92}      & 0.76            & 0.83          & 301.87           &  &  & k-means                                & 1           & \textbf{0.78}      & 0.70            & 0.74          & 51.05            \\ \cline{1-6} \cline{9-14} 
k-means                                & 20          & 0.47               & \textbf{0.78}   & 0.58          & 301.87           &  &  & k-means                                & 20          & 0.21               & \textbf{0.78}   & 0.32          & 51.05            \\ \cline{1-6} \cline{9-14} 
k-means                                & 1           & 0.92               & 0.76            & \textbf{0.83} & 301.87           &  &  & k-means                                & 1           & 0.78               & 0.70            & \textbf{0.74} & 51.05            \\ \cline{1-6} \cline{9-14} 
LOL Normal 10                          & N/A         & \textbf{1,00}      & 1,00            & \textbf{1,00} & N/A              &  &  & LOL Normal 10                          & N/A         & \textbf{1,00}      & \textbf{1,00}   & \textbf{1,00} & N/A              \\ \cline{1-6} \cline{9-14} 
LOL Normal 15                          & N/A         & 0,71               & \textbf{1,00}   & 0,83          & N/A              &  &  & LOL Normal 15                          & N/A         & \textbf{0,73}      & 1,00            & 0,84          & N/A              \\ \cline{1-6} \cline{9-14} 
LOL Normal 20                          & N/A         & \textbf{0,52}      & 1,00            & 0,68          & N/A              &  &  & LOL Normal 20                          & N/A         & 0,54               & \textbf{1,00}   & 0,70          & N/A              \\ \cline{1-6} \cline{9-14} 
LOL Normal 25                          & N/A         & 0,43               & \textbf{1,00}   & 0,60          & N/A              &  &  & LOL Normal 25                          & N/A         & 0,44               & \textbf{1,00}   & \textbf{0,61} & N/A              \\ \cline{1-6} \cline{9-14} 

KNN-10                                 & 1           & \textbf{0.94}      & 0.87            & 0.91          & 156.26           &  &  & KNN-10                                 & 1           & \textbf{0.88}      & 1.00            & 0.93          & 7.86             \\ \cline{1-6} \cline{9-14} 
KNN-10                                 & 20          & 0.47               & \textbf{0.88}   & 0.62          & 156.26           &  &  & KNN-10                                 & 1           & 0.88               & \textbf{1.00}   & 0.93          & 7.86             \\ \cline{1-6} \cline{9-14} 
KNN-10                                 & 1           & 0.94               & 0.87            & \textbf{0.91} & 156.26           &  &  & KNN-10                                 & 1           & 0.88               & 1.00            & \textbf{0.93} & 7.86             \\ \cline{1-6} \cline{9-14} 
KNN-15                                 & 1           & \textbf{0.94}      & 0.92            & 0.93          & 56.03            &  &  & KNN-15                                 & 1           & \textbf{0.88}      & 1.00            & 0.93          & 7.86             \\ \cline{1-6} \cline{9-14} 
KNN-15                                 & 20          & 0.50               & \textbf{0.96}   & 0.66          & 56.03            &  &  & KNN-15                                 & 1           & 0.88               & \textbf{1.00}   & 0.93          & 7.86             \\ \cline{1-6} \cline{9-14} 
KNN-15                                 & 1           & 0.94               & 0.92            & \textbf{0.93} & 56.03            &  &  & KNN-15                                 & 1           & 0.88               & 1.00            & \textbf{0.93} & 7.86             \\ \cline{1-6} \cline{9-14} 
KNN-20                                 & 1           & \textbf{0.94}      & 0.92            & 0.93          & 37.86            &  &  & KNN-20                                 & 1           & \textbf{0.88}      & 1.00            & 0.93          & 7.86             \\ \cline{1-6} \cline{9-14} 
KNN-20                                 & 20          & 0.50               & \textbf{0.96}   & 0.66          & 37.86            &  &  & KNN-20                                 & 1           & 0.88               & \textbf{1.00}   & 0.93          & 7.86             \\ \cline{1-6} \cline{9-14} 
KNN-20                                 & 1           & 0.94               & 0.92            & \textbf{0.93} & 37.86            &  &  & KNN-20                                 & 1           & 0.88               & 1.00            & \textbf{0.93} & 7.86             \\ \cline{1-6} \cline{9-14} 
KNN-25                                 & 1           & \textbf{0.94}      & 0.92            & 0.93          & 34.92            &  &  & KNN-25                                 & 1           & \textbf{0.88}      & \textbf{1.00}   & \textbf{0.93} & 7.86             \\ \cline{1-6} \cline{9-14} 
KNN-25                                 & 20          & 0.50               & \textbf{0.96}   & 0.66          & 34.92            &  &  & KNN-25                                 & 1           & 0.88               & \textbf{1.00}   & 0.93          & 7.86             \\ \cline{1-6} \cline{9-14} 
KNN-25                                 & 1           & 0.94               & 0.92            & \textbf{0.93} & 34.92            &  &  & KNN-25                                 & 1           & 0.88               & 1.00            & \textbf{0.93} & 7.86           




\\    \hline \hline
\end{tabular}
\end{table*}

==> tables/Result_Synthetic_all_Anomaly_groups.tex <==




\begin{table}[h]
\caption{Results for the synthetic datasets}
\label{Table:result:synthetic}
\tiny
\centering
% \begin{tabular}{lc|cccc|lccccc}
% \hline \hline
% % \cline{1-6} \cline{10-15}
% %\cline{1-6} \cline{7-12}
% \multicolumn{2}{c|}{}&
% \multicolumn{4}{c|}{\textbf{Without Pruning}}                                                                                & \multicolumn{6}{c}{\textbf{With Pruning}}                                                                   \\ \cline{1-6} \cline{7-12} 
% \multicolumn{1}{c}{\textbf{Algo.}} & \textbf{SC} & \textbf{Prec.} & \textbf{Rec.} & \textbf{F1}    & \textbf{DC} & \multicolumn{1}{c}{\textbf{Algo.}} & \textbf{SC} & \textbf{Prec.} & \textbf{Rec.} & \textbf{F1}    & \textbf{DC} \\   \hline \hline

% SIF                       & 1           & \textbf{0.94}      & 0.88            & 0.91          & 41.11            & SIF                       & 1           & \textbf{0.94}      & 0.90                & 0.92                & \textbf{35.48}      \\ \cline{1-6} \cline{7-12} 
% SIF                       & 20          & 0.50               & \textbf{0.94}   & 0.65          & 41.11            & SIF                       & 20          & 0.50               & \textbf{0.94}       & 0.65                &  \textbf{35.48}      \\ \cline{1-6} \cline{7-12} 
% SIF                       & 1           & 0.94               & 0.88            & \textbf{0.91} & 41.11            & SIF                       & 1           & 0.94               & 0.90                & \textbf{0.92}       & \textbf{35.48}      \\ \cline{1-6} \cline{7-12} 
% IF                    & N/A         & \textbf{0.00}      & \textbf{0.00}            &\textbf{ 0.00  }        & N/A              & IF                    & N/A         & \textbf{0.06}      &\textbf{ 0.17}                & \textbf{0.08}                & N/A              \\ \cline{1-6} \cline{7-12} 
% SHAC                                     & 1           & \textbf{0.92}      & 0.75            & 0.83          & 247.88           & SHAC                                     & 1           & \textbf{0.92}      & 0.77                & 0.84                & 50.00            \\ \cline{1-6} \cline{7-12} 
% SHAC                                     & 20          & 0.46               & \textbf{0.76}   & 0.58          & 247.88           & SHAC                                     & 20          & 0.46               & \textbf{0.80}       & 0.59                & 50.00            \\ \cline{1-6} \cline{7-12} 
% SHAC                                     & 1           & 0.92               & 0.75            & \textbf{0.83} & 247.88           & SHAC                                     & 1           & 0.92               & 0.77                & \textbf{0.84}       & 50.00            \\ \cline{1-6} \cline{7-12} 
% SKM                                & 1           & \textbf{0.92}      & 0.76            & 0.83          & 298.66           & SKM                                & 1           & \textbf{0.92}      & 0.69                & 0.79                & 60.79            \\ \cline{1-6} \cline{7-12} 
% SKM                                & 20          & 0.47               & \textbf{0.78}   & 0.58          & 298.66           & SKM                                & 20          & 0.43               & \textbf{0.75}       & 0.55                & 60.79            \\ \cline{1-6} \cline{7-12} 
% SKM                                & 1           & 0.92               & 0.76            & \textbf{0.83} & 298.66           & SKM                                & 1           & 0.92               & 0.69                & \textbf{0.79}       & 60.79            \\ \cline{1-6} \cline{7-12} 
% LOF-10                          & N/A         & \textbf{\underline{1.00}}     & \textbf{0.83}  & \textbf{0.91}          & N/A              & LOF-10                          & N/A         & \textbf{1.00}    & \textbf{0.83}               & \textbf{0.91}       & N/A              \\ \cline{1-6} \cline{7-12} 
% LOF-15                          & N/A         &\textbf{0.75}             &\textbf{0.88}          & \textbf{0.81} & N/A              & LOF-15                          & N/A         & \textbf{0.79}      &\textbf{0.88}                &\textbf{ 0.83 }               & N/A              \\ \cline{1-6} \cline{7-12} 
% LOF-20                          & N/A         &\textbf{0.62}             & \textbf{0.91}  & \textbf{0.73}          & N/A              & LOF-20                          & N/A         & \textbf{0.65}               & \textbf{0.91}       & \textbf{0.76}                & N/A              \\ \cline{1-6} \cline{7-12} 
% LOF-25                          & N/A         &\textbf{0.55}             & \textbf{0.93}  & \textbf{0.69} & N/A              & LOF-25                          & N/A         &\textbf{0.58}               & \textbf{0.93}       & \textbf{0.71}       & N/A              \\ \cline{1-6} \cline{7-12} 
% SKNN-10                                 & 1           & \textbf{0.94}      & 0.87            & 0.91          & 156.25           & SKNN-10                                 & 1           & \textbf{0.94}      & 0.88                & 0.91                & 59.18            \\ \cline{1-6} \cline{7-12} 
% SKNN-10                                 & 20          & 0.47               & \textbf{0.88}   & 0.62          & 156.25           & SKNN-10                                 & 20          & 0.43               &  \textbf{\underline{0.96}} & 0.59                & 59.18            \\ \cline{1-6} \cline{7-12} 
% SKNN-10                                 & 1           & 0.94               & 0.87            & \textbf{0.91} & 156.25           & SKNN-10                                 & 1           & 0.94               & 0.88                & \textbf{0.91}       & 59.18            \\ \cline{1-6} \cline{7-12} 
% SKNN-15                                 & 1           & \textbf{0.94}      & 0.92            & \underline{0.93}          & 56.01            & SKNN-15                                 & 1           & \textbf{\underline{0.95}}      & 0.93                & \underline{0.94}                & 36.44            \\ \cline{1-6} \cline{7-12} 
% SKNN-15                                 & 20          & 0.50               & \textbf{\underline{0.96}}   & 0.66          & 56.01            & SKNN-15                                 & 20          & 0.51               & \textbf{0.95}       & 0.66                & 36.44            \\ \cline{1-6} \cline{7-12} 
% SKNN-15                                 & 1           & 0.94               & 0.92            & \textbf{\underline{0.93}} & 56.01            & SKNN-15                                 & 1           & \underline{0.95}               & 0.93                & \textbf{\underline{0.94}} & 36.44            \\ \cline{1-6} \cline{7-12} 
% SKNN-20                                 & 1           & \textbf{0.94}      & 0.92            & \underline{0.93}          & 37.85            & SKNN-20                                 & 1           & \textbf{0.94}      & 0.89                & 0.92                & 37.98            \\ \cline{1-6} \cline{7-12} 
% SKNN-20                                 & 20          & 0.50               & \textbf{\underline{0.96}}   & 0.66          & 37.85            & SKNN-20                                 & 20          & 0.50               & \textbf{0.92}       & 0.65                & 37.98            \\ \cline{1-6} \cline{7-12} 
% SKNN-20                                 & 1           & 0.94               & 0.92            & \textbf{\underline{0.93}} & 37.85            & SKNN-20                                 & 1           & 0.94               & 0.89                & \textbf{0.92}       & 37.98            \\ \cline{1-6} \cline{7-12} 
% SKNN-25                                 & 1           & \textbf{0.94}      & 0.92            & \underline{0.93}          & \textbf{34.91}            & SKNN-25                                 & 1           & \textbf{0.94}      & 0.86                & \textbf{0.90}       & 41.19            \\ \cline{1-6} \cline{7-12} 
% SKNN-25                                 & 20          & 0.50               & \textbf{\underline{0.96}}   & 0.66          & \textbf{34.91}            & SKNN-25                                 & 20          & 0.49               & \textbf{0.88}       & 0.63                & 41.19            \\ \cline{1-6} \cline{7-12} 
% SKNN-25                                 & 1           & 0.94               & 0.92            & \textbf{\underline{0.93}} & \textbf{34.91}            & SKNN-25                                 & 1           & 0.94               & 0.86                & \textbf{0.90}       & 41.19  

\begin{tabular}{lccccc|ccccc}
\hline \hline

\multicolumn{6}{c|}{\textbf{Without Pruning}}                                                                                            & \multicolumn{5}{c}{\textbf{With Pruning}}                                                      \\ \hline
\multicolumn{1}{c|}{\textbf{Algorithm}} & \textbf{SC} & \textbf{Prec.}      & \textbf{Rec.}       & \textbf{F1}         & \textbf{DC}    & \textbf{SC} & \textbf{Prec.}      & \textbf{Rec.}       & \textbf{F1}         & \textbf{DC}    \\ \hline \hline
\multicolumn{1}{l|}{SIF}                & 1           & \textbf{0,94}       & 0,88                & 0,91                & 41,11          & 1           & \textbf{0,94}       & 0,90                & 0,92                & \textbf{35,48} \\ \hline
\multicolumn{1}{l|}{SIF}                & 20          & 0,50                & \textbf{0,94}       & 0,65                & 41,11          & 20          & 0,50                & \textbf{0,94}       & 0,65                & \textbf{35,48} \\ \hline
\multicolumn{1}{l|}{SIF}                & 1           & 0,94                & 0,88                & \textbf{0,91}       & 41,11          & 1           & 0,94                & 0,90                & \textbf{0,92}       & \textbf{35,48} \\ \hline
\multicolumn{1}{l|}{IF}                 & N/A         & \textbf{0,00}       & \textbf{0,00}       & \textbf{0,00}       & N/A            & N/A         & \textbf{0,06}       & 0,17                & 0,08                & N/A            \\ \hline
\multicolumn{1}{l|}{SHAC}               & 1           & \textbf{0,92}       & 0,75                & 0,83                & 247,88         & 1           & \textbf{0,92}       & 0,77                & 0,84                & 50,00          \\ \hline
\multicolumn{1}{l|}{SHAC}               & 20          & 0,46                & \textbf{0,76}       & 0,58                & 247,88         & 20          & 0,46                & \textbf{0,80}       & 0,59                & 50,00          \\ \hline
\multicolumn{1}{l|}{SHAC}               & 1           & 0,92                & 0,75                & \textbf{0,83}       & 247,88         & 1           & 0,92                & 0,77                & \textbf{0,84}       & 50,00          \\ \hline
\multicolumn{1}{l|}{SKM}                & 1           & \textbf{0,92}       & 0,76                & 0,83                & 298,66         & 1           & \textbf{0,92}       & 0,69                & 0,79                & 60,79          \\ \hline
\multicolumn{1}{l|}{SKM}                & 20          & 0,47                & \textbf{0,78}       & 0,58                & 298,66         & 20          & 0,43                & \textbf{0,75}       & 0,55                & 60,79          \\ \hline
\multicolumn{1}{l|}{SKM}                & 1           & 0,92                & 0,76                & \textbf{0.83}       & 298,66         & 1           & 0,92                & 0,69                & \textbf{0,79}       & 60,79          \\ \hline
\multicolumn{1}{l|}{LOF-10}             & N/A         & {\ul \textbf{1,00}} & \textbf{0,83}       & \textbf{0,91}       & N/A            & N/A         & \textbf{1,00}       & 0,83                & \textbf{0,91}       & N/A            \\ \hline
\multicolumn{1}{l|}{LOF-15}             & N/A         & \textbf{0,75}       & \textbf{0.88}       & \textbf{0,81}       & N/A            & N/A         & \textbf{0,79}       & 0,88                & 0,83                & N/A            \\ \hline
\multicolumn{1}{l|}{LOF-20}             & N/A         & \textbf{0,62}       & \textbf{0,91}       & \textbf{0.73}       & N/A            & N/A         & 0,65                & \textbf{0,91}       & 0,76                & N/A            \\ \hline
\multicolumn{1}{l|}{LOF-25}             & N/A         & \textbf{0,55}       & \textbf{0,93}       & \textbf{0,70}       & N/A            & N/A         & 0,58                & \textbf{0,93}       & \textbf{0,71}       & N/A            \\ \hline
\multicolumn{1}{l|}{SKNN-10}            & 1           & \textbf{0,94}       & 0,87                & 0,91                & 156,25         & 1           & \textbf{0,94}       & 0,88                & 0,91                & 59,18          \\ \hline
\multicolumn{1}{l|}{SKNN-10}            & 20          & 0,47                & \textbf{0,88}       & 0,62                & 156,25         & 20          & 0,43                & {\ul \textbf{0,96}} & 0,59                & 59,18          \\ \hline
\multicolumn{1}{l|}{SKNN-10}            & 1           & 0,94                & 0,87                & \textbf{0,91}       & 156,25         & 1           & 0,94                & 0,88                & \textbf{0,91}       & 59,18          \\ \hline
\multicolumn{1}{l|}{SKNN-15}            & 1           & \textbf{0,94}       & 0,92                & {\ul 0,93}          & 56,01          & 1           & {\ul \textbf{0,95}} & 0,93                & {\ul 0,94}          & 36,44          \\ \hline
\multicolumn{1}{l|}{SKNN-15}            & 20          & 0,50                & {\ul \textbf{0,96}} & 0,66                & 56,01          & 20          & 0,51                & \textbf{0,95}       & 0,66                & 36,44          \\ \hline
\multicolumn{1}{l|}{SKNN-15}            & 1           & 0,94                & 0,92                & {\ul \textbf{0,93}} & 56,01          & 1           & {\ul 0,95}          & 0,93                & {\ul \textbf{0,94}} & 36,44          \\ \hline
\multicolumn{1}{l|}{SKNN-20}            & 1           & \textbf{0,94}       & 0,92                & {\ul 0,93}          & 37,85          & 1           & \textbf{0,94}       & 0,89                & 0,92                & 37,98          \\ \hline
\multicolumn{1}{l|}{SKNN-20}            & 20          & 0,50                & \textbf{0,96}       & 0,66                & 37,85          & 20          & 0,50                & \textbf{0,92}       & 0,65                & 37,98          \\ \hline
\multicolumn{1}{l|}{SKNN-20}            & 1           & 0,94                & 0,92                & {\ul \textbf{0,93}} & 37,85          & 1           & 0,94                & 0,89                & \textbf{0,92}       & 37,98          \\ \hline
\multicolumn{1}{l|}{SKNN-25}            & 1           & \textbf{0,94}       & 0,92                & {\ul 0,93}          & \textbf{34,91} & 1           & \textbf{0,94}       & 0,86                & \textbf{0,90}       & 41,19          \\ \hline
\multicolumn{1}{l|}{SKNN-25}            & 20          & 0,50                & {\ul \textbf{0,96}} & 0,66                & \textbf{34,91} & 20          & 0,49                & \textbf{0,88}       & 0,63                & 41,19          \\ \hline
\multicolumn{1}{l|}{SKNN-25}            & 1           & 0,94                & 0,92                & {\ul \textbf{0,93}} & \textbf{34,91} & 1           & 0,94                & 0,86                & \textbf{0,90}       & 41,19

\\ \hline \hline
\end{tabular}
% \begin{minipHACe}[t]{14.5cm}
%\begin{tabbing}
% \vspace{1mm} % just a little padding from table
% \textbf{Abbreviation Terms}:\\
% \hspace{2mm}\textbf{SIF:} Sorted Isolation Forest.
% \hspace{2mm}\textbf{SKNN:} Sorted K Nearest Neighbour.
% \hspace{2mm}\textbf{DC:} Debugging Cost



% \end{minipHACe}



\end{table}

==> tables/Result_real.tex <==


\begin{table*}[h]
\caption{Results for full Real data and without zero}
\label{Table:result:realistic}
\tiny
\begin{tabular}{lcccccllllccccc}
\hline \hline
% \cline{1-6} \cline{10-15}
\multicolumn{6}{c}{\textbf{Real Data Full}}                                                                                &  &  &  & \multicolumn{6}{c}{\textbf{Real Data without Zero Rows}}                                                                   \\ \cline{1-6} \cline{10-15} 
\multicolumn{1}{c}{\textbf{Algorithm}} & \textbf{SC} & \textbf{Precision} & \textbf{Recall} & \textbf{F1}    & \textbf{Ins@100} &  &  &  & \multicolumn{1}{c}{\textbf{Algorithm}} & \textbf{SC} & \textbf{Precision} & \textbf{Recall} & \textbf{F1}    & \textbf{Ins@100} \\ \hline\hline
Isolation Forest                       & 20          & \textbf{0,319}     & 1,000           & 0,484          & 9,980            &  &  &  & Isolation Forest                       & 20          & \textbf{0,417}     & 1,000           & 0,588          & 14,480           \\ \cline{1-6} \cline{10-15} 
Isolation Forest                       & 20          & 0,319              & \textbf{1,000}  & 0,484          & 9,980            &  &  &  & Isolation Forest                       & 20          & 0,417              & \textbf{1,000}  & 0,588          & 14,480           \\ \cline{1-6} \cline{10-15} 
Isolation Forest                       & 20          & 0,319              & 1,000           & \textbf{0,484} & 9,980            &  &  &  & Isolation Forest                       & 20          & 0,417              & 1,000           & \textbf{0,588} & 14,480           \\ \cline{1-6} \cline{10-15} 
Isolation Fores-N                      & N/A         & \textbf{0,004}     & 0,335           & 0,008          & N/A              &  &  &  & Isolation Forest-N                     & N/A         & \textbf{0,585}     & 0,969           & 0,730          & N/A              \\ \cline{1-6} \cline{10-15} 
AG                                     & 1           & \textbf{0,383}     & 0,500           & 0,434          & 10,400           &  &  &  & AG                                     & 20          & \textbf{0,417}     & 1,000           & 0,588          & 15,000           \\ \cline{1-6} \cline{10-15} 
AG                                     & 20          & 0,319              & \textbf{1,000}  & 0,484          & 10,400           &  &  &  & AG                                     & 20          & 0,417              & \textbf{1,000}  & 0,588          & 15,000           \\ \cline{1-6} \cline{10-15} 
AG                                     & 20          & 0,319              & 1,000           & \textbf{0,484} & 10,400           &  &  &  & AG                                     & 20          & 0,417              & 1,000           & \textbf{0,588} & 15,000           \\ \cline{1-6} \cline{10-15} 
k-means                                & 1           & \textbf{0,343}     & 0,450           & 0,389          & 10,010           &  &  &  & k-means                                & 20          & \textbf{0,419}     & 1,000           & 0,590          & 15,120           \\ \cline{1-6} \cline{10-15} 
k-means                                & 20          & 0,319              & \textbf{1,000}  & 0,484          & 10,010           &  &  &  & k-means                                & 20          & 0,419              & \textbf{1,000}  & 0,590          & 15,120           \\ \cline{1-6} \cline{10-15} 
k-means                                & 20          & 0,319              & 1,000           & \textbf{0,484} & 10,010           &  &  &  & k-means                                & 20          & 0,419              & 1,000           & \textbf{0,590} & 15,120           \\ \cline{1-6} \cline{10-15} 
LOL Normal 10                          & N/A         & 0,319              & 0,665           & 0,432          & N/A              &  &  &  & LOL Normal 10                          & N/A         & 0,000              & 0,000           & 0,000          & N/A              \\ \cline{1-6} \cline{10-15} 
LOL Normal 15                          & N/A         & 0,319              & 0,665           & 0,432          & N/A              &  &  &  & LOL Normal 15                          & N/A         & 0,000              & 0,000           & 0,000          & N/A              \\ \cline{1-6} \cline{10-15} 
LOL Normal 20                          & N/A         & 0,319              & 0,665           & 0,432          & N/A              &  &  &  & LOL Normal 20                          & N/A         & 0,000              & 0,000           & 0,000          & N/A              \\ \cline{1-6} \cline{10-15} 
LOL Normal 25                          & N/A         & 0,319              & 0,665           & 0,432          & N/A              &  &  &  & LOL Normal 25                          & N/A         & 0,000              & 0,000           & 0,000          & N/A              \\ \cline{1-6} \cline{10-15} 
KNN-10                                 & 20          & \textbf{0,319}     & 1,000           & 0,484          & 11,250           &  &  &  & KNN-10                                 & 20          & \textbf{0,417}     & 1,000           & 0,588          & 17,500           \\ \cline{1-6} \cline{10-15} 
KNN-10                                 & 20          & 0,319              & \textbf{1,000}  & 0,484          & 11,250           &  &  &  & KNN-10                                 & 20          & 0,417              & \textbf{1,000}  & 0,588          & 17,500           \\ \cline{1-6} \cline{10-15} 
KNN-10                                 & 20          & 0,319              & 1,000           & \textbf{0,484} & 11,250           &  &  &  & KNN-10                                 & 20          & 0,417              & 1,000           & \textbf{0,588} & 17,500           \\ \cline{1-6} \cline{10-15} 
KNN-15                                 & 20          & \textbf{0,319}     & 1,000           & 0,484          & 10,850           &  &  &  & KNN-15                                 & 20          & \textbf{0,417}     & 1,000           & 0,588          & 15,500           \\ \cline{1-6} \cline{10-15} 
KNN-15                                 & 20          & 0,319              & \textbf{1,000}  & 0,484          & 10,850           &  &  &  & KNN-15                                 & 20          & 0,417              & \textbf{1,000}  & 0,588          & 15,500           \\ \cline{1-6} \cline{10-15} 
KNN-15                                 & 20          & 0,319              & 1,000           & \textbf{0,484} & 10,850           &  &  &  & KNN-15                                 & 20          & 0,417              & 1,000           & \textbf{0,588} & 15,500           \\ \cline{1-6} \cline{10-15} 
KNN-20                                 & 20          & \textbf{0,319}     & 1,000           & 0,484          & 10,850           &  &  &  & KNN-20                                 & 20          & \textbf{0,417}     & 1,000           & 0,588          & 15,500           \\ \cline{1-6} \cline{10-15} 
KNN-20                                 & 20          & 0,319              & \textbf{1,000}  & 0,484          & 10,850           &  &  &  & KNN-20                                 & 20          & 0,417              & \textbf{1,000}  & 0,588          & 15,500           \\ \cline{1-6} \cline{10-15} 
KNN-20                                 & 20          & 0,319              & 1,000           & \textbf{0,484} & 10,850           &  &  &  & KNN-20                                 & 20          & 0,417              & 1,000           & \textbf{0,588} & 15,500           \\ \cline{1-6} \cline{10-15} 
KNN-25                                 & 20          & \textbf{0,319}     & 1,000           & 0,484          & 10,85            &  &  &  & KNN-25                                 & 20          & \textbf{0,417}     & 1,000           & 0,588          & 15,5             \\ \cline{1-6} \cline{10-15} 
KNN-25                                 & 20          & 0,319              & \textbf{1,000}  & 0,484          & 10,85            &  &  &  & KNN-25                                 & 20          & 0,417              & \textbf{1,000}  & 0,588          & 15,5             \\ \cline{1-6} \cline{10-15} 
KNN-25                                 & 20          & 0,319              & 1,000           & \textbf{0,484} & 10,85            &  &  &  & KNN-25                                 & 20          & 0,417              & 1,000           & \textbf{0,588} & 15,5             \\  \hline\hline
\end{tabular}
\end{table*}





==> tables/budgets.tex <==
% !TEX root =  ../MAIN.tex

\begin{table}[tb]
\footnotesize
\begin{tabular}{|p{7mm}|p{1.2cm}|p{10.5cm}|}
\hline

\textbf{Phase}&\textbf{Budget}&\textbf{Strategy}\\
\hline
\multirow{2}{*}{Phase1}&Phase&Infinite, i.e., all the target windows are exercised till stagnation is detected or all the targets are covered.\\
\cline{2-3}
&Reachability&Infinite, i.e., all the paths are traversed in this phase.\\
\cline{2-3}
 &Target&Infinite, i.e., all the target Inputs are tried in this phase.\\
\cline{2-3} 
  &Random Exploration&Set to $\mathit{scaleFactor}*\mathit{NumberOfActionsForActiveWindow}$. In our experiments, we set $\mathit{scaleFactor}$ to $1$ for an overall test budget of one hour, to $2$ for a test budget of five hours. Random exploration is triggered by either \emph{reachTargetNode} or \emph{identifyPathToTarget}.\\
 \hline 
 \multirow{3}{*}{Phase2}&Phase&Set to $\mathit{scaleFactor}*\mathit{NumberOfTargetWindows}$.\\
  \cline{2-3}
& Reachability&Set to $\mathit{scaleFactor}*\mathit{actionsThreshold}$. The value is reset every time a new TargetWindow is identified.  We set $\mathit{actionsThreshold}$ to $25$.\\
 \cline{2-3}
 & Target&Set to be equal to what remains of the {ReachabilityBudget} after the target window is reached. In other words, $\mathit{ReachabilityBudget} + \mathit{TargetBudget} = \mathit{scaleFactor}*\mathit{actionsThreshold}$ \\
  \cline{2-3}
 &Random Exploration&Set to $\mathit{scaleFactor}*\mathit{randomThreshold}$. Random exploration is triggered by either \emph{reachTargetNode} or \emph{identifyPathToTarget}. We set $\mathit{randomThreshold}$ equal to $\mathit{actionsThreshold}$.\\
\hline
 \multirow{3}{*}{Phase3}&Reachability&Not used in this phase.\\
 \cline{2-3}
 & Target&Set to $\mathit{scaleFactor}*\mathit{actionsThreshold}$. It is reset every time a new TargetEvent is identified.\\
 \cline{2-3}
&Random Exploration&Set to $\mathit{scaleFactor}*\mathit{actionsThreshold}$. Random exploration is triggered (1) to explore the related Window, (2) when the related Window cannot be reached through the identified path, (3) 
when the target Window cannot be reached through the identified path (see Section~\ref{sec:phase3}). We set $\mathit{randomThreshold}$ to $5$.\\
% \cline{2-3}
% & Target&.\\
\hline
\end{tabular}
\caption{Strategies adopted, in different \APPR phases, to define the budget allocated to distinct test activities.}
\label{table:budgets}
\end{table}%


==> tables/caseStudies.tex <==
%% !TEX root =  ../MAIN.tex


% !TEX root =  ../MAIN.tex

\begin{table}[tb]
\caption{Selected subject systems.}
\label{table:caseStudies}
\scriptsize
\begin{tabular}{|p{3mm}|
>{\raggedleft\arraybackslash}p{6mm}@{\hspace{1pt}}|
@{\hspace{1pt}}>{\raggedleft\arraybackslash}p{6mm}@{\hspace{1pt}}|
@{\hspace{1pt}}>{\raggedleft\arraybackslash}p{6mm}@{\hspace{1pt}}|
@{\hspace{1pt}}>{\raggedleft\arraybackslash}p{6mm}@{\hspace{1pt}}|
@{\hspace{1pt}}>{\raggedleft\arraybackslash}p{6mm}@{\hspace{1pt}}|
@{\hspace{1pt}}>{\raggedleft\arraybackslash}p{6mm}@{\hspace{1pt}}|
@{\hspace{1pt}}>{\raggedleft\arraybackslash}p{6mm}@{\hspace{1pt}}|
@{\hspace{1pt}}>{\raggedleft\arraybackslash}p{6mm}@{\hspace{1pt}}|
@{\hspace{1pt}}>{\raggedleft\arraybackslash}p{6mm}@{\hspace{1pt}}|
@{\hspace{1pt}}>{\raggedleft\arraybackslash}p{6mm}@{\hspace{1pt}}|
}
\hline
\multicolumn{1}{|c|}{\textbf{App}}
&\multicolumn{1}{@{\hspace{1pt}}
>{\centering\arraybackslash}p{6mm}@{\hspace{1pt}}|}{\textbf{V0}}
&\multicolumn{1}{@{\hspace{1pt}}
>{\centering\arraybackslash}p{6mm}@{\hspace{1pt}}|}{\textbf{V1}}
&\multicolumn{1}{@{\hspace{1pt}}
>{\centering\arraybackslash}p{6mm}@{\hspace{1pt}}|}{\textbf{V2}}
&\multicolumn{1}{@{\hspace{1pt}}
>{\centering\arraybackslash}p{6mm}@{\hspace{1pt}}|}{\textbf{V3}}
&\multicolumn{1}{@{\hspace{1pt}}
>{\centering\arraybackslash}p{6mm}@{\hspace{1pt}}|}{\textbf{V4}}
&\multicolumn{1}{@{\hspace{1pt}}
>{\centering\arraybackslash}p{6mm}@{\hspace{1pt}}|}{\textbf{V5}}
&\multicolumn{1}{@{\hspace{1pt}}
>{\centering\arraybackslash}p{6mm}@{\hspace{1pt}}|}{\textbf{V6}}
&\multicolumn{1}{@{\hspace{1pt}}
>{\centering\arraybackslash}p{6mm}@{\hspace{1pt}}|}{\textbf{V7}}
&\multicolumn{1}{@{\hspace{1pt}}
>{\centering\arraybackslash}p{6mm}@{\hspace{1pt}}|}{\textbf{V8}}
&\multicolumn{1}{@{\hspace{1pt}}
>{\centering\arraybackslash}p{6mm}@{\hspace{1pt}}|}{\textbf{V9}}
\\

%\textbf{\#}&\textbf{Name}&&\\
% \hline
%1&Jamendo
%&V&32& 35& 37& 38\\
%&&AM&1043& 1046& 1094& 1100\\
%&&UM&1043& 82& 53& 2\\
%&&AI&9360& 9383& 10055& 10073\\
%&&UI&9360& 1914& 857& 41\\
\hline
AD
&105& 	111& 	115& 	118& 	122& 	125& 	130& 	131& 	134 &\\
%&\textbf{AM}&260& 	333& 	333& 	333& 	450& 	479& 	540& 	540& 	659&\\
%&\textbf{UM}&260& 	18& 	3& 	12& 	117& 	39& 	28& 	1& 	49&\\
%&\textbf{AI}&3667& 	4832& 	4831& 	4880& 	6613& 	7052& 	8247& 	8251& 	10622&\\
%&\textbf{UI}&3667& 	558& 	21& 	599& 	3393& 	2027& 	1535& 	15& 	2459&\\
\hline
BM
&5.1.0& 		5.10.0& 	5.11.0& 	5.12.0& 	5.13.0& 	5.4.0& 	5.5.0& 	5.6.0& 	5.8.1& 	5.9.0\\
%&\textbf{AM}&10706& 	8724& 	8792& 	8902& 	8926& 	9945& 	10380& 	10696& 	10200& 	8939\\
%&\textbf{UM}&10706& 	649& 	27& 	44& 	25& 	603& 	242& 	553& 	77& 	95\\
%&\textbf{AI}&76649& 	61604& 	62078& 	62937& 	63232& 	71053& 	73082& 	73950& 	72439& 	61618\\
%&\textbf{UI}&76649& 	11182& 	1557& 	2288& 	2101& 	10637& 	6324& 	9484& 	1638& 	3274\\
\hline
CM
&9.1& 		9.2& 	9.3& 	9.4& 	9.5& 	9.6& 	9.7& 	9.8& 	9.9& 	10.0 \\
%&\textbf{AM}&9629& 	9499& 	9599& 	9491& 	9602& 	9761& 	9868& 	9929& 	9884& 	10050 \\
%&\textbf{UM}&9629& 	51& 	37& 	55& 	73& 	119& 	76& 	73& 	12& 	69\\
%&\textbf{AI}&155117& 	154086& 	157036& 	153200& 	155950& 	161914& 	164267& 	165747& 	165747& 	163303 \\
%&\textbf{UI}&155117& 	2726& 	2286& 	2075& 	3160& 	6262& 	2756& 	2340& 	1372& 	3775 \\
\hline
FM
&44& 	53& 	77& 	79& 	82&\multicolumn{5}{c|}{}\\
%&\textbf{AM}&2042& 	2132& 	3422& 	3430& 	3648&\multicolumn{5}{c|}{}\\
%&\textbf{UM}&2042& 	306& 	415& 	11& 	644&\multicolumn{5}{c|}{}\\
%&\textbf{AI}&34389& 	34931& 	48241& 	48294& 	51755&\multicolumn{5}{c|}{}\\
%&\textbf{UI}&34389& 	14510& 	13744& 	703& 	24960&\multicolumn{5}{c|}{}\\
\hline
WI								
&198& 10239& 10263& 10264& 10269 &\multicolumn{5}{c|}{}\\
%&\textbf{AM}&7477& 	8814& 	8751& 	8759& 	8793&\multicolumn{5}{c|}{}\\
%&\textbf{UM}&292& 	1430& 	535& 	13& 	94&\multicolumn{5}{c|}{}\\
%&\textbf{AI}&54759& 	68207& 	69471& 	69533& 	69856&\multicolumn{5}{c|}{}\\
%&\textbf{UI}&6345& 	24536& 	12724& 	281& 	2698&\multicolumn{5}{c|}{}\\
\hline
VP
&3.1.4& 		3.1.5& 	3.1.7& 	3.2.12& 	3.2.2& 	3.2.3& 	3.2.6& 	3.2.7& 	3.2.9&\multicolumn{1}{c|}{}\\
%&\textbf{AM}&6796& 	6843& 	6854& 	8681& 	8544& 	8551& 	8621& 	8641& 	8676&\multicolumn{1}{c|}{}\\
%&\textbf{UM}&6796& 	672& 	26& 	3& 	149& 	13& 	51& 	33& 	42&\multicolumn{1}{c|}{}\\
%&\textbf{AI}&86266& 	87560& 	87886& 	117207& 	115344& 	115412& 	116409& 	116647& 	117071&\multicolumn{1}{c|}{}\\
%&\textbf{UI}&86266& 	34086& 	1522& 	150& 	9611& 	1163& 	3527& 	1961& 	3010&\multicolumn{1}{c|}{}\\
\hline
YM
&1.16.0& 	1.16.1& 	1.16.2& 	1.17.3& 	1.18.1& 	1.19.1& 	1.20.1& 	1.20.3& 	1.20.5& 	1.20.7 \\
%&\textbf{AM}&2932&  2904&  2904& 	2630& 	3105& 	3109& 	3178& 	3255& 	3255& 	3303 \\
%&\textbf{UM}&2932&  5&   4& 	243& 	10& 	16& 	118& 	101& 	12& 	9 \\
%&\textbf{AI}&38015&     37867&     37857& 	34220& 	38219& 	38211& 	39086& 	39439& 	39439& 	39462\\
%&\textbf{UI}&38015&     417&     272& 	10198& 	857& 	588& 	4295& 	3842& 	689& 	961\\
\hline 



\end{tabular}
%Case 8
%The instrumented apk files of these versions cannot be installed.
%Error message: Failure [INSTALL_FAILED_INVALID_APK: Failed to extract native libraries&  res=-2]
%This error sometimes occurs after rebuilding the app with apktool.
%Related issue: https://github.com/iBotPeaches/Apktool/issues/1626

\footnotesize{
\textbf{Legend:} 
AD: Activity Diary.
BM: BBC Mobile.
CM: Citymapper.
FM: Amaze File Manager.
WI: Wikipedia
VP: VLC Player Android
YM: Yahooweather Mobile}

% V: ID of the version under test. 
% %AM: number of methods implemented in V (All Methods). 
% UM: number of Updated Methods in V. 
% %AI: number of instructions in V (All Instructions). 
% UI: number of instructions belonging to updated methods.}
\end{table}%




%\begin{table}[tb]
%\footnotesize
%\begin{tabular}{|p{2mm}|p{1.2cm}|p{1cm}|p{0.5cm}|p{0.9cm}|p{0.5cm}|p{0.9cm}|}
%\hline
%\multicolumn{2}{c}{\textbf{Case study}}&\textbf{Version}&\multicolumn{2}{c}{\textbf{Methods}}&\multicolumn{2}{c}{\textbf{Instructions}}\\
%\textbf{\#}&\textbf{Name}&&\textbf{All}&\textbf{Updated}&\textbf{All}&\textbf{Updated}\\
%\hline
%1&Jamendo
%&V0: 32
%&1043	
%&1043	
%&9360	
%&9360	
%\\
%&&V1: 35	
%&1046	
%&82	
%&9383	
%&1914	
%\\
%&&V2: 37
%&1094	
%&35	
%&10055	
%&857	
%\\
%&&V3: 38
%&1100	
%&2
%&10073
%&41
%\\
%\hline
%2&Wikipedia								
%&V0: 110	&3767 &3767	
%&32208		
%&32208	
%\\
%&&V1: 144	&5009 &446	
%&38913	
%&11000	
%\\
%&&V2: 146	&5646 &195	
%&43753	
%&4157	
%\\
%&&V3: 150	&6435 &108	
%&48761	
%&2441	
%\\
%&&V4: 190	&6943 &370
%&51147	
%&6606		
%\\
%&&V5: 198	&7477 &292
%&54759	
%&6345	
%\\
%&&V6: 10239	&8814 &1430	
%&68207	
%&24536	
%\\
%&&V7: 10263	&8751 &535	
%&69471	
%&12724	
%\\
%&&V8: 10264	&8759 &1430	
%&69533	
%&281	
%\\
%&&V9: 10269	&8793 &94
%&69856
%&2698
%\\
%\hline
%3&ActivityDiary
%&V0: 105	
%&260	
%&260	
%&3667	
%&3667	
%\\
%&&V1: 111
%&333	
%&18	
%&4832	
%&558	
%\\	
%&&V2: 115
%&333	
%&3	
%&4831	
%&21		
%\\
%&&V3: 117
%&333	
%&7	
%&4834	
%&295		
%\\
%&&V4: 118	
%&333	
%&12	
%&4880	
%&599	
%\\
%&&V5: 122
%&450	
%&117	
%&6613	
%&3393		
%\\
%&&V6: 125	
%&479	
%&39	
%&7052	
%&2027	
%\\
%&&V7: 130	
%&540	
%&28	
%&8247	
%&1535	
%\\
%&&V8: 131
%&540	
%&1	
%&8251	
%&15		
%\\
%&&V9: 134
%&659
%&49
%&10622
%&2459
%\\
%\hline
%4&FileManager
%&V0: 44	
%&2042	
%&2042	
%&34389	
%&34389	
%\\
%&&V1: 53	
%&2132	
%&306	
%&34931	
%&14510	
%\\
%&&V2: 77	
%&3422
%&415	
%&48241	
%&13744	
%\\
%&&V3: 79
%&3430	
%&11	
%&48294	
%&703		
%\\
%&&V4: 82	
%&3648
%&644	
%&51755	
%&24960
%\\
%&&V5: 84
%&3648
%&2
%&51789
%&143
%\\
%\hline
%5&Nuzzel
%&V0: 302 
%&4223	
%&4223	
%&40522	
%&40522	
%\\
%&&V1: 316    	
%&4220	
%&8	
%&40449	
%&151	
%\\
%&&V2: 329 
%&4524	
%&717	
%&43309
%&18335	
%\\	
%&&V3: 323 	
%&4498	
%&75	
%&43083	
%&2952	
%\\
%&&V4: 325 	
%&4527	
%&33	
%&43403
%&1593
%\\		
%&&V5: 328 	
%&4650	
%&41	
%&44234
%&1990		
%\\
%&&V6: 329 	
%&4771	
%&21
%&45331
%&647		
%\\
%&&V7: 330	
%&4832	
%&21	
%&45908
%&1378		
%\\
%&&V8: 331	
%&4833	
%&1	
%&45913
%&35		
%\\
%&&V9: 333
%&4833
%&1
%&45916
%&69
%\\
%\hline
%6&Yahoo weather
%&V0: 1.16.0
%&2932	
%&2932	
%&38015	
%&38015	
%\\
%&&V1: 1.16.1    	
%&2904	
%&5	
%&37896	
%&417	
%\\
%&&V2: 1.16.2 
%&2904	
%&4	
%&37857
%&272	
%\\	
%&&V3: 1.17.3 	
%&2630	
%&243	
%&34220	
%&10198	
%\\
%&&V4: 1.18.1 	
%&3105	
%&10	
%&38219
%&857
%\\		
%&&V5: 1.19.1 	
%&3109	
%&16	
%&38211
%&588		
%\\
%&&V6: 1.20.1 	
%&3178	
%&118
%&39086
%&4295		
%\\
%&&V7: 1.20.3	
%&3255	
%&101	
%&39439
%&3842		
%\\
%&&V8: 1.20.5	
%&3255	
%&12	
%&39439
%&689			
%\\
%&&V9: 1.20.7
%&3303
%&9
%&39462
%&961
%\\
%\hline
%7&Wikihow
%&V0: 2.7.3 
%&333	
%&333	
%&3704	
%&3704	
%\\
%&&V1: 2.8.0    	
%&333	
%&111    
%&3992	
%&2279	
%\\
%&&V2: 2.8.1 
%&333	
%&1	
%&3941
%&39	
%\\	
%&&V3: 2.8.3 	
%&333	
%&1
%&3944	
%&42	
%\\
%&&V4: 2.9.1 	
%&325	
%&65	
%&3808
%&1370
%\\		
%&&V5: 2.9.2 	
%&322	
%&4	
%&3761
%&93		
%\\
%&&V6: 2.9.3 	
%&319	
%&18
%&3657
%&543		
%\\
%\hline
%8&BBC Mobile
%&V0: 5.1.0 
%&10706  
%&10706  
%&76649  
%&76649  
%\\
%&&V1: 5.10.0    
%&8724   
%&649    
%&61604  
%&11182  
%\\
%&&V2: 5.11.0    
%&8792   
%&27 
%&62078  
%&1557   
%\\	
%&&V3: 5.12.0    
%&8902   
%&44 
%&62937  
%&2288   
%\\
%&&V4: 5.13.0    
%&8926   
%&25 
%&63232  
%&2101   
%\\		
%&&V5: 5.4.0 
%&9945   
%&603    
%&71053  
%&10637  
%\\
%&&V6: 5.5.0 
%&10380  
%&242    
%&73082  
%&6324   
%\\
%&&V7: 5.6.0 
%&10696  
%&553    
%&73950  
%&9484   
%\\
%&&V8: 5.8.1 
%&10200  
%&77 
%&72439  
%&1638   
%\\
%&&V9: 5.9.0 
%&8939   
%&95 
%&61618  
%&3274   
%\\
%\hline
%9&VLC player
%&V0: 3.1.4
%&6796
%&6796
%&86266
%&86266
%\\
%&&V1: 3.1.5
%&6843
%&672
%&87560
%&34086	
%\\
%&&V2: 3.1.7
%&6854
%&26
%&87886
%&1522	
%\\	
%&&V3: 3.2.12
%&8681
%&3
%&117207
%&150	
%\\
%&&V4: 3.2.2
%&8544
%&149
%&115344
%&9611
%\\		
%&&V5: 3.2.3
%&8551
%&13
%&115412
%&1163		
%\\
%&&V6: 3.2.6
%&8621
%&51
%&116409
%&3527		
%\\
%&&V7: 3.2.7
%&8641
%&33
%&116647
%&1961		
%\\
%&&V8: 3.2.9
%&8676
%&42
%&117071
%&3010	
%\\
%\hline
%10&Citymapper
%&V0: 9.1
%&9629
%&9629
%&155117
%&155117
%\\
%&&V1: 9.2
%&9499
%&51
%&154086
%&2726	
%\\
%&&V2: 9.3
%&9599
%&37
%&157036
%&2286	
%\\	
%&&V3: 9.4
%&9491
%&55
%&153200
%&2075
%\\
%&&V4: 9.5
%&9602
%&73
%&155950
%&3160
%\\		
%&&V5: 9.6
%&9761
%&119
%&161914
%&6262		
%\\
%&&V6: 9.7
%&9868
%&76
%&164267
%&2756		
%\\
%&&V7: 9.8
%&9929
%&73
%&165747
%&2340	
%\\
%&&V8: 9.9
%&9884
%&12
%&163303
%&1372	
%\\
%&&V9: 10
%&10050
%&69
%&174791
%&3775
%\\
%\hline
%\end{tabular}
%\caption{Overview of case study systems.}
%\label{table:caseStudies}
%\end{table}%


==> tables/effectSizeInputs.tex <==
%% !TEX root =  ../MAIN.tex

\begin{table}[tb]
\footnotesize
\caption{Statistical significance and effect size for Figure~\ref{fig:RQ3:Inputs:1} and ~\ref{fig:RQ3:Inputs:5}.}
\label{table:effectSize:inputs}
\begin{tabular}{
|>{\raggedleft\arraybackslash}p{2mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{6mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{6mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{6mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{5mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{5mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{5mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{6mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{6mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{6mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{5mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{5mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{5mm}@{\hspace{1pt}}|
}
\hline
&
\multicolumn{6}{c|}{\textbf{1 hour budget}}&
\multicolumn{6}{c|}{\textbf{5 hours budget}}\\
&
\multicolumn{3}{c|}{\textbf{p-value}}&
\multicolumn{3}{c|}{\textbf{$A_{12}$}}&
\multicolumn{3}{c|}{\textbf{p-value}}&
\multicolumn{3}{c|}{\textbf{$A_{12}$}}\\
\cline{2-13}
\textbf{S}&
D&M&A&
D&M&A&
D&M&A&
D&M&A\\
\hline
1&<0.05&<0.05&<0.05&.018&.000&.000&<0.05&<0.05&<0.05&\R{.630}&.000&.000\\
2&<0.05&<0.05&<0.05&.000&.000&.000&<0.05&<0.05&<0.05&.020&.000&.000\\
3&<0.05&<0.05&<0.05&.039&.000&.000&<0.05&<0.05&<0.05&.093&.000&.000\\
4&<0.05&<0.05&<0.05&.099&.000&.000&<0.05&<0.05&<0.05&.278&.000&.000\\
5&<0.05&<0.05&<0.05&.074&.000&.397&<0.05&<0.05&\R{0.81}&.090&.000&\R{.490}\\
6&<0.05&<0.05&<0.05&.360&.000&.000&\R{0.15}&<0.05&<0.05&.425&.000&.000\\
7&<0.05&<0.05&<0.05&.117&.000&.000&<0.05&<0.05&<0.05&.123&.000&.000\\
8&<0.05&<0.05&<0.05&.405&.000&.000&<0.05&<0.05&<0.05&.075&.000&.000\\
9&<0.05&<0.05&<0.05&\R{.048}&.000&.000&<0.05&<0.05&<0.05&.001&.000&.000\\
\hline
\end{tabular}

\textbf{Legend}: \emph{S}, subject. \emph{D}, comparison with DM2, \emph{M}, Monkey, \emph{A}, APE. We underline the few cases in which statistics indicate that \APPR shows no significant difference (i.e., \emph{p-value} $\ge 0.05$) or no higher chances of generating less instructions ($A_{12} > 0.44$) than state-of-the-art approaches.
\end{table}%




%\begin{table}[tb]
%\footnotesize
%\begin{tabular}{|p{2mm}|p{1.2cm}|p{1cm}|p{0.5cm}|p{0.9cm}|p{0.5cm}|p{0.9cm}|}
%\hline
%\multicolumn{2}{c}{\textbf{Case study}}&\textbf{Version}&\multicolumn{2}{c}{\textbf{Methods}}&\multicolumn{2}{c}{\textbf{Instructions}}\\
%\textbf{\#}&\textbf{Name}&&\textbf{All}&\textbf{Updated}&\textbf{All}&\textbf{Updated}\\
%\hline
%1&Jamendo
%&V0: 32
%&1043	
%&1043	
%&9360	
%&9360	
%\\
%&&V1: 35	
%&1046	
%&82	
%&9383	
%&1914	
%\\
%&&V2: 37
%&1094	
%&35	
%&10055	
%&857	
%\\
%&&V3: 38
%&1100	
%&2
%&10073
%&41
%\\
%\hline
%2&Wikipedia								
%&V0: 110	&3767 &3767	
%&32208		
%&32208	
%\\
%&&V1: 144	&5009 &446	
%&38913	
%&11000	
%\\
%&&V2: 146	&5646 &195	
%&43753	
%&4157	
%\\
%&&V3: 150	&6435 &108	
%&48761	
%&2441	
%\\
%&&V4: 190	&6943 &370
%&51147	
%&6606		
%\\
%&&V5: 198	&7477 &292
%&54759	
%&6345	
%\\
%&&V6: 10239	&8814 &1430	
%&68207	
%&24536	
%\\
%&&V7: 10263	&8751 &535	
%&69471	
%&12724	
%\\
%&&V8: 10264	&8759 &1430	
%&69533	
%&281	
%\\
%&&V9: 10269	&8793 &94
%&69856
%&2698
%\\
%\hline
%3&ActivityDiary
%&V0: 105	
%&260	
%&260	
%&3667	
%&3667	
%\\
%&&V1: 111
%&333	
%&18	
%&4832	
%&558	
%\\	
%&&V2: 115
%&333	
%&3	
%&4831	
%&21		
%\\
%&&V3: 117
%&333	
%&7	
%&4834	
%&295		
%\\
%&&V4: 118	
%&333	
%&12	
%&4880	
%&599	
%\\
%&&V5: 122
%&450	
%&117	
%&6613	
%&3393		
%\\
%&&V6: 125	
%&479	
%&39	
%&7052	
%&2027	
%\\
%&&V7: 130	
%&540	
%&28	
%&8247	
%&1535	
%\\
%&&V8: 131
%&540	
%&1	
%&8251	
%&15		
%\\
%&&V9: 134
%&659
%&49
%&10622
%&2459
%\\
%\hline
%4&FileManager
%&V0: 44	
%&2042	
%&2042	
%&34389	
%&34389	
%\\
%&&V1: 53	
%&2132	
%&306	
%&34931	
%&14510	
%\\
%&&V2: 77	
%&3422
%&415	
%&48241	
%&13744	
%\\
%&&V3: 79
%&3430	
%&11	
%&48294	
%&703		
%\\
%&&V4: 82	
%&3648
%&644	
%&51755	
%&24960
%\\
%&&V5: 84
%&3648
%&2
%&51789
%&143
%\\
%\hline
%5&Nuzzel
%&V0: 302 
%&4223	
%&4223	
%&40522	
%&40522	
%\\
%&&V1: 316    	
%&4220	
%&8	
%&40449	
%&151	
%\\
%&&V2: 329 
%&4524	
%&717	
%&43309
%&18335	
%\\	
%&&V3: 323 	
%&4498	
%&75	
%&43083	
%&2952	
%\\
%&&V4: 325 	
%&4527	
%&33	
%&43403
%&1593
%\\		
%&&V5: 328 	
%&4650	
%&41	
%&44234
%&1990		
%\\
%&&V6: 329 	
%&4771	
%&21
%&45331
%&647		
%\\
%&&V7: 330	
%&4832	
%&21	
%&45908
%&1378		
%\\
%&&V8: 331	
%&4833	
%&1	
%&45913
%&35		
%\\
%&&V9: 333
%&4833
%&1
%&45916
%&69
%\\
%\hline
%6&Yahoo weather
%&V0: 1.16.0
%&2932	
%&2932	
%&38015	
%&38015	
%\\
%&&V1: 1.16.1    	
%&2904	
%&5	
%&37896	
%&417	
%\\
%&&V2: 1.16.2 
%&2904	
%&4	
%&37857
%&272	
%\\	
%&&V3: 1.17.3 	
%&2630	
%&243	
%&34220	
%&10198	
%\\
%&&V4: 1.18.1 	
%&3105	
%&10	
%&38219
%&857
%\\		
%&&V5: 1.19.1 	
%&3109	
%&16	
%&38211
%&588		
%\\
%&&V6: 1.20.1 	
%&3178	
%&118
%&39086
%&4295		
%\\
%&&V7: 1.20.3	
%&3255	
%&101	
%&39439
%&3842		
%\\
%&&V8: 1.20.5	
%&3255	
%&12	
%&39439
%&689			
%\\
%&&V9: 1.20.7
%&3303
%&9
%&39462
%&961
%\\
%\hline
%7&Wikihow
%&V0: 2.7.3 
%&333	
%&333	
%&3704	
%&3704	
%\\
%&&V1: 2.8.0    	
%&333	
%&111    
%&3992	
%&2279	
%\\
%&&V2: 2.8.1 
%&333	
%&1	
%&3941
%&39	
%\\	
%&&V3: 2.8.3 	
%&333	
%&1
%&3944	
%&42	
%\\
%&&V4: 2.9.1 	
%&325	
%&65	
%&3808
%&1370
%\\		
%&&V5: 2.9.2 	
%&322	
%&4	
%&3761
%&93		
%\\
%&&V6: 2.9.3 	
%&319	
%&18
%&3657
%&543		
%\\
%\hline
%8&BBC Mobile
%&V0: 5.1.0 
%&10706  
%&10706  
%&76649  
%&76649  
%\\
%&&V1: 5.10.0    
%&8724   
%&649    
%&61604  
%&11182  
%\\
%&&V2: 5.11.0    
%&8792   
%&27 
%&62078  
%&1557   
%\\	
%&&V3: 5.12.0    
%&8902   
%&44 
%&62937  
%&2288   
%\\
%&&V4: 5.13.0    
%&8926   
%&25 
%&63232  
%&2101   
%\\		
%&&V5: 5.4.0 
%&9945   
%&603    
%&71053  
%&10637  
%\\
%&&V6: 5.5.0 
%&10380  
%&242    
%&73082  
%&6324   
%\\
%&&V7: 5.6.0 
%&10696  
%&553    
%&73950  
%&9484   
%\\
%&&V8: 5.8.1 
%&10200  
%&77 
%&72439  
%&1638   
%\\
%&&V9: 5.9.0 
%&8939   
%&95 
%&61618  
%&3274   
%\\
%\hline
%9&VLC player
%&V0: 3.1.4
%&6796
%&6796
%&86266
%&86266
%\\
%&&V1: 3.1.5
%&6843
%&672
%&87560
%&34086	
%\\
%&&V2: 3.1.7
%&6854
%&26
%&87886
%&1522	
%\\	
%&&V3: 3.2.12
%&8681
%&3
%&117207
%&150	
%\\
%&&V4: 3.2.2
%&8544
%&149
%&115344
%&9611
%\\		
%&&V5: 3.2.3
%&8551
%&13
%&115412
%&1163		
%\\
%&&V6: 3.2.6
%&8621
%&51
%&116409
%&3527		
%\\
%&&V7: 3.2.7
%&8641
%&33
%&116647
%&1961		
%\\
%&&V8: 3.2.9
%&8676
%&42
%&117071
%&3010	
%\\
%\hline
%10&Citymapper
%&V0: 9.1
%&9629
%&9629
%&155117
%&155117
%\\
%&&V1: 9.2
%&9499
%&51
%&154086
%&2726	
%\\
%&&V2: 9.3
%&9599
%&37
%&157036
%&2286	
%\\	
%&&V3: 9.4
%&9491
%&55
%&153200
%&2075
%\\
%&&V4: 9.5
%&9602
%&73
%&155950
%&3160
%\\		
%&&V5: 9.6
%&9761
%&119
%&161914
%&6262		
%\\
%&&V6: 9.7
%&9868
%&76
%&164267
%&2756		
%\\
%&&V7: 9.8
%&9929
%&73
%&165747
%&2340	
%\\
%&&V8: 9.9
%&9884
%&12
%&163303
%&1372	
%\\
%&&V9: 10
%&10050
%&69
%&174791
%&3775
%\\
%\hline
%\end{tabular}
%\caption{Overview of case study systems.}
%\label{table:caseStudies}
%\end{table}%


==> tables/effectSizeInputsRatio.tex <==
%% !TEX root =  ../MAIN.tex

\begin{table}[tb]
\footnotesize
\caption{Statistical significance and effect size for target instructions/inputs ratios.}
\label{table:effectSize:ratio}
\begin{tabular}{
|>{\raggedleft\arraybackslash}p{2mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{6mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{6mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{6mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{5mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{5mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{5mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{6mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{6mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{6mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{5mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{5mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{5mm}@{\hspace{1pt}}|
}
\hline
&
\multicolumn{6}{c|}{\textbf{1 hour budget}}&
\multicolumn{6}{c|}{\textbf{5 hours budget}}\\
&
\multicolumn{3}{c|}{\textbf{p-value}}&
\multicolumn{3}{c|}{\textbf{$A_{12}$}}&
\multicolumn{3}{c|}{\textbf{p-value}}&
\multicolumn{3}{c|}{\textbf{$A_{12}$}}\\
\cline{2-13}
\textbf{S}&
D&M&A&
D&M&A&
D&M&A&
D&M&A\\
\hline
1&\R{0.10}&<0.05&<0.05&.728&1.00&.975&\R{0.69}&<0.05&<0.05&\R{.555}&.963&.901\\
2&\R{0.17}&<0.05&<0.05&.703&.906&.875&\R{0.14}&<0.05&<0.05&.719&.938&.875\\
3&\R{0.29}&\R{0.09}&\R{0.09}&.700&.820&.820&\R{0.25}&\R{0.08}&\R{0.17}&.720&.840&.760\\
4&\R{0.33}&<0.05&\R{0.05}&.636&.895&.772&\R{0.38}&<0.05&<0.05&.623&.895&.747\\
5&\R{0.17}&<0.05&<0.05&.691&1.00&.901&\R{0.17}&<0.05&<0.05&.691&.950&.827\\
6&\R{0.63}&<0.05&<0.05&.583&1.00&1.00&\R{0.52}&<0.05&<0.05&.611&1.00&1.00\\
7&\R{0.27}&<0.05&<0.05&.654&1.00&1.00&\R{0.27}&<0.05&<0.05&.654&1.00&1.00\\
8&\R{0.60}&<0.05&<0.05&.578&1.00&.953&\R{0.92}&<0.05&<0.05&\R{.516}&.968&.906\\
9&\R{0.39}&<0.05&<0.05&.642&1.00&1.00&<0.05&<0.05&<0.05&.914&1.00&1.00
\\
\hline
\end{tabular}

\textbf{Legend}: \emph{S}, subject. \emph{D}, comparison with DM2, \emph{M}, Monkey, \emph{A}, APE. We underline the few cases in which statistics indicate that \APPR shows no significant difference (i.e., \emph{p-value} $\ge 0.05$) or no higher likelihood of achieving a higher instructions/inputs ratio (i.e., $A_{12} < 0.56$) than state-of-the-art approaches.
\end{table}%




%\begin{table}[tb]
%\footnotesize
%\begin{tabular}{|p{2mm}|p{1.2cm}|p{1cm}|p{0.5cm}|p{0.9cm}|p{0.5cm}|p{0.9cm}|}
%\hline
%\multicolumn{2}{c}{\textbf{Case study}}&\textbf{Version}&\multicolumn{2}{c}{\textbf{Methods}}&\multicolumn{2}{c}{\textbf{Instructions}}\\
%\textbf{\#}&\textbf{Name}&&\textbf{All}&\textbf{Updated}&\textbf{All}&\textbf{Updated}\\
%\hline
%1&Jamendo
%&V0: 32
%&1043	
%&1043	
%&9360	
%&9360	
%\\
%&&V1: 35	
%&1046	
%&82	
%&9383	
%&1914	
%\\
%&&V2: 37
%&1094	
%&35	
%&10055	
%&857	
%\\
%&&V3: 38
%&1100	
%&2
%&10073
%&41
%\\
%\hline
%2&Wikipedia								
%&V0: 110	&3767 &3767	
%&32208		
%&32208	
%\\
%&&V1: 144	&5009 &446	
%&38913	
%&11000	
%\\
%&&V2: 146	&5646 &195	
%&43753	
%&4157	
%\\
%&&V3: 150	&6435 &108	
%&48761	
%&2441	
%\\
%&&V4: 190	&6943 &370
%&51147	
%&6606		
%\\
%&&V5: 198	&7477 &292
%&54759	
%&6345	
%\\
%&&V6: 10239	&8814 &1430	
%&68207	
%&24536	
%\\
%&&V7: 10263	&8751 &535	
%&69471	
%&12724	
%\\
%&&V8: 10264	&8759 &1430	
%&69533	
%&281	
%\\
%&&V9: 10269	&8793 &94
%&69856
%&2698
%\\
%\hline
%3&ActivityDiary
%&V0: 105	
%&260	
%&260	
%&3667	
%&3667	
%\\
%&&V1: 111
%&333	
%&18	
%&4832	
%&558	
%\\	
%&&V2: 115
%&333	
%&3	
%&4831	
%&21		
%\\
%&&V3: 117
%&333	
%&7	
%&4834	
%&295		
%\\
%&&V4: 118	
%&333	
%&12	
%&4880	
%&599	
%\\
%&&V5: 122
%&450	
%&117	
%&6613	
%&3393		
%\\
%&&V6: 125	
%&479	
%&39	
%&7052	
%&2027	
%\\
%&&V7: 130	
%&540	
%&28	
%&8247	
%&1535	
%\\
%&&V8: 131
%&540	
%&1	
%&8251	
%&15		
%\\
%&&V9: 134
%&659
%&49
%&10622
%&2459
%\\
%\hline
%4&FileManager
%&V0: 44	
%&2042	
%&2042	
%&34389	
%&34389	
%\\
%&&V1: 53	
%&2132	
%&306	
%&34931	
%&14510	
%\\
%&&V2: 77	
%&3422
%&415	
%&48241	
%&13744	
%\\
%&&V3: 79
%&3430	
%&11	
%&48294	
%&703		
%\\
%&&V4: 82	
%&3648
%&644	
%&51755	
%&24960
%\\
%&&V5: 84
%&3648
%&2
%&51789
%&143
%\\
%\hline
%5&Nuzzel
%&V0: 302 
%&4223	
%&4223	
%&40522	
%&40522	
%\\
%&&V1: 316    	
%&4220	
%&8	
%&40449	
%&151	
%\\
%&&V2: 329 
%&4524	
%&717	
%&43309
%&18335	
%\\	
%&&V3: 323 	
%&4498	
%&75	
%&43083	
%&2952	
%\\
%&&V4: 325 	
%&4527	
%&33	
%&43403
%&1593
%\\		
%&&V5: 328 	
%&4650	
%&41	
%&44234
%&1990		
%\\
%&&V6: 329 	
%&4771	
%&21
%&45331
%&647		
%\\
%&&V7: 330	
%&4832	
%&21	
%&45908
%&1378		
%\\
%&&V8: 331	
%&4833	
%&1	
%&45913
%&35		
%\\
%&&V9: 333
%&4833
%&1
%&45916
%&69
%\\
%\hline
%6&Yahoo weather
%&V0: 1.16.0
%&2932	
%&2932	
%&38015	
%&38015	
%\\
%&&V1: 1.16.1    	
%&2904	
%&5	
%&37896	
%&417	
%\\
%&&V2: 1.16.2 
%&2904	
%&4	
%&37857
%&272	
%\\	
%&&V3: 1.17.3 	
%&2630	
%&243	
%&34220	
%&10198	
%\\
%&&V4: 1.18.1 	
%&3105	
%&10	
%&38219
%&857
%\\		
%&&V5: 1.19.1 	
%&3109	
%&16	
%&38211
%&588		
%\\
%&&V6: 1.20.1 	
%&3178	
%&118
%&39086
%&4295		
%\\
%&&V7: 1.20.3	
%&3255	
%&101	
%&39439
%&3842		
%\\
%&&V8: 1.20.5	
%&3255	
%&12	
%&39439
%&689			
%\\
%&&V9: 1.20.7
%&3303
%&9
%&39462
%&961
%\\
%\hline
%7&Wikihow
%&V0: 2.7.3 
%&333	
%&333	
%&3704	
%&3704	
%\\
%&&V1: 2.8.0    	
%&333	
%&111    
%&3992	
%&2279	
%\\
%&&V2: 2.8.1 
%&333	
%&1	
%&3941
%&39	
%\\	
%&&V3: 2.8.3 	
%&333	
%&1
%&3944	
%&42	
%\\
%&&V4: 2.9.1 	
%&325	
%&65	
%&3808
%&1370
%\\		
%&&V5: 2.9.2 	
%&322	
%&4	
%&3761
%&93		
%\\
%&&V6: 2.9.3 	
%&319	
%&18
%&3657
%&543		
%\\
%\hline
%8&BBC Mobile
%&V0: 5.1.0 
%&10706  
%&10706  
%&76649  
%&76649  
%\\
%&&V1: 5.10.0    
%&8724   
%&649    
%&61604  
%&11182  
%\\
%&&V2: 5.11.0    
%&8792   
%&27 
%&62078  
%&1557   
%\\	
%&&V3: 5.12.0    
%&8902   
%&44 
%&62937  
%&2288   
%\\
%&&V4: 5.13.0    
%&8926   
%&25 
%&63232  
%&2101   
%\\		
%&&V5: 5.4.0 
%&9945   
%&603    
%&71053  
%&10637  
%\\
%&&V6: 5.5.0 
%&10380  
%&242    
%&73082  
%&6324   
%\\
%&&V7: 5.6.0 
%&10696  
%&553    
%&73950  
%&9484   
%\\
%&&V8: 5.8.1 
%&10200  
%&77 
%&72439  
%&1638   
%\\
%&&V9: 5.9.0 
%&8939   
%&95 
%&61618  
%&3274   
%\\
%\hline
%9&VLC player
%&V0: 3.1.4
%&6796
%&6796
%&86266
%&86266
%\\
%&&V1: 3.1.5
%&6843
%&672
%&87560
%&34086	
%\\
%&&V2: 3.1.7
%&6854
%&26
%&87886
%&1522	
%\\	
%&&V3: 3.2.12
%&8681
%&3
%&117207
%&150	
%\\
%&&V4: 3.2.2
%&8544
%&149
%&115344
%&9611
%\\		
%&&V5: 3.2.3
%&8551
%&13
%&115412
%&1163		
%\\
%&&V6: 3.2.6
%&8621
%&51
%&116409
%&3527		
%\\
%&&V7: 3.2.7
%&8641
%&33
%&116647
%&1961		
%\\
%&&V8: 3.2.9
%&8676
%&42
%&117071
%&3010	
%\\
%\hline
%10&Citymapper
%&V0: 9.1
%&9629
%&9629
%&155117
%&155117
%\\
%&&V1: 9.2
%&9499
%&51
%&154086
%&2726	
%\\
%&&V2: 9.3
%&9599
%&37
%&157036
%&2286	
%\\	
%&&V3: 9.4
%&9491
%&55
%&153200
%&2075
%\\
%&&V4: 9.5
%&9602
%&73
%&155950
%&3160
%\\		
%&&V5: 9.6
%&9761
%&119
%&161914
%&6262		
%\\
%&&V6: 9.7
%&9868
%&76
%&164267
%&2756		
%\\
%&&V7: 9.8
%&9929
%&73
%&165747
%&2340	
%\\
%&&V8: 9.9
%&9884
%&12
%&163303
%&1372	
%\\
%&&V9: 10
%&10050
%&69
%&174791
%&3775
%\\
%\hline
%\end{tabular}
%\caption{Overview of case study systems.}
%\label{table:caseStudies}
%\end{table}%


==> tables/effectSizeRQ21.tex <==
%% !TEX root =  ../MAIN.tex


% !TEX root =  ../MAIN.tex

\begin{table}[tb]
\footnotesize
\caption{Statistical significance and effect size for RQ2.}
\label{table:effectSize:rq21}
\begin{tabular}{
|>{\raggedleft\arraybackslash}p{2mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{6mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{6mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{6mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{5mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{5mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{5mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{6mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{6mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{6mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{5mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{5mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{5mm}@{\hspace{1pt}}|
}
\hline
&
\multicolumn{6}{c|}{\textbf{1 hour budget}}&
\multicolumn{6}{c|}{\textbf{5 hours budget}}\\
&
\multicolumn{3}{c|}{\textbf{p-value}}&
\multicolumn{3}{c|}{\textbf{$A_{12}$}}&
\multicolumn{3}{c|}{\textbf{p-value}}&
\multicolumn{3}{c|}{\textbf{$A_{12}$}}\\
\cline{2-13}
\textbf{C}&
D&M&A&
D&M&A&
D&M&A&
D&M&A\\
\hline
&
\multicolumn{12}{c|}{\textbf{Coverage of target methods}}\\
\cline{2-13}
1&<0.05&<0.05&<0.05&.857&.994&.956&<0.05&<0.05&\R{0.14}&.703&.935&.564\\
2&<0.05&<0.05&<0.05&.733&.868&.703&<0.05&<0.05&<0.05&.774&.832&.623\\
3&\R{0.41}&<0.05&<0.05&\R{.548}&.795&.684&\R{0.61}&<0.05&0.99&\R{.529}&.767&\R{.501}\\
4&\R{0.16}&<0.05&\R{0.07}&.560&.852&.577&\R{0.16}&<0.05&\R{0.08}&.560&.760&.575\\
5&<0.05&<0.05&<0.05&.735&.814&.920&<0.05&<0.05&<0.05&.713&.702&.841\\
6&\R{0.08}&<0.05&<0.05&.587&.838&.689&\R{0.2}&<0.05&<0.05&.564&.719&.681\\
7&<0.05&<0.05&<0.05&.614&.836&.762&\R{0.78}&<0.05&<0.05&\R{.488}&.879&.879\\
8&\R{0.23}&<0.05&<0.05&\R{.554}&.997&.972&\R{0.05}&<0.05&<0.05&.588&.995&.892\\
9&<0.05&<0.05&<0.05&.587&.981&.878&<0.05&<0.05&<0.05&.685&.992&.918\\
\hline
&\multicolumn{12}{c|}{\textbf{Coverage of target instructions}}\\
\cline{2-13}
1&<0.05&<0.05&<0.05&.853&.991&.936&<0.05&<0.05&\R{0.15}&.735&.884&.562\\
2&<0.05&<0.05&<0.05&.707&.843&.783&<0.05&<0.05&<0.05&.756&.829&.721\\
3&\R{0.31}&<0.05&\R{0.14}&\R{.559}&.774&.585&\R{0.18}&<0.05&\R{0.70}&.577&.705&\R{.478}\\
4&<0.05&<0.05&\R{0.07}&.600&.861&.579&\R{0.05}&<0.05&<0.05&.584&.764&.594\\
5&<0.05&<0.05&<0.05&.684&.748&.886&<0.05&<0.05&<0.05&.659&.623&.822\\
6&\R{0.42}&<0.05&<0.05&\R{.542}&.788&.827&\R{0.47}&<0.05&<0.05&\R{.538}&.727&.786\\
7&<0.05&<0.05&<0.05&.598&.735&.695&\R{0.65}&<0.05&<0.05&\R{.480}&.780&.780\\
8&\R{0.06}&<0.05&<0.05&.586&.999&.984&\R{0.33}&<0.05&<0.05&.633&.999&.936\\
9&0.05&<0.05&<0.05&.584&.980&.822&<0.05&<0.05&<0.05&.671&.988&.896\\
\hline
\end{tabular}

\textbf{Legend}: \emph{C}, case study. \emph{D}, comparison with DM2, \emph{M}, Monkey, \emph{A}, APE. We underline the few cases in which statistics indicate that \APPR shows no significant difference (i.e., \emph{p-value} $\ge 0.05$ ) or no higher likelihood (i.e., $A_{12} < 0.56$) of covering more targets  than state-of-the-art approaches.
\end{table}%


==> tables/effectSizeRQ22.tex <==
%% !TEX root =  ../MAIN.tex


% !TEX root =  ../MAIN.tex

\begin{table}[tb]
\footnotesize
\caption{Statistical significance and effect size for RQ2.2.}
\label{table:effectSize:rq22}
\begin{tabular}{
|>{\raggedleft\arraybackslash}p{2mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{5mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{5mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{5mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{4mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{4mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{4mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{5mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{5mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{5mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{4mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{4mm}@{\hspace{1pt}}|
>{\raggedleft\arraybackslash}p{4mm}@{\hspace{1pt}}|
}
\hline
\textbf{}&
\multicolumn{6}{c|}{\textbf{1 hour budget}}&
\multicolumn{6}{c|}{\textbf{5 hours budget}}\\
&
\multicolumn{3}{c|}{\textbf{p-value}}&
\multicolumn{3}{c|}{\textbf{$A_{12}$}}&
\multicolumn{3}{c|}{\textbf{p-value}}&
\multicolumn{3}{c|}{\textbf{$A_{12}$}}\\
\cline{2-13}
\textbf{C}&
D&M&A&
D&M&A&
D&M&A&
D&M&A\\
\hline
&
\multicolumn{12}{c|}{\textbf{Coverage of target methods}}\\
\cline{2-13}
1&<0.05&<0.05&<0.05&.890&1.00&.890
&<0.05&<0.05&<0.05&.640&.820&\R{.320}\\
2&<0.05&<0.05&<0.05&\R{.370}&.990&.850
&<0.05&<0.05&<0.05&.890&1.00&1.00\\
3&\R{0.80}&<0.05&<0.05&\R{.350}&1.00&.900
&\R{0.46}&<0.05&0.99&.845&.975&.600\\
4&<0.05&<0.05&<0.05&.960&1.00&.950
&<0.05&<0.05&<0.05&.950&1.00&.980\\
5&<0.05&<0.05&<0.05&1.00&1.00&1.00
&<0.05&<0.05&<0.05&\R{.200}&\R{.280}&1.00\\
6&<0.05&<0.05&<0.05&.650&1.00&.920&
<0.05&<0.05&<0.05&.690&1.00&.630\\
7&<0.05&<0.05&<0.05&.950&1.00&.970
&<0.05&<0.05&<0.05&\R{.530}&1.00&1.00\\
8&\R{0.46}&<0.05&<0.05&\R{.530}&1.00&.990
&<0.05&<0.05&<0.05&.810&1.00&1.00\\
9&<0.05&<0.05&\R{1.00}&.650&1.00&1.00
&<0.05&<0.05&\R{1.00}&.800&1.00&1.00\\
\hline
&\multicolumn{12}{c|}{\textbf{Coverage of target instructions}}\\
\cline{2-13}
1&<0.05&<0.05&<0.05&.900&.990&.880
&<0.05&<0.05&<0.05&.660&.760&\R{.350}\\
2&<0.05&<0.05&<0.05&.620&.980&.560
&<0.05&<0.05&<0.05&.940&.980&\R{.200}\\
3&\R{0.81}&<0.05&<0.05&\R{.490}&1.00&.980
&<0.05&<0.05&<0.05&.960&1.00&.760\\
4&<0.05&<0.05&<0.05&.950&1.00&.940
&<0.05&<0.05&<0.05&.940&1.00&.980\\
5&<0.05&<0.05&<0.05&1.00&1.00&1.00
&<0.05&<0.05&<0.05&\R{.200}&\R{.280}&1.00\\
6&<0.05&<0.05&<0.05&.790&1.00&.610
&<0.05&<0.05&<0.05&.720&1.00&\R{.400}\\
7&<0.05&<0.05&<0.05&.970&1.00&.990
&<0.05&<0.05&<0.05&\R{.550}&1.00&1.00\\
8&<0.05&<0.05&<0.05&.660&1.00&.990
&<0.05&<0.05&<0.05&.900&1.00&1.00\\
9&\R{0.05}&<0.05&\R{1.00}&.680&1.00&.728
&<0.05&<0.05&\R{1.00}&.810&1.00&.656\\
\hline
\end{tabular}
\textbf{Legend}: \emph{C}, case study. \emph{D}, comparison with DM2, \emph{M}, Monkey, \emph{A}, APE. We underline the few cases in which statistics indicate that \APPR shows no significant difference (i.e., \emph{p-value} $\ge 0.05$ ) or no higher likelihood (i.e., $A_{12} < 0.56$) of covering more targets  than state-of-the-art approaches.
\end{table}%


==> tables/ewtgmodel.tex <==
% \begin{table*}
% \footnotesize
% \begin{tabular}{ |p{2cm}|p{1.5cm}|p{2cm}|p{9cm}|  }
%  \hline
%  \textbf{EWTG Element} & \textbf{Type} & \textbf{Attribute / Reference name} &
%  \textbf{Description}\\
%  \hline
%  \multirow{4}{*}{Window}   & Attribute & className & for Activity and Dialog, this is the name of implementation class; for OptionsMenu and ContextMenu, this is the className of the Activity declaring the menu.\\
%  \cline{2-4}
%   & Attribute & windowType & i.e., Activity, Dialog, OptionsMenu, ContextMenu. \\
%  \cline{2-4}
% & Reference & ownerActivity & reserved only for Dialog; this is the Activity that use the dialog.\\
%  \cline{2-4}
%  & Attribute & createdLocation & reserved only for Dialog; this is the statement (instruction) where the dialog is instantiated. \\
%  \hline
%  \multirow{4}{*}{Widget}  & Attribute & className & the class name of Widget's type (e.g. LinearLayout, TextView). \\
%  \cline{2-4}
%  & Attribute & resourceId & the id name assigned to the Widget in an xml layout. \\
%  \cline{2-4}
%  & Reference& parent & the containing widget \\
%  \cline{2-4}
%  & Attribute& xpath & the XMLPath of the widget, which helps to locate the widget in a GUI tree. \\
%  \hline
%  \multirow{4}{*}{Transition} & Attribute& action & e.g. click, swipe, press back. \\
%  \cline{2-4}
%  &Attribute &targetWidget & the widget trigger with the action. Some actions do not need a target (e.g. press back, press menu.)\\
%  \cline{2-4}
%  &Reference &source & the window before executing the transition\\
%  \cline{2-4}
%  &Reference& destination & the window after executing the transition\\
%  \hline
% \end{tabular}
% \caption{EWTG elements considered when deriving an RCVDiff model to compare EWTGs belonging to two App versions}
% \label{tab:ewtgmodel}
% \end{table*}

\begin{table}
\footnotesize
\begin{tabular}{ |p{2.7cm}|p{1cm}|p{4cm}|  }
 \hline
 \textbf{EWTG Element} & \textbf{RCVDiff Element} & \textbf{Description}\\
 \hline
 Window instance  & MElement& A Window.\\
 className attribute  & MAttribute& implementng class or className declaring the menu (for menus)\\
  windowType attribute & MAttribute&Activity, Dialog, OptionsMenu, or ContextMenu\\
 ownerActivity association & MReference& Activity that uses the Window, if a Window is a Dialog.\\
 createdLocation attribute & MAttribute & Statement instantiating the dialog. \\
 \hline
 Widget instance  & MElement& A Widget.\\
 className attribute & MAttribute &  Widget's type (e.g. LinearLayout). \\
 resourceId attribute & MAttribute & ID assigned to the Widget in a layout. \\
 parent attribute & MReference&  Containing Widget. \\
 xpath attribute & MAttribute&  XMLPath of the widget. \\
 \hline
 Transition instance  & MElement& A Transition.\\
 action attribute & MAttribute& Action (e.g., click, swipe, press back). \\
 targetWidget attribute & MAttribute & The target of the corresponding Action.\\
 source attribute &MReference & Active Window before the Transition.\\
 destination attribute& MReference& Active Window after the Transition.\\
 \hline
\end{tabular}
\caption{EWTG elements considered when deriving an RCVDiff model to compare EWTGs belonging to two App versions}
\label{tab:ewtgmodel}
\end{table}

==> tables/exerciseStrategies.tex <==
% !TEX root =  ../MAIN.tex

\begin{table}[tb]
\footnotesize
\begin{tabular}{|p{2cm}|p{11cm}|}
\hline

\textbf{Widget type}&\textbf{Input generation procedure}\\
\hline
Any widget& Trigger an InputEvent among the ones for which an event handler has been declared.\\
\hline
Textarea & Randomly apply one of the following: 
(1) leave it empty,
(2) reuse a string already used in the past,
(3) reuse a string already used for the same widget,
(4) reuse a string literal extracted with static analysis,
(5) use a randomly generated alphabetic string~\cite{Borges-Droidmate2-ASE-2018},
(6) use a randomly generated non alphabetic char.\\
\hline
Radio buttons and check boxes& Randomly select one of the possible options (e.g., checked/not checked, for check boxes). \\
\hline
Widgets with manual input& Randomly select one of the available InputInstances, if more than one is available, and then assign the specified value.\\
\hline
Intent& If the current activity declares an Intent, it triggers the Intent specified by the engineer.\\
\hline
\end{tabular}
\caption{\APPR Input generation procedures.}
\label{table:exerciseWidgets}
\end{table}%


==> tables/fap.tex <==
% !TEX root =  ../MAIN.tex

\begin{figure}[htp]
\footnotesize
\begin{tabular}{|p{0.5cm}|p{7.5cm}|}
\hline
$w_1=$& $\langle \{i=0,t=FL,a=\emptyset\}, \{i=0,t=LL,a=\emptyset\}, \{i=1,t=FL,a=\emptyset\} \rangle$\\
$w_2=$& $\langle \{i=0,t=FL,a=\emptyset\}, \{i=0,t=LL,a=\emptyset\}, \{i=1,t=FL,a=\emptyset\}, \{i=1,t=LL,a=\emptyset\}  \rangle$\\
$w_3=$& $\langle \{i=0,t=FL,a=\emptyset\}, \{i=0,t=LL,a=\emptyset\}, \{i=1,t=FL,a=\emptyset\}, \{i=2,t=LL,a=\emptyset\}, \{i=1,t=LL,a=\mathit{Radio}\}  \rangle$\\
\hline
\end{tabular}
FL: FrameLayout, LL=LinearLayout, LV=ListView, TW=TextView.

\caption{Full Attribute Paths for the widgets in Figure~\ref{}.}
\label{fig:fullAttributePaths}
\end{figure}%


==> tables/features.tex <==
\begin{table}[tb]
\caption{Description of features in data}
\centering
\label{Table:features}
\begin{tabular}{ll}
\hline \hline
\multicolumn{1}{c}{\textbf{Feature}} & \multicolumn{1}{c}{\textbf{Description}} \\ \hline \hline
IP\_V1                               & IP of host in initial configuration      \\ \hline
IP\_V2                               & IP of host in updated configuration      \\ \hline
MAC\_V1                              & MAC of host in initial configuration     \\ \hline
MAC\_V2                              & MAC of host in updated configuration     \\ \hline
Port                                 & (state of port) * \textbf{\textit{N}}                      \\ \hline
IP\_Changed                          & To track if IP changed during update     \\ \hline
MAC\_Changed                         & To track if MAC cahnged during update    \\ \hline \hline
\end{tabular}
% \vspace{20mm}
\begin{minipage}[t]{7cm}
%\begin{tabbing}
\textbf{Abbreviation Terms}:\\
\hspace{2mm}\textbf{\textit{N}}: Unique ports identified in initial and updated xml files(Number of ports may vary based on senarios, hence its dynamic in nature to deal with ports).  
%\end{tabbing}
\end{minipage}


\end{table}

==> tables/manualInputs.tex <==
%% !TEX root =  ../MAIN.tex


% !TEX root =  ../MAIN.tex

\begin{table}[tb]
\footnotesize
\caption{Case studies with manual inputs.}
\label{table:manualInputs}
\begin{tabular}{
|@{\hspace{1pt}}p{1.5cm}@{\hspace{1pt}}|
p{6cm}|
p{1cm}|
p{1cm}|
p{1cm}|
}
\hline
\textbf{Case study}&
\textbf{Feature tested}&
\multicolumn{1}{c|}{\textbf{\# Windows}}&
\multicolumn{1}{c|}{\textbf{\# Data fields}}&
\multicolumn{1}{c|}{\textbf{\# Instances}}\\
\hline
\multirow{2}{*}{Wikipedia}&
Log-in functionality&1&2&1\\
\cline{2-5}
&Creation of a new account&
1&
4&
14								
\\
\hline
\multirow{2}{*}{VLC}
&
Play a video stream using a URL
&
1
&
1
&
2
\\
\cline{2-5}
&
Populate the library with all the videos on the device
&
1
&
1
&
1
\\
\hline
Nuzzel
&
Request an e-mail newsletter
&
1
&
1
&
1
\\
\hline
\end{tabular}
\end{table}%




%\begin{table}[tb]
%\footnotesize
%\begin{tabular}{|p{2mm}|p{1.2cm}|p{1cm}|p{0.5cm}|p{0.9cm}|p{0.5cm}|p{0.9cm}|}
%\hline
%\multicolumn{2}{c}{\textbf{Case study}}&\textbf{Version}&\multicolumn{2}{c}{\textbf{Methods}}&\multicolumn{2}{c}{\textbf{Instructions}}\\
%\textbf{\#}&\textbf{Name}&&\textbf{All}&\textbf{Updated}&\textbf{All}&\textbf{Updated}\\
%\hline
%1&Jamendo
%&V0: 32
%&1043	
%&1043	
%&9360	
%&9360	
%\\
%&&V1: 35	
%&1046	
%&82	
%&9383	
%&1914	
%\\
%&&V2: 37
%&1094	
%&35	
%&10055	
%&857	
%\\
%&&V3: 38
%&1100	
%&2
%&10073
%&41
%\\
%\hline
%2&Wikipedia								
%&V0: 110	&3767 &3767	
%&32208		
%&32208	
%\\
%&&V1: 144	&5009 &446	
%&38913	
%&11000	
%\\
%&&V2: 146	&5646 &195	
%&43753	
%&4157	
%\\
%&&V3: 150	&6435 &108	
%&48761	
%&2441	
%\\
%&&V4: 190	&6943 &370
%&51147	
%&6606		
%\\
%&&V5: 198	&7477 &292
%&54759	
%&6345	
%\\
%&&V6: 10239	&8814 &1430	
%&68207	
%&24536	
%\\
%&&V7: 10263	&8751 &535	
%&69471	
%&12724	
%\\
%&&V8: 10264	&8759 &1430	
%&69533	
%&281	
%\\
%&&V9: 10269	&8793 &94
%&69856
%&2698
%\\
%\hline
%3&ActivityDiary
%&V0: 105	
%&260	
%&260	
%&3667	
%&3667	
%\\
%&&V1: 111
%&333	
%&18	
%&4832	
%&558	
%\\	
%&&V2: 115
%&333	
%&3	
%&4831	
%&21		
%\\
%&&V3: 117
%&333	
%&7	
%&4834	
%&295		
%\\
%&&V4: 118	
%&333	
%&12	
%&4880	
%&599	
%\\
%&&V5: 122
%&450	
%&117	
%&6613	
%&3393		
%\\
%&&V6: 125	
%&479	
%&39	
%&7052	
%&2027	
%\\
%&&V7: 130	
%&540	
%&28	
%&8247	
%&1535	
%\\
%&&V8: 131
%&540	
%&1	
%&8251	
%&15		
%\\
%&&V9: 134
%&659
%&49
%&10622
%&2459
%\\
%\hline
%4&FileManager
%&V0: 44	
%&2042	
%&2042	
%&34389	
%&34389	
%\\
%&&V1: 53	
%&2132	
%&306	
%&34931	
%&14510	
%\\
%&&V2: 77	
%&3422
%&415	
%&48241	
%&13744	
%\\
%&&V3: 79
%&3430	
%&11	
%&48294	
%&703		
%\\
%&&V4: 82	
%&3648
%&644	
%&51755	
%&24960
%\\
%&&V5: 84
%&3648
%&2
%&51789
%&143
%\\
%\hline
%5&Nuzzel
%&V0: 302 
%&4223	
%&4223	
%&40522	
%&40522	
%\\
%&&V1: 316    	
%&4220	
%&8	
%&40449	
%&151	
%\\
%&&V2: 329 
%&4524	
%&717	
%&43309
%&18335	
%\\	
%&&V3: 323 	
%&4498	
%&75	
%&43083	
%&2952	
%\\
%&&V4: 325 	
%&4527	
%&33	
%&43403
%&1593
%\\		
%&&V5: 328 	
%&4650	
%&41	
%&44234
%&1990		
%\\
%&&V6: 329 	
%&4771	
%&21
%&45331
%&647		
%\\
%&&V7: 330	
%&4832	
%&21	
%&45908
%&1378		
%\\
%&&V8: 331	
%&4833	
%&1	
%&45913
%&35		
%\\
%&&V9: 333
%&4833
%&1
%&45916
%&69
%\\
%\hline
%6&Yahoo weather
%&V0: 1.16.0
%&2932	
%&2932	
%&38015	
%&38015	
%\\
%&&V1: 1.16.1    	
%&2904	
%&5	
%&37896	
%&417	
%\\
%&&V2: 1.16.2 
%&2904	
%&4	
%&37857
%&272	
%\\	
%&&V3: 1.17.3 	
%&2630	
%&243	
%&34220	
%&10198	
%\\
%&&V4: 1.18.1 	
%&3105	
%&10	
%&38219
%&857
%\\		
%&&V5: 1.19.1 	
%&3109	
%&16	
%&38211
%&588		
%\\
%&&V6: 1.20.1 	
%&3178	
%&118
%&39086
%&4295		
%\\
%&&V7: 1.20.3	
%&3255	
%&101	
%&39439
%&3842		
%\\
%&&V8: 1.20.5	
%&3255	
%&12	
%&39439
%&689			
%\\
%&&V9: 1.20.7
%&3303
%&9
%&39462
%&961
%\\
%\hline
%7&Wikihow
%&V0: 2.7.3 
%&333	
%&333	
%&3704	
%&3704	
%\\
%&&V1: 2.8.0    	
%&333	
%&111    
%&3992	
%&2279	
%\\
%&&V2: 2.8.1 
%&333	
%&1	
%&3941
%&39	
%\\	
%&&V3: 2.8.3 	
%&333	
%&1
%&3944	
%&42	
%\\
%&&V4: 2.9.1 	
%&325	
%&65	
%&3808
%&1370
%\\		
%&&V5: 2.9.2 	
%&322	
%&4	
%&3761
%&93		
%\\
%&&V6: 2.9.3 	
%&319	
%&18
%&3657
%&543		
%\\
%\hline
%8&BBC Mobile
%&V0: 5.1.0 
%&10706  
%&10706  
%&76649  
%&76649  
%\\
%&&V1: 5.10.0    
%&8724   
%&649    
%&61604  
%&11182  
%\\
%&&V2: 5.11.0    
%&8792   
%&27 
%&62078  
%&1557   
%\\	
%&&V3: 5.12.0    
%&8902   
%&44 
%&62937  
%&2288   
%\\
%&&V4: 5.13.0    
%&8926   
%&25 
%&63232  
%&2101   
%\\		
%&&V5: 5.4.0 
%&9945   
%&603    
%&71053  
%&10637  
%\\
%&&V6: 5.5.0 
%&10380  
%&242    
%&73082  
%&6324   
%\\
%&&V7: 5.6.0 
%&10696  
%&553    
%&73950  
%&9484   
%\\
%&&V8: 5.8.1 
%&10200  
%&77 
%&72439  
%&1638   
%\\
%&&V9: 5.9.0 
%&8939   
%&95 
%&61618  
%&3274   
%\\
%\hline
%9&VLC player
%&V0: 3.1.4
%&6796
%&6796
%&86266
%&86266
%\\
%&&V1: 3.1.5
%&6843
%&672
%&87560
%&34086	
%\\
%&&V2: 3.1.7
%&6854
%&26
%&87886
%&1522	
%\\	
%&&V3: 3.2.12
%&8681
%&3
%&117207
%&150	
%\\
%&&V4: 3.2.2
%&8544
%&149
%&115344
%&9611
%\\		
%&&V5: 3.2.3
%&8551
%&13
%&115412
%&1163		
%\\
%&&V6: 3.2.6
%&8621
%&51
%&116409
%&3527		
%\\
%&&V7: 3.2.7
%&8641
%&33
%&116647
%&1961		
%\\
%&&V8: 3.2.9
%&8676
%&42
%&117071
%&3010	
%\\
%\hline
%10&Citymapper
%&V0: 9.1
%&9629
%&9629
%&155117
%&155117
%\\
%&&V1: 9.2
%&9499
%&51
%&154086
%&2726	
%\\
%&&V2: 9.3
%&9599
%&37
%&157036
%&2286	
%\\	
%&&V3: 9.4
%&9491
%&55
%&153200
%&2075
%\\
%&&V4: 9.5
%&9602
%&73
%&155950
%&3160
%\\		
%&&V5: 9.6
%&9761
%&119
%&161914
%&6262		
%\\
%&&V6: 9.7
%&9868
%&76
%&164267
%&2756		
%\\
%&&V7: 9.8
%&9929
%&73
%&165747
%&2340	
%\\
%&&V8: 9.9
%&9884
%&12
%&163303
%&1372	
%\\
%&&V9: 10
%&10050
%&69
%&174791
%&3775
%\\
%\hline
%\end{tabular}
%\caption{Overview of case study systems.}
%\label{table:caseStudies}
%\end{table}%


==> tables/tableSignatures.tex <==
\begin{table}[]
\begin{tabular}{ |c|c|c| } 
 \hline
 \textbf{EWTG Element} & \textbf{Attribute/Reference} &
 \textbf{Description}\\
 \hline
 Window & className & \\
 \hline
  & windowType & \\
 \hline
& ownerActivity & \\
 \hline
 & createdLocation & \\
\end{tabular}
\caption{Signatures of different types of element}
\label{tab:signature}
\end{table}
